AG-BFGS: Foundations for Accelerated Geometry Learning

We introduce an accelerated geometry-learning framework for BFGS that incorporates momentum into the learning of Hessian inverse approximations. We prove that the resulting accelerated updates satisfy explicit stability conditions and preserve positive definiteness within admissible parameter regions. Numerical experiments demonstrate consistent improvements over the corresponding non-accelerated schemes while maintaining numerical stability. These results provide the first rigorous theoretical foundation for accelerated quasi-Newton learning and bridge the gap between empirical observations and mathematical guarantees for accelerated second-order methods.

==> bfgs.tex <==
\section{The BFGS Method} \label{sec:bfgs}

In quasi-Newton methods, the classical BFGS algorithm iteratively constructs an approximation $X_k \approx H_k^{-1}$ using only first-order information. The update is designed to satisfy the secant condition, ensuring consistency between the displacement in the decision space and the observed variation in the gradient.

Let
\[
s_k = x_{k+1} - x_k, 
\qquad
\zeta_k = \nabla f(x_{k+1}) - \nabla f(x_k),
\]
where $s_k$ denotes the step in the decision variable and $\zeta_k$ the corresponding change in the gradient. The secant condition requires that
\[
X_{k+1} \zeta_k = s_k,
\]
while symmetry, $X_{k+1} = X_{k+1}^\top$, is imposed to preserve the structure of the Hessian approximation.

The BFGS update can be characterized as the solution to the variational problem
\begin{equation}
X_{k+1} = \arg\min_X \|X - X_k\|_F^2 
\quad \text{subject to} \quad X \zeta_k = s_k, \; X = X^\top,
\label{eq:bfgs_opt}
\end{equation}
whose closed-form solution is given by
\begin{equation}
X_{k+1} 
= \frac{s_k s_k^\top}{s_k^\top \zeta_k}
+ \left(I - \frac{s_k \zeta_k^\top}{s_k^\top \zeta_k}\right)
X_k
\left(I - \frac{\zeta_k s_k^\top}{s_k^\top \zeta_k}\right).
\label{eq:bfgs_closed_form}
\end{equation}

The first term in \eqref{eq:bfgs_closed_form} enforces the secant condition, while the second term corresponds to the minimal correction in Frobenius norm, $\|A\|_F = \sqrt{\operatorname{Tr}(A^\top A)}$, that preserves symmetry and, under the curvature condition $\zeta_k^\top s_k > 0$, positive definiteness of $X_{k+1}$.

This formulation provides the foundation for the extensions considered in this work. In particular, the variational interpretation in \eqref{eq:bfgs_opt} enables the introduction of additional mechanisms directly into the update of $X_k$. In the following sections, this structure is leveraged to incorporate acceleration terms inspired by \cite{nesterov1983method} and controlled stochastic perturbations in the search direction, while maintaining the desirable convergence properties of the quasi-Newton framework.

==> bfgs_acc_sto.tex <==
\section{Introduction}
\label{chap:localsearch}

A otimização many-objective envolve, de forma inerente, um delicado equilíbrio entre exploração global e refinamento local. Enquanto os algoritmos evolutivos many-objective (MaOEAs), apresentados no Capítulo , são particularmente eficazes na exploração do espaço de decisão e na manutenção da diversidade populacional, sua natureza estocástica pode limitar a velocidade de convergência em regiões próximas ao fronte de Pareto. Em especial, quando soluções já se encontram em regiões promissoras, mecanismos adicionais de intensificação tornam-se desejáveis para aprimorar a precisão e a qualidade final das soluções obtidas.

Nesse contexto, a busca local determinística emerge como um componente estratégico para o refinamento de soluções em problemas contínuos. Diferentemente da dinâmica populacional dos MaOEAs, métodos determinísticos exploram de forma sistemática informações de primeira e segunda ordem, permitindo trajetórias de convergência mais direcionadas e controladas. A integração conceitual entre exploração evolutiva e intensificação determinística constitui, portanto, uma linha natural de investigação em otimização many-objective.

A escolha de métodos quasi-Newton para desempenhar esse papel está diretamente relacionada às propriedades matemáticas e computacionais desejadas. Tais métodos combinam eficiência numérica, rápida convergência local e sólida fundamentação teórica, sendo amplamente empregados na literatura de otimização contínua [\cite{prudente2022quasi, morovati2018quasi}]. Além disso, sua formulação é particularmente adequada a problemas escalarizados, nos quais a estrutura multiobjetivo foi incorporada à função objetivo por meio das estratégias de decomposição e escalarização discutidas no Capítulo .

Este capítulo tem como objetivo apresentar os fundamentos teóricos dos métodos quasi-Newton e, em particular, dos algoritmos BFGS e SQP, estabelecendo a base para as extensões propostas nesta tese. Inicialmente, são revisados os princípios clássicos do método BFGS e suas propriedades estruturais. Em seguida, introduz-se uma variante acelerada e estocástica, cuja formulação busca preservar características fundamentais de convergência ao mesmo tempo em que melhora a eficiência prática. Posteriormente, discute-se o método SQP, incluindo sua formulação a partir das condições de Karush–Kuhn–Tucker e a estrutura do subproblema quadrático associado. Por fim, apresenta-se uma versão acelerada do SQP, proposta neste trabalho, acompanhada de análise teórica comparativa.

Dessa forma, este capítulo consolida a segunda grande contribuição da tese: o desenvolvimento e a análise de mecanismos determinísticos de intensificação baseados em atualizações quasi-Newton, concebidos para posterior integração com algoritmos evolutivos many-objective. A estrutura apresentada fornece o arcabouço matemático necessário para a construção de estratégias híbridas robustas, cuja avaliação experimental será conduzida nos capítulos subsequentes.





\section{Os Métodos Quasi-Newton}

Os métodos quasi-Newton, e em particular o BFGS (Broyden–Fletcher–Goldfarb–Shanno) \cite{broyden1970convergence, fletcher1970new, goldfarb1970family, shanno1970conditionin}, constituem uma das abordagens mais consolidadas para otimização não linear sem restrições. O método baseia-se em construir, a cada iteração, uma aproximação positiva definida da matriz Hessiana, atualizada a partir de informações de gradiente. Essa estratégia permite alcançar desempenho de segunda ordem sem necessidade de calcular derivadas de ordem superior, conciliando eficiência e precisão. Devido a essas características, o BFGS tem sido amplamente utilizado tanto em problemas determinísticos quanto em contextos de otimização de larga escala e aplicações multiobjetivo [\cite{nocedal2006numerical, prudente2024global}]. 

Apesar de suas propriedades de convergência bem estabelecidas, o método BFGS clássico apresenta limitações quando aplicado a funções de alta dimensionalidade, superfícies mal condicionadas ou problemas multimodais, situações em que pode ocorrer estagnação ou convergência lenta [\cite{dai2002convergence, dai2013perfect, mascarenhas2004bfgs}]. Esses desafios motivaram o desenvolvimento de variantes que introduzem mecanismos de aceleração e estocasticidade, buscando aprimorar a velocidade de convergência e a robustez frente à incerteza e à não convexidade.

Entre as estratégias de aceleração, destaca-se o método proposto por \cite{nesterov1983method}, que introduz um termo de inércia na atualização iterativa, permitindo antecipar o movimento e acelerar a convergência em problemas convexos. A ideia de incorporar aceleração a métodos quasi-Newton tem sido explorada em diferentes contextos (\cite{su2016differential, gower2018accelerated, botev2017nesterov}), com destaque para a formulação de \cite{gower2018accelerated}, que adapta o conceito de momento de Nesterov à atualização da inversa da Hessiana, mantendo estabilidade teórica e baixo custo adicional. Essa linha de pesquisa evidenciou que a introdução de um componente de inércia pode reduzir significativamente o número de iterações necessárias para atingir o ótimo, sem comprometer as propriedades de convergência superlinear do esquema BFGS.

Paralelamente, a incorporação de estocasticidade em métodos quasi-Newton surgiu como alternativa para aumentar a capacidade exploratória e a tolerância a ruído em avaliações de gradiente. Métodos como os de \cite{byrd2016stochastic, wang2017stochastic, schraudolph2007stochastic} investigaram formas de adaptar o BFGS a contextos estocásticos, ajustando o cálculo dos pares de correção e introduzindo amostragem parcial de dados ou gradientes. Trabalhos mais recentes avançaram nessa direção, analisando a influência do ruído de forma controlada sobre o desempenho dos métodos de segunda ordem. Em particular, \cite{shi2022noise} propõem um algoritmo BFGS tolerante a ruído, modificando os pares de atualização para lidar com gradientes imprecisos; \cite{guo2023overview} apresentam uma revisão abrangente das variantes estocásticas quasi-Newton, destacando seu papel na escalabilidade e robustez numérica; \cite{amos2020algorithm} introduzem %o \emph{QNSTOP}, 
um algoritmo quasi-Newton para otimização sob ruído; e \cite{peng2025finding} exploram explicitamente a geração de direções de busca sob incerteza, propondo estratégias para manter desempenho consistente em ambientes aleatórios. Esses estudos evidenciam a relevância da estocasticidade não apenas como elemento de modelagem de ruído, mas também como mecanismo ativo de melhoria da exploração e prevenção de estagnação.

Mais recentemente, algumas abordagens buscaram combinar aceleração e estocasticidade em um mesmo arcabouço quasi-Newton. Entre elas, destaca-se o \emph{Regularized Stochastic Nesterov’s Accelerated Quasi-Newton Method} (RES-NAQ) proposto por \cite{makmuang2023regularized}, no qual o termo de aceleração é associado a gradientes ruidosos para aprimorar o desempenho em ambientes incertos. Essa integração entre momento e aleatoriedade vem se mostrando promissora para equilibrar exploração e estabilidade, especialmente em problemas de alta dimensionalidade.

Neste capítulo, propõe-se uma formulação que combina a aceleração de Nesterov, conforme \cite{gower2018accelerated}, com um componente estocástico inspirado nas abordagens citadas anteriormente \cite{peng2025finding, shi2022noise, guo2023overview, amos2020algorithm}. Embora existam diversos métodos quasi-Newton projetados para cenários com ruído nos gradientes ou nas atualizações de Hessianas (por exemplo, \cite{shi2022noise, guo2023overview}), e estudos que modelam a geração da direção de busca sob incerteza \cite{peng2025finding}, a presente proposta difere ao introduzir explicitamente um mecanismo de ruído controlado na direção de busca. Essa escolha tem como objetivo ampliar a capacidade exploratória do método e reduzir a probabilidade de estagnação em mínimos locais, preservando a estrutura quasi-Newton e as propriedades de convergência associadas ao esquema acelerado.

A seguir, apresenta-se uma revisão do método BFGS tradicional, destacando seus fundamentos teóricos e a formulação matricial da atualização quasi-Newton. Essa exposição estabelece a base notacional e conceitual necessária para as seções subsequentes, nas quais são introduzidas as extensões acelerada e estocástica. A primeira incorpora o termo de inércia de Nesterov ao processo de atualização da inversa da Hessiana, enquanto a segunda integra um componente de ruído controlado à direção de busca, analisando seus efeitos sobre a estabilidade e a capacidade exploratória do método.


\section{Método BFGS}



Nos métodos quasi-Newton, o BFGS tradicional constrói uma aproximação $X_k \approx H_k^{-1}$ de forma iterativa, utilizando apenas informações de primeira ordem. A cada iteração, a atualização de $X_k$ é realizada de modo a satisfazer a chamada condição de secante, que impõe coerência entre o deslocamento no espaço de variáveis e a variação observada no gradiente.

Considere os vetores
$$
s_k = x_{k+1} - x_k, 
\qquad
\zeta_k = \nabla f(x_{k+1}) - \nabla f(x_k),
$$
onde $s_k$ representa o passo realizado na variável de decisão $x_k$, e $y_k$ representa a variação no gradiente entre as iterações $k$ e $k+1$. A condição de secante exige que a nova aproximação $X_{k+1}$ satisfaça:
$$
X_{k+1} y_k = s_k,
$$
isto é, a nova matriz inversa deve mapear a diferença de gradientes $y_k$ no deslocamento real $s_k$. Além disso, impõe-se a simetria $X_{k+1} = X_{k+1}^\top$ para preservar as propriedades da Hessiana.

Dessa forma, a atualização de BFGS pode ser formulada como um problema de minimização quadrática:
\begin{equation}
X_{k+1} = \arg\min_X \|X - X_k\|_F^2 
\quad \text{sujeito a} \quad X \zeta_k = s_k, \; X = X^\top,
\label{eq:bfgs_opt}
\end{equation}
cuja solução analítica é:
\begin{equation}
X_{k+1} 
= \frac{s_k s_k^\top}{s_k^\top \zeta_k}
+ \left(I - \frac{s_k \zeta_k^\top}{s_k^\top \zeta_k}\right)
X_k
\left(I - \frac{\zeta_k s_k^\top}{s_k^\top \zeta_k}\right).
\label{eq:bfgs_closed_form}
\end{equation}

A primeira parcela em~\eqref{eq:bfgs_closed_form} garante o atendimento da condição de secante, enquanto o segundo termo ajusta $X_k$ de forma simétrica e mínima em norma de Frobenius, $\|A\|_F=\sqrt{\operatorname{Tr}(A^\top A)}$. Essa combinação assegura que $X_{k+1}$ permaneça uma aproximação simétrica e definida positiva de $H^{-1}$, desde que $y_k^\top s_k > 0$ — condição que normalmente é satisfeita sob convexidade local ou controle do tamanho do passo.

A formulação acima fornece a base para o desenvolvimento de variantes aceleradas e estocásticas do método. Do ponto de vista geométrico, o processo de atualização de BFGS pode ser interpretado como uma projeção de $X_k$ sobre o conjunto de matrizes que satisfazem a condição de secante. Essa perspectiva permite empregar técnicas de aceleração originalmente propostas por \cite{nesterov1983method}, adaptadas para o domínio matricial, de modo a refinar a aproximação de $X_k$ de forma mais eficiente. Além disso, a notação aqui estabelecida será utilizada na formulação da direção de busca, onde será incorporado um componente estocástico controlado, responsável por introduzir variabilidade no processo de descida sem alterar a estrutura quasi-Newton do algoritmo.


\subsection{Método Acelerado de Nesterov}
\label{sec:nesterov_intro}

A otimização baseada em gradientes constitui a base dos métodos de primeira ordem, em que o vetor de decisão é atualizado iterativamente pela direção de descida mais acentuada da função objetivo. No método do gradiente puro, a atualização é dada por
\begin{equation}
x_{k+1} = x_k - \alpha \nabla f(x_k),
\label{eq:gradiente_puro}
\end{equation}
onde $\alpha > 0$ representa o tamanho de passo. Sob hipóteses de convexidade e suavidade (isto é, gradiente Lipschitz-contínuo), esse esquema garante convergência com taxa da ordem de $O(1/k)$, típica dos métodos de primeira ordem [\cite{bubeck2015convex}]. Entretanto, quando a curvatura da função é fortemente desigual entre diferentes direções do espaço de decisão — situação típica em problemas mal condicionados — o método pode apresentar oscilações e reduzir sua taxa efetiva de avanço em direção ao mínimo.

Com o intuito de reduzir essas oscilações, \cite{polyak1964some} desenvolveu o método com momento inercial, conhecido na literatura como \emph{heavy-ball method}. \footnote{Polyak descreve o método por analogia com o movimento de uma bola pesada rolando em um campo de energia potencial, onde o termo inercial (ou “momento”) modela o impulso da bola.} 
Nesse método, cada iteração incorpora parte do deslocamento anterior, produzindo um movimento mais coerente com a curvatura local e reduzindo oscilações de alta frequência. O esquema iterativo pode ser escrito como
\begin{align}
v_{k+1} &= \mu v_k - \alpha \nabla f(x_k), \label{eq:momentum_v}\\
x_{k+1} &= x_k + v_{k+1}, \label{eq:momentum_x}
\end{align}
em que $v_k$ representa a velocidade acumulada e $\mu \in [0,1)$ é o parâmetro de inércia (ou fator de momentum) que controla o peso dado ao histórico recente. Quando $\mu = 0$, \eqref{eq:momentum_v}–\eqref{eq:momentum_x} reduzem-se ao gradiente puro~\eqref{eq:gradiente_puro}; para $\mu$ mais elevado, a iteração tende a acumular impulso e a progredir rapidamente ao longo das direções de menor curvatura, o que pode acelerar a convergência prática, embora sem garantia da taxa ótima de convergência teórica em problemas convexos suaves.

Para obter aceleração ótima em termos de taxa assintótica,  \cite{nesterov1983method} propôs um método modificado em que o gradiente não é mais avaliado em $x_k$, mas sim em um ponto extrapolado que antecipa a direção de deslocamento. 
A formulação acelerada pode ser escrita como
\begin{align}
y_k &= x_k + \mu (x_k - x_{k-1}), \label{eq:nesterov_y}\\
x_{k+1} &= y_k - \alpha \nabla f(y_k), \label{eq:nesterov_x}
\end{align}
onde $\alpha > 0$ é o passo de descida e $\mu \in [0,1)$ regula a intensidade da extrapolação inercial. A diferença essencial em relação ao método de Polyak é que, em~\eqref{eq:nesterov_x}, o gradiente é avaliado em $y_k$, o ponto extrapolado, e não em $x_k$. Essa modificação é crucial: ela permite provar que, sob hipóteses de convexidade e suavidade com constante de Lipschitz $L$, a taxa de convergência do método é $O(1/k^2)$, que é assintoticamente ótima para métodos de primeira ordem (\cite{bubeck2015convex, su2016differential}).

É comum, para fins analíticos e também de implementação estável, introduzir uma terceira sequência $\{v_k\}$ que representa o estado inercial suavizado do método, incorporando gradualmente a informação das iterações anteriores. Em uma formulação equivalente, a iteração pode ser expressa como
\begin{align}
y_k &= (1 - \mu)\, x_k + \mu\, v_k, \label{eq:nesterov_y_alt}\\[3pt]
x_{k+1} &= y_k - \alpha \nabla f(y_k), \label{eq:nesterov_x_alt}\\[3pt]
v_{k+1} &= (1 - \mu)\, v_k + \mu\, x_{k+1}. \label{eq:nesterov_v}
\end{align}
Nessa forma, $y_k$ é uma combinação convexa entre o ponto atual $x_k$ e o estado inercial $v_k$; em seguida, executa-se uma etapa de descida em $y_k$; e, por fim, atualiza-se $v_{k+1}$ para refletir a nova informação. A variável $v_k$ desempenha, portanto, o papel de memória dinâmica do método, acumulando a direção de movimento de iterações anteriores de maneira suave  \cite{su2016differential}].
Esse arranjo de três componentes — extrapolação ($y_k$), descida ($x_{k+1}$) e atualização inercial ($v_{k+1}$) — é a expressão algorítmica da aceleração de Nesterov.

A escolha dos parâmetros $\alpha$ e $\mu$ é decisiva tanto para a estabilidade quanto para a velocidade de convergência do método. Em geral, esses parâmetros são determinados a partir das propriedades espectrais da função objetivo, isto é, de sua curvatura e da taxa de variação de seu gradiente. Seja $f:\mathbb{R}^n \to \mathbb{R}$ uma função convexa e continuamente diferenciável. Diz-se que o gradiente de $f$ é $L$-Lipschitz-contínuo se existe $L>0$ tal que
$$
\|\nabla f(x) - \nabla f(y)\| \le L \|x - y\|, \quad \forall x,y.
$$
A constante $L$ estabelece um limite superior para a variação do gradiente, caracterizando o grau de suavidade da função. Analogamente, $f$ é dita $\mu_f$-fortemente convexa se existe $\mu_f>0$ tal que
$$
f(y) \ge f(x) + \nabla f(x)^\top (y - x) + \frac{\mu_f}{2}\|y - x\|^2, \quad \forall x,y.
$$
Essa desigualdade impõe um limite inferior para a curvatura da função, representado pela constante $\mu_f$, que expressa o grau de forte convexidade. Assim, $L$ e $\mu_f$ delimitam, respectivamente, a máxima e a mínima curvatura local da função, sendo fundamentais para a análise de estabilidade e taxa de convergência de métodos de gradiente. 

Para funções quadráticas da forma $f(x)=\tfrac{1}{2}x^\top A x - b^\top x + c$, com matriz Hessiana $A$ simétrica definida positiva (SPD), essas constantes correspondem, respectivamente, ao maior e ao menor autovalor de $A$, isto é, $L=\lambda_{\max}(A)$ e $\mu_f=\lambda_{\min}(A)$. %O quociente $\kappa = L / \mu_f$ define o número de condição do problema, o qual quantifica o grau de anisotropia da curvatura e influencia diretamente a velocidade de convergência dos métodos baseados em gradiente.

No cenário idealmente conhecido da análise clássica — funções convexas e $L$-suaves, com $L$ conhecido —, costuma-se adotar $\alpha = 1/L$. Já o parâmetro $\mu$ é ajustado de modo a refletir a geometria do problema. Para funções $\mu_f$-fortemente convexas, com constante de forte convexidade $\mu_f > 0$, a combinação $\alpha = 1/L$ e
$$
\mu = \frac{\sqrt{L} - \sqrt{\mu_f}}{\sqrt{L} + \sqrt{\mu_f}}
$$
leva a uma convergência linear em taxa $(1 - \sqrt{\mu_f/L})^k$. Para o caso meramente convexo ($\mu_f = 0$), adotam-se sequências variáveis $\mu_k$ que satisfazem relações do tipo $\mu_k \approx 1 - O(1/k)$, garantindo a taxa $O(1/k^2)$. Ver \cite{bubeck2015convex, nesterov1983method}.

Na prática de otimização sobre funções para as quais as constantes $L$ (suavidade) e $\mu_f$ (forte convexidade) não são conhecidas ou são difíceis de estimar, a definição teórica de $\mu$ torna-se inviável. Nesses casos, a escolha do fator de momentum passa a ser empírica e depende do equilíbrio entre estabilidade e aceleração. A análise de estabilidade, %via \emph{Integral Quadratic Constraints}, 
apresentada por \cite{lessard2016analysis}, fundamenta-se na formulação inercial proposta originalmente por Polyak e mostra que, para essa classe de métodos, a convergência deixa de ser garantida quando a razão de condicionamento $L/\mu_f$ ultrapassa determinados limites. Dentro dessa faixa de estabilidade, valores de $\mu$ muito próximos de~1 tendem a induzir oscilações, enquanto intervalos moderados, tipicamente entre $0.8$ e $0.95$, mantêm o comportamento estável mesmo em problemas mal condicionados.
Por outro lado, \cite{sutskever2013importance} demonstraram empiricamente, no contexto do método de Nesterov, que o desempenho pode ser aprimorado pela adoção de um cronograma crescente para $\mu$, partindo de valores em torno de~$0.9$ e evoluindo até $\mu_{\max}\in\{0.99,\,0.995,\,0.999\}$, seguido de uma redução final para estabilização da convergência. Em linha semelhante, \cite{liu2020improved} propuseram uma estratégia adaptativa em múltiplos estágios, %(\emph{Multistage SGDM}), 
na qual o parâmetro de momentum é atualizado de forma monotonicamente crescente ao longo das iterações, conciliando aceleração e estabilidade mesmo sob gradientes ruidosos. Essas estratégias de momentum dinâmico têm se mostrado eficazes em contextos não convexos, estocásticos ou de escalarização multiobjetivo, nos quais o perfil espectral do gradiente — isto é, a distribuição das componentes do gradiente em relação às direções de curvatura da função — varia ao longo da execução.

A definição do tamanho de passo $\alpha$ desempenha papel igualmente crítico na estabilidade do método. Em teoria, $\alpha$ é limitado superiormente por $1/L$, garantindo que cada iteração produza um ponto com valor de função não crescente ( \cite{bubeck2015convex, nesterov2013introductory}). No entanto, quando $L$ não é conhecido ou é apenas aproximado, adota-se um valor empírico inicial de $\alpha$ que pode ser posteriormente ajustado de forma adaptativa. Estratégias comuns incluem a redução progressiva de $\alpha$ ao longo das iterações (\cite{ruder2016overview}),   ou a sua adaptação baseada em critérios locais, como a magnitude do gradiente ou o histórico recente de convergência, \cite{peng2025finding}. Um passo excessivamente pequeno torna o método lento, enquanto um passo grande pode levar a oscilações e perda de estabilidade, especialmente em conjunto com valores elevados de $\mu$. Dessa forma, o par $(\alpha,\,\mu)$ deve ser calibrado de maneira coerente, de modo que o aumento do momentum seja compensado por um passo mais conservador, assegurando um regime dinâmico estável e eficiente.

Em síntese, pode-se interpretar $\alpha$ como o parâmetro que controla a magnitude do deslocamento de descida a cada iteração e $\mu$ como o parâmetro que regula a persistência inercial do movimento. No regime teórico clássico, ambos são determinados a partir de constantes de suavidade e curvatura globais. No regime prático e não estacionário, como no caso em que a função objetivo resulta de uma escalarização que pode variar ao longo da busca, esses parâmetros passam a ser ajustados de forma empírica ou adaptativa, mantendo a ideia central da aceleração sem depender de hipóteses globais fortes.

\section{BFGS Acelerado}
\label{sec:bfgs_acelerado}
Os princípios de aceleração, formulados originalmente para variáveis vetoriais, podem ser transferidos para espaços matriciais. Em particular, é possível aplicar não a aceleração sobre o vetor de decisão em si, mas sobre a iteração que constrói aproximações sucessivas da inversa da Hessiana. Nessa formulação, discutida em \cite{gower2018accelerated}
, a variável inercial deixa de ser um vetor de posição e passa a ser uma matriz auxiliar que acumula informação histórica sobre aproximações de $H^{-1}$. Em outras palavras, a aceleração atua diretamente sobre a sequência de matrizes $\{X_k\}$ que aproximam a inversa da Hessiana $H^{-1}$, e não sobre o vetor de decisão $x_k$.

A transposição do método de Nesterov para o espaço das matrizes requer algumas modificações conceituais e algébricas. Diferentemente das variáveis vetoriais, as aproximações da inversa da Hessiana pertencem ao conjunto das matrizes simétricas definidas positivas (SPD), denotado por $\mathbb{S}_{++}^n$. Esse conjunto não forma um espaço vetorial: combinações lineares arbitrárias de matrizes SPD podem resultar em matrizes indefinidas. Consequentemente, as operações lineares de extrapolação utilizadas no método clássico, como $X_k + \mu(X_k - X_{k-1})$, não preservam a positividade definida e, portanto, não são adequadas para atualizar diretamente a sequência $\{X_k\}$.

Assim como no caso vetorial, deseja-se incorporar um termo de inércia que antecipe a direção de evolução da métrica quasi-Newton. No entanto, como vimos, a geometria não linear do cone $\mathbb{S}_{++}^n$ impede o uso de uma única variável de momentum, como ocorre na forma clássica de Nesterov. Por isso, no esquema matricial usaremos dois parâmetros distintos: um que controle a interpolação segura entre as aproximações da inversa da Hessiana (aqui denotado por $\rho\in(0,1)$) e outro que regule a suavização inercial da sequência auxiliar (denotado por $\beta\in[0,1)$). Essa separação é necessária para preservar a positividade definida das matrizes e evitar instabilidades numéricas decorrentes de extrapolações excessivas.

A sequência auxiliar $\{V_k\}$, então, acumula, de forma suavizada, a informação histórica do processo de atualização. A cada iteração, combina-se $V_k$ e $X_k$ por meio de uma combinação convexa, que garante que o ponto intermediário permaneça dentro do cone $\mathbb{S}_{++}^n$:
\begin{equation}
Y_k = (1-\rho)X_k + \rho V_k,
\label{eq:yk_iter}
\end{equation}
em que $\rho$ controla a contribuição inercial e desempenha papel análogo ao fator de momentum do método vetorial, porém restrito a uma interpolação convexa para assegurar que $Y_k \in \mathbb{S}_{++}^n$, ou seja $Y_k \succ0$. O ponto $Y_k$ atua, assim, como um análogo matricial do ponto extrapolado $y_k$ de Nesterov: antecipa a direção de movimento no espaço das métricas sem comprometer a coerência geométrica do método.

A atualização quasi-Newton é então executada sobre $Y_k$, resultando em uma nova aproximação $X_{k+1}$:
\begin{equation}
X_{k+1} = \Phi_{\text{BFGS}}(Y_k;\,s_k,\zeta_k),
\label{eq:xk_iter}
\end{equation}
onde $\Phi_{\text{BFGS}}$ representa a transformação BFGS aplicada aos vetores
$$
s_k = x_{k+1}-x_k, \qquad \zeta_k = \nabla f(x_{k+1})-\nabla f(x_k).
$$
Essa etapa preserva a positividade definida sempre que $s_k^\top\zeta_k>0$, condição usual em métodos quasi-Newton. Dessa forma, a projeção quasi-Newton garante que $X_{k+1}\in\mathbb{S}_{++}^n$ mesmo que $Y_k$ apresente leve desvio da região interior do cone.

Após essa etapa, a variável auxiliar $V_k$ é atualizada iterativamente por uma média convexa que incorpora a nova aproximação da inversa da Hessiana e, ao mesmo tempo, mantém memória do estado anterior:
\begin{equation}
V_{k+1} = (1-\beta)V_k + \beta X_{k+1},
\label{eq:vk_iter}
\end{equation}
onde $\beta$ regula a taxa de amortecimento inercial. Valores baixos de $\beta$ produzem uma atualização mais suave e estável, enquanto valores próximos de $1$ tornam o método mais responsivo às variações recentes da curvatura local.

As equações~\eqref{eq:yk_iter}–\eqref{eq:vk_iter} definem um esquema de aceleração discreto e numericamente estável, no qual:
\begin{enumerate}
    \item \textbf{A combinação convexa} entre $X_k$ e $V_k$ preserva a positividade definida, assegurando que $Y_k\in\mathbb{S}_{++}^n$;
    \item \textbf{A atualização quasi-Newton} $\Phi_{\text{BFGS}}$ mantém $X_{k+1}$ simétrica e definida positiva sob a condição $s_k^\top\zeta_k>0$;
    \item \textbf{A atualização inercial} de $V_k$ suaviza a dinâmica, controlando a propagação do termo de inércia e evitando oscilações em regiões mal condicionadas.
\end{enumerate}

Em termos conceituais, a iteração acelerada quasi-Newton pode ser vista como um sistema de duas camadas: a camada interna, representada pela transformação $\Phi_{\text{BFGS}}$, assegura a coerência geométrica no cone das SPD; a camada externa, definida pelas atualizações de $Y_k$ e $V_k$, reproduz o comportamento inercial do método de Nesterov em um formato totalmente discreto e compatível com o domínio matricial. O resultado é uma formulação iterativa que combina a adaptabilidade dos métodos quasi-Newton com uma dinâmica de aceleração controlada, dispensando a necessidade de análise contínua ou de parâmetros derivados de sistemas diferenciais.

\subsection{Análise iterativa e preservação de propriedades estruturais}
\label{subsec:analise_iterativa}

Para fundamentar as propriedades estruturais e de estabilidade do esquema iterativo descrito acima, são apresentados a seguir alguns resultados auxiliares. Esses resultados estabelecem condições suficientes para a preservação da positividade definida e para o decréscimo monótono de um funcional de Lyapunov, $\mathcal{E}_k$, associado às sequências $\{X_k,V_k,x_k\}$.

\begin{lemma}%[Convexidade de $\mathbb{S}_{++}^n$ e herança de cotas espectrais]
\label{lem:convex_spd_bounds}
Se $X_k,V_k\in\mathbb{S}_{++}^n$ satisfazem $mI\preceq X_k,V_k\preceq MI$ para algum $0<m\le M$, então, para todo $\rho\in(0,1)$,
$$
Y:=(1-\rho)X_k+\rho V_k\in\mathbb{S}_{++}^n
\quad\text{e}\quad
mI\preceq Y\preceq MI.
$$
\begin{proof} Para todo $z\neq 0$, $$z^\top Y_k z=(1-\rho)z^\top X_k z+\rho z^\top V_k z>0$$
Além disso, $$\lambda_{\min}(Y_k)\ge (1-\rho)\lambda_{\min}(X_k)+\rho\lambda_{\min}(V_k)\ge m$$ e 
$$\lambda_{\max}(Y_k)\le (1-\rho)\lambda_{\max}(X_k)+\rho\lambda_{\max}(V_k)\le M$$ 
\end{proof}
\end{lemma}

Um argumento inteiramente análogo pode ser aplicado à variável auxiliar $V_k$, cuja atualização iterativa é dada por uma média convexa entre duas matrizes simétricas definidas positivas. De fato, se $V_k, X_{k+1} \in \mathbb{S}_{++}^n$ satisfazem $mI \preceq (\cdot) \preceq MI$ para algum $0 < m \le M$, então, para qualquer $\beta \in (0,1)$,
$$
V_{k+1} = (1-\beta)V_k + \beta X_{k+1} \in \mathbb{S}_{++}^n,
\qquad
mI \preceq V_{k+1} \preceq MI.
$$
Logo, tanto $Y_k$ quanto $V_{k+1}$ preservam a positividade definida por construção, assegurando que todas as variáveis matriciais do método permaneçam no cone $\mathbb{S}_{++}^n$ ao longo das iterações.
A garantia de que as variáveis intermediárias $Y_k$ e $V_k$ permanecem no cone $\mathbb{S}_{++}^n$ é essencial para que a etapa quasi-Newton subsequente preserve a estrutura definida positiva da matriz de curvatura. Uma vez assegurada essa propriedade de convexidade matricial, pode-se aplicar a atualização clássica de BFGS sobre $Y_k$, conforme estabelecido no Lema \ref{lem:bfgs_spd}. Tal resultado demonstra que, sob a condição de curvatura $s_k^\top \zeta_k > 0$, a transformação de BFGS mantém a positividade definida da nova matriz $X_{k+1}$, completando assim o ciclo de estabilidade estrutural entre as etapas de extrapolação e de atualização quasi-Newton.

\begin{lemma}%[Preservação de SPD pelo BFGS]
\label{lem:bfgs_spd}
Considere $Y_k\in\mathbb{S}_{++}^n$ e vetores $s,\zeta\in\mathbb{R}^n$ tais que $\zeta^\top s>0$. 
A atualização BFGS clássica
$$
X_{k+1}
= \Big(I-\tfrac{s \zeta^\top}{\zeta^\top s}\Big)\,Y_k\,\Big(I-\tfrac{\zeta s^\top}{\zeta^\top s}\Big)
  + \tfrac{s s^\top}{\zeta^\top s}
$$
satisfaz $X_{k+1}\in\mathbb{S}_{++}^n$. 
\begin{proof}
Seja $Y_k\in\mathbb{S}_{++}^n$ e $s,\zeta\in\mathbb{R}^n$ com $\zeta^\top s>0$. 
Defina
$$
\phi := \frac{1}{\zeta^\top s} \;>\; 0
\qquad\text{e}\qquad
M := I - \phi\,\zeta s^\top .
$$
Note que $M^\top = I - \phi\, s\zeta^\top$. A atualização BFGS-inversa pode ser escrita como
$$
X_{k+1}
= \big(I-\phi\, s\zeta^\top\big)\,Y_k\,\big(I-\phi\,\zeta s^\top\big)
  + \phi\,ss^\top
= M^\top Y_k M + \phi\,ss^\top .
$$
Para qualquer $z\neq 0$,
$$
z^\top X_{k+1} z
= (Mz)^\top Y_k (Mz) \;+\; \phi\,(s^\top z)^2 .
$$
Como $Y\succ 0$, temos $(Mz)^\top Y_k (Mz) > 0$ sempre que $Mz\neq 0$. Portanto, 
no caso $Mz\neq 0$ já concluímos $z^\top X_{k+1} z>0$.

Resta analisar o caso $Mz=0$. Da definição de $M$,
$$
Mz=0 \;\;\Longleftrightarrow\;\; z - \phi\,\zeta (s^\top z)=0 
\;\;\Longleftrightarrow\;\; z = \phi\,\zeta (s^\top z).
$$
Como $z\neq 0$ e $\phi>0$, segue que $s^\top z \neq 0$. Logo, o segundo termo acima satisfaz
$$
\phi\,(s^\top z)^2 \;>\; 0,
$$
o que implica novamente $z^\top X_{k+1} z>0$. Em ambas as situações, para todo $z\neq 0$,
temos $z^\top X_{k+1} z>0$, isto é, $X_{k+1}\in\mathbb{S}_{++}^n$.
Além disso, a simetria de $X_{k+1}$ decorre do fato de que $Y_k$ é simétrica e as operações
utilizadas preservam simetria.
\end{proof}

\end{lemma}

Com base nos resultados acima, é possível conduzir a análise de estabilidade do esquema completo, considerando de forma conjunta a evolução das variáveis $x_k$ e das aproximações da Hessiana. O Teorema \ref{thm:Lyapunov} formaliza esse resultado, mostrando que, sob hipóteses de suavidade e passos $\eta_k$ suficientemente pequenos, existe uma função de Lyapunov $\mathcal{E}_k$ que decresce monotonamente ao longo das iterações. Essa função combina o valor da função objetivo com um termo de coerência entre as matrizes $X_k$ e $V_k$, refletindo tanto o progresso do método quanto a estabilidade das aproximações obtidas. 

Além disso, na demonstração do teorema verifica-se que essa propriedade de
decréscimo exige apenas que os parâmetros de aceleração $\rho$ e $\beta$
pertencentes ao intervalo $(0,1)$ sejam escolhidos dentro de uma faixa
compatível com as desigualdades envolvidas. Em particular, valores
moderados desses parâmetros garantem que os termos inerciais sejam
suficientemente amortecidos, assegurando que a dinâmica acoplada entre
$X_k$ e $V_k$ permaneça estável. Dessa forma, o teorema sintetiza não
apenas as propriedades de preservação estrutural e estabilidade numérica
do método, mas também estabelece condições explícitas sobre os parâmetros
de aceleração que asseguram a consistência do BFGS acelerado proposto.
\begin{theorem}%[Decrescimento tipo-Lyapunov para o esquema acelerado quasi-Newton]
\label{thm:Lyapunov}
Considere $f:\mathbb{R}^n\to\mathbb{R}$ de classe $C^1$ com gradiente 
$L$-Lipschitz em uma região compacta que contém a sequência iterativa.
Seja o esquema definido por
\begin{align*}
x_{k+1} &= x_k - \eta_k X_k \nabla f(x_k),\\[0.1cm]
Y_k &= (1-\rho)X_k + \rho V_k,\qquad \rho\in(0,\rho_{\max}),\\[0.1cm]
X_{k+1} &= \Phi_{\mathrm{BFGS}}(Y_k;\, s_k,\zeta_k),\quad
s_k := x_{k+1}-x_k,\quad 
\zeta_k := \nabla f(x_{k+1})-\nabla f(x_k),\\[0.1cm]
V_{k+1} &= (1-\beta)V_k + \beta X_{k+1},\qquad \beta\in(\beta_{\min},1),
\end{align*}
com inicialização $X_0 = V_0 = I$.

Suponha que $s_k^\top \zeta_k > 0$ para todo $k$ (o que garante que 
$X_{k+1}\in S_{++}^n$) e que existem constantes $0 < m_* \le M_* < \infty$ tais que
\[
m_* I \preceq X_k,\,V_k,\,Y_k \preceq M_* I,\qquad\text{para todo }k.
\]

Assuma ainda que os passos $\eta_k$ satisfazem uma condição de 
decréscimo suficiente, isto é, existe $c_1>0$ tal que
\begin{equation}\label{eq:suf-descent}
f(x_{k+1}) \le f(x_k) - c_1\|\nabla f(x_k)\|^2 ,
\end{equation}
como obtido, por exemplo, por uma busca de linha do tipo Armijo.

Defina, para $\kappa>0$,
\[
\mathcal{E}_k := f(x_k)-f^* + \kappa\|X_k - V_k\|_F^2 .
\]

Então, existem $\kappa^*>0$ e uma constante $c_2>0$
(dependentes apenas de $m_*,M_*,L,\rho_{\max},\beta_{\min}$)
tais que, para qualquer $\kappa\in(0,\kappa^*)$ e para todo $k$,
\begin{equation}\label{eq:lyapunov-descent}
\mathcal{E}_{k+1}
\;\le\; 
\mathcal{E}_k
\;-\;
c_1\|\nabla f(x_k)\|^2
\;-\;
c_2\|X_{k+1}-V_k\|_F^2 .
\end{equation}

Em particular, a sequência $\{\mathcal{E}_k\}$ é não crescente,
o que garante estabilidade discreta no sentido de Lyapunov e assegura
que $\|X_k - V_k\|_F \to 0$ ao longo das iterações.
\end{theorem}

\begin{proof}
Defina, para $\kappa>0$, a função de Lyapunov
\[
\mathcal{E}_k \;:=\; f(x_k)-f^* \;+\; \kappa\|X_k - V_k\|_F^2.
\]
Nosso objetivo é mostrar que, para escolhas apropriadas de
$\rho\in(0,\rho_{\max})$, $\beta\in(\beta_{\min},1)$ e $\kappa>0$
suficientemente pequeno, existem constantes $c_1,c_2>0$ tais que
\begin{equation}\label{eq:Lyap-target}
\mathcal{E}_{k+1}
\;\le\;
\mathcal{E}_k
-
c_1\|\nabla f(x_k)\|^2
-
c_2\|X_{k+1}-V_k\|_F^2
\qquad\text{para todo }k.
\end{equation}

\medskip
\noindent\textbf{Passo 1: Decomposição da variação de $\mathcal{E}_k$.}
Pela definição de $\mathcal{E}_k$,
\[
\mathcal{E}_{k+1}-\mathcal{E}_k
=
\underbrace{f(x_{k+1})-f(x_k)}_{\text{termo I}}
+
\kappa\underbrace{\Big(\|X_{k+1}-V_{k+1}\|_F^2-\|X_k-V_k\|_F^2\Big)}_{\text{termo II}}.
\]
 Pelo $L$-Lipschitz do gradiente,
$$
f(x_{k+1}) \le f(x_k) - \eta_k \nabla f(x_k)^\top X_k \nabla f(x_k) + \tfrac{L}{2}\eta_k^2 \|X_k\nabla f(x_k)\|^2.
$$
Usando $m_\ast I\preceq X_k\preceq M_\ast I$ obtém-se
$$
f(x_{k+1}) \le f(x_k) - c_1 \|\nabla f(x_k)\|^2
$$
com $c_1=\eta_k m_\ast - \tfrac{L}{2}\eta_k^2 M_\ast^2>0$ quando $\eta_k\le 1/(M_\ast L)$, o que coincide com \eqref{eq:suf-descent}.

Resta, portanto, controlar o termo II
\[
\Delta_k^{\mathrm{mat}}
:=
\|X_{k+1}-V_{k+1}\|_F^2-\|X_k-V_k\|_F^2.
\]

\medskip
\noindent\textbf{Passo 2: Reescrita do termo II.}
Da definição de $V_{k+1}$,
\[
V_{k+1} = (1-\beta)V_k + \beta X_{k+1},
\]
deduzimos
\[
X_{k+1}-V_{k+1}
=
X_{k+1} - \big((1-\beta)V_k+\beta X_{k+1}\big)
=
(1-\beta)(X_{k+1}-V_k),
\]
de modo que
\[
\|X_{k+1}-V_{k+1}\|_F^2
=
(1-\beta)^2\|X_{k+1}-V_k\|_F^2.
\]
Logo,
\begin{equation}\label{eq:Delta-mat-0}
\Delta_k^{\mathrm{mat}}
=
(1-\beta)^2\|X_{k+1}-V_k\|_F^2 - \|X_k-V_k\|_F^2.
\end{equation}

\medskip
\noindent\textbf{Passo 3: Desigualdade de Young matricial com parâmetros $\theta$ e $\varepsilon$.}
Sejam $\theta,\varepsilon\in(0,1)$ a serem fixados adiante. Escrevemos
\[
-\|X_k-V_k\|_F^2
=
-\theta\|X_k-V_k\|_F^2
-
(1-\theta)\|X_k-V_k\|_F^2.
\]
Aplicamos, então, a desigualdade de Young matricial na forma
\[
\|A\|_F^2
\ge
(1-\varepsilon)\|B\|_F^2
-
\Big(\tfrac{1}{\varepsilon}-1\Big)\|A-B\|_F^2,
\]
válida para quaisquer $A,B\in\mathbb{R}^{n\times n}$ e $\varepsilon\in(0,1)$.
Tomando $A:=X_k-V_k$ e $B:=X_{k+1}-V_k$, obtemos
\[
-\,(1-\theta)\|X_k-V_k\|_F^2
\;\le\;
-(1-\theta)(1-\varepsilon)\|X_{k+1}-V_k\|_F^2
+
(1-\theta)\Big(\tfrac{1}{\varepsilon}-1\Big)\|X_{k+1}-X_k\|_F^2.
\]
Substituindo na expressão de $\Delta_k^{\mathrm{mat}}$ em
\eqref{eq:Delta-mat-0}, resulta
\begin{align}
\Delta_k^{\mathrm{mat}}
&\le
(1-\beta)^2\|X_{k+1}-V_k\|_F^2
-\theta\|X_k-V_k\|_F^2 \nonumber\\
&\quad
-(1-\theta)(1-\varepsilon)\|X_{k+1}-V_k\|_F^2
+
(1-\theta)\Big(\tfrac{1}{\varepsilon}-1\Big)\|X_{k+1}-X_k\|_F^2
\nonumber\\[0.1cm]
&=
\underbrace{\Big((1-\beta)^2-(1-\theta)(1-\varepsilon)\Big)}_{=:~\Gamma_1}\,
\|X_{k+1}-V_k\|_F^2
-
\theta\|X_k-V_k\|_F^2
\nonumber\\
&\quad
+
\underbrace{(1-\theta)\Big(\tfrac{1}{\varepsilon}-1\Big)}_{=:~\Gamma_0}\,
\|X_{k+1}-X_k\|_F^2.\label{eq:Delta-mat-1}
\end{align}

\medskip
\noindent\textbf{Passo 4: Cota de $\|X_{k+1}-X_k\|_F^2$.}
Pelo Lema quasi-Newton (baseado na forma de BFGS sobre $Y_k$) e pelas
cotas espectrais $m_*I\preceq X_k,V_k,Y_k\preceq M_*I$, existe uma
constante $A>0$ (dependente apenas de $m_*,M_*,L$) tal que
\begin{equation}\label{eq:bound-Xdiff-1}
\|X_{k+1}-Y_k\|_F
\;\le\;
A\,\|s_k\|\,\|\zeta_k\|.
\end{equation}
Como $s_k = x_{k+1}-x_k = -\eta_k X_k\nabla f(x_k)$, segue que
\[
\|s_k\|
\le
\eta_k\|X_k\|\,\|\nabla f(x_k)\|
\le
\eta_k M_* \|\nabla f(x_k)\|.
\]
Por Lipschitz-continuidade do gradiente,
$\|\zeta_k\|=\|\nabla f(x_{k+1})-\nabla f(x_k)\|\le L\|s_k\|$, o que implica
\[
\|\zeta_k\|
\le L\|s_k\|
\le L\eta_k M_*\|\nabla f(x_k)\|.
\]
Substituindo em \eqref{eq:bound-Xdiff-1}, obtemos
\[
\|X_{k+1}-Y_k\|_F
\le
A\,\|s_k\|\,\|\zeta_k\|
\le
AL M_*^2 \eta_k^2 \|\nabla f(x_k)\|^2.
\]
Consequentemente, existe $A_1>0$ tal que
\begin{equation}\label{eq:bound-Xdiff-2}
\|X_{k+1}-Y_k\|_F^2
\;\le\;
A_1\,\eta_k^4\,\|\nabla f(x_k)\|^4.
\end{equation}

Além disso, como $Y_k = (1-\rho)X_k + \rho V_k$, obtemos $Y_k-X_k=\rho(V_k-X_k)$. Deste fato e da desilgualdade triangular em $X_{k+1}-X_k=X_{k+1}-Y_k+Y_k-X_k$, temos
\begin{equation}\label{eq:bound-Xdiff-3}
\|X_{k+1}-X_k\|_F
\;\le\;
\|X_{k+1}-Y_k\|_F+\rho\|X_{k}-V_k\|_F
\end{equation}
 e então, de \eqref{eq:bound-Xdiff-2} e da desigualdade de Cauchy-Schwarz (caso especial), concluímos que  

\begin{equation}\label{eq:bound-Xdiff-4}
\|X_{k+1}-X_k\|_F^2
\;\le\;
2A_1\,\eta_k^4\,\|\nabla f(x_k)\|^4
+
2\,\rho^2\,\|X_k-V_k\|_F^2.
\end{equation}


\medskip
\noindent\textbf{Passo 5: Substituição em $\Delta_k^{\mathrm{mat}}$ e escolha de $\beta_{\min}$ e $\rho_{\max}$.}
Substituindo a estimativa \eqref{eq:bound-Xdiff-4} em \eqref{eq:Delta-mat-1}, obtemos
\begin{align}
\Delta_k^{\mathrm{mat}}
&\le
\Gamma_1\,\|X_{k+1}-V_k\|_F^2
-
\theta\|X_k-V_k\|_F^2
+
\Gamma_0\Big(2A_1\eta_k^4\|\nabla f(x_k)\|^4 + 2\rho^2\|X_k-V_k\|_F^2\Big)
\nonumber\\[0.1cm]
&=
\Gamma_1\,\|X_{k+1}-V_k\|_F^2
+
\underbrace{\big(-\theta + 2\Gamma_0 \rho^2\big)}_{=:~\Gamma_2}\,
\|X_k-V_k\|_F^2
+
2\Gamma_0 A_1\eta_k^4\|\nabla f(x_k)\|^4.
\label{eq:Delta-mat-2}
\end{align}

Para controlar simultaneamente os coeficientes $\Gamma_1$ e $\Gamma_2$,
impomos, sem perda de generalidade, a relação $\theta+\varepsilon=1$.
Sob essa escolha, a validade da desigualdade de Lyapunov
\eqref{eq:lyapunov-descent} reduz-se a garantir que
\[
\Gamma_1 < 0
\qquad\text{e}\qquad
\Gamma_2 < 0.
\]

\medskip
\noindent\textbf{Escolha de $\beta_{\min}$.}
A expressão de $\Gamma_1$ no caso $\theta+\varepsilon=1$ torna-se
\[
\Gamma_1 = (1-\beta)^2 - (1-\theta)(1-\varepsilon)
           = (1-\beta)^2 - \theta(1-\theta).
\]
A função $\theta(1-\theta)$ atinge seu máximo no ponto $\theta=\tfrac{1}{2}$,
com valor $1/4$. Assim,
\[
\Gamma_1 < 0
\quad\Longleftrightarrow\quad
(1-\beta)^2 < \tfrac14
\quad\Longleftrightarrow\quad
\beta > \tfrac12.
\]
Portanto, qualquer parâmetro
\[
\beta \in (\beta_{\min},1),
\qquad
\beta_{\min} := \tfrac12,
\]
garante a existência de uma constante $\gamma_1>0$ tal que
\begin{equation}\label{eq:Gamma1-neg}
\Gamma_1 \le -\gamma_1 < 0.
\end{equation}

\medskip
\noindent\textbf{Escolha de $\rho_{\max}$.}
Pela definição de $\Gamma_0$ em \eqref{eq:Delta-mat-1}, e usando
$\theta+\varepsilon=1$, obtemos $\Gamma_0=\theta$. Assim,
\[
\Gamma_2 = -\theta + 2\theta\rho^2
          = \theta(2\rho^2 - 1).
\]
A condição $\Gamma_2<0$ equivale a
\[
2\rho^2 - 1 < 0
\quad\Longleftrightarrow\quad
\rho < \frac{1}{\sqrt{2}}.
\]
Logo, para qualquer
\[
\rho \in (0,\rho_{\max}),
\qquad
\rho_{\max}:=\frac{1}{\sqrt{2}},
\]
existe uma constante $\gamma_2>0$ tal que
\begin{equation}\label{eq:Gamma2-neg}
\Gamma_2 \le -\gamma_2 < 0.
\end{equation}

\medskip
Concluímos, portanto, que a análise de Lyapunov exige parâmetros de aceleração
restritos às faixas
\[
\beta \in (\beta_{\min},1),
\qquad
\rho \in (0,\rho_{\max}),
\]
com $\beta_{\min}=\tfrac12$ e
$\rho_{\max} = \tfrac{1}{\sqrt{2}}$, assegurando que tanto
$\Gamma_1$ quanto $\Gamma_2$ contribuam com termos dissipativos na
desigualdade de decréscimo \eqref{eq:lyapunov-descent}.

\medskip
\noindent\textbf{Passo 6: Combinação dos termos e escolha de $\kappa^*$.}
Com \eqref{eq:Gamma1-neg} e \eqref{eq:Gamma2-neg}, a desigualdade
\eqref{eq:Delta-mat-2} implica que, para $\rho\in(0,\rho_{\max})$ e
$\beta\in(\beta_{\min},1)$,
\[
\Delta_k^{\mathrm{mat}}
\le
-\gamma_1\|X_{k+1}-V_k\|_F^2
-\gamma_2\|X_k-V_k\|_F^2
+
2\Gamma_0 A_1\eta_k^4\|\nabla f(x_k)\|^4.
\]
Multiplicando por $\kappa>0$ e somando a \eqref{eq:suf-descent}, obtemos
\begin{align}
\mathcal{E}_{k+1}-\mathcal{E}_k
&\le
-c_1\|\nabla f(x_k)\|^2
-\kappa\gamma_1\|X_{k+1}-V_k\|_F^2
-\kappa\gamma_2\|X_k-V_k\|_F^2
+
2\kappa \Gamma_0 A_1\eta_k^4\|\nabla f(x_k)\|^4.
\label{eq:Delta-Ek-pre}
\end{align}

Como a sequência $(x_k)$ permanece em uma região compacta e o gradiente
é Lipschitz-contínuo, existe $G_*>0$ tal que
$\|\nabla f(x_k)\|\le G_*$ para todo $k$. Além disso, a busca linear
garante que $\eta_k\le\eta_{\max}$. Assim,
\[
\eta_k^4\|\nabla f(x_k)\|^4
\le
\eta_{\max}^4 G_*^2\,\|\nabla f(x_k)\|^2.
\]
Definindo
\[
C_* := 2\Gamma_0 A_1 \eta_{\max}^4 G_*^2,
\]
segue que
\[
2\kappa \Gamma_0 A_1\eta_k^4\|\nabla f(x_k)\|^4
\le
\kappa C_* \|\nabla f(x_k)\|^2.
\]

Escolhemos, então, $\kappa>0$ suficientemente pequeno para que
\[
\kappa C_* \le \frac{c_1}{2}.
\]
Note que tal escolha sempre existe, e definimos
\[
\kappa^* := \frac{c_1}{2C_*},
\]
de modo que a condição acima é satisfeita para qualquer
$\kappa\in(0,\kappa^*)$.

Sob essa escolha, a desigualdade \eqref{eq:Delta-Ek-pre} reduz-se a
\begin{equation}\label{eq:Delta-Ek-final}
\mathcal{E}_{k+1}-\mathcal{E}_k
\;\le\;
-\frac{c_1}{2}\|\nabla f(x_k)\|^2
-\kappa\gamma_1\|X_{k+1}-V_k\|_F^2.
\end{equation}
Definindo $c_2 := \kappa\gamma_1>0$, obtemos exatamente a forma
\eqref{eq:Lyap-target} com $c_1$ substituído por $c_1/2$, o que não
altera a natureza do resultado.

Em particular, $\{\mathcal{E}_k\}$ é não crescente para qualquer
$\kappa\in(0,\kappa^*)$, o que garante estabilidade no sentido de
Lyapunov e implica que $\|X_k - V_k\|_F \to 0$ ao longo das iterações.

\end{proof}

\noindent\textbf{Interpretação do resultado.}
O Teorema~\ref{thm:Lyapunov} estabelece uma forma discreta de estabilidade
para o esquema acelerado quasi-Newton. A desigualdade
\eqref{eq:lyapunov-descent} garante que a sequência
$(\mathcal{E}_k)_{k\ge0}$ é não crescente, de modo que o método mantém um
regime de decréscimo controlado ao longo de toda a iteração. Esse controle
atua simultaneamente sobre a variável $x_k$ e sobre as aproximações
matriciais $X_k$ e $V_k$, assegurando que a aceleração não introduz
oscilações que comprometam a coerência entre as atualizações quasi-Newton.

O termo $\|X_{k+1}-V_k\|_F^2$, que aparece com coeficiente negativo em
\eqref{eq:lyapunov-descent}, mede o desvio entre a matriz produzida pela
atualização quasi-Newton e a matriz inercial acumulada pelo esquema
acelerado. O fato de esse termo surgir com peso dissipativo implica que as
iterações tendem a aproximar progressivamente essas duas sequências,
reduzindo gradualmente a diferença entre elas. Em particular, o método força
$X_k$ e $V_k$ a permanecerem próximos ao longo de toda a dinâmica,
convergindo para o regime no qual $X_k\simeq V_k$.

Do ponto de vista analítico, a existência de $\kappa^*>0$ assegura que é
possível escolher $\kappa$ pequeno o suficiente para que a parte quadrática
de ordem superior (decorrente dos termos $\eta_k^4\|\nabla f(x_k)\|^4$)
seja absorvida pelo decrescimento de $f(x_k)$. Isso gera uma
interação consistentemente amortecida entre a evolução escalar
$f(x_k)$ e a evolução matricial $(X_k,V_k)$, evitando a amplificação de
oscilações provocadas pelos termos de inércia. Além disso, as restrições
$\beta>\beta_{\min}$ e $\rho<\rho_{\max}$ — determinadas explicitamente na
demonstração — garantem que os coeficientes $\Gamma_1$ e $\Gamma_2$ sejam
negativos, assegurando que tanto o desvio $X_{k+1}-V_k$ quanto o desvio
$X_k-V_k$ contribuam para o decaimento de $\mathcal{E}_k$.

Consequentemente, a atualização acelerada preserva a positividade definida
das matrizes, mantém as cotas espectrais uniformes
$m_\ast I\preceq X_k,V_k\preceq M_\ast I$ e produz uma sequência
$(x_k,X_k,V_k)$ estável no sentido de Lyapunov, isto é, confinada em uma
região compacta e aproximando monotonicamente a configuração de equilíbrio
caracterizada por $\nabla f(x_k)\to 0$ e $X_k\simeq V_k$.

Em termos práticos, o teorema mostra que o termo de aceleração não compromete
a estabilidade do processo quasi-Newton, desde que os parâmetros de
aceleração satisfaçam $\beta\in(\beta_{\min},1)$ e $\rho\in(0,\rho_{\max})$.
Dentro dessas faixas, a interação entre $X_k$ e $V_k$ permanece
controlada e a dinâmica converge para um regime estacionário no qual as
matrizes sucessivas tornam-se praticamente indistinguíveis. Esse resultado é
essencial para garantir que o método acelerado preserve as propriedades
estruturais do BFGS e mantenha coerência geométrica no cone
$\mathbb{S}_{++}^n$ ao longo de toda a iteração.

\subsection{Componente Estocástico na Direção de Busca}
\label{sec:stochastic_bfgs}

A formulação estocástica proposta neste trabalho introduz aleatoriedade controlada diretamente na direção de busca gerada pelo método quasi-Newton. Diferentemente de abordagens que aplicam estocasticidade no cálculo ou na atualização da matriz Hessiana, aqui o ruído é incorporado ao vetor de deslocamento, preservando a estrutura determinística da atualização de $X_k$ e mantendo as propriedades locais de convergência associadas ao esquema BFGS.

A introdução desse componente estocástico tem como principal motivação ampliar a capacidade exploratória do método e reduzir a probabilidade de estagnação em mínimos locais ou regiões de curvatura degenerada. Métodos puramente determinísticos, embora eficientes em regiões convexas, tendem a apresentar comportamento \emph{guloso}, avançando sempre na direção de maior descida local e, por consequência, podem convergir prematuramente em superfícies multimodais. A incorporação de uma perturbação aleatória controlada atua como um mecanismo de escape dessas regiões, permitindo que o algoritmo explore o espaço de busca de forma mais ampla sem comprometer sua estabilidade assintótica. Assim como o termo de inércia introduzido na atualização da inversa da Hessiana, a estocasticidade aqui atua como um mecanismo adicional de regularização dinâmica, ampliando a robustez global do método.

Essa estratégia baseia-se em estudos recentes sobre a robustez de métodos quasi-Newton sob ruído e incerteza [\cite{shi2022noise, guo2023overview, amos2020algorithm, peng2025finding}], os quais demonstram que perturbações probabilísticas moderadas podem melhorar o comportamento global de busca sem degradar o desempenho local. Inspirando-se nesses resultados, o ruído é introduzido de modo a preservar a natureza descendente da direção de busca, evitando que a perturbação anule o efeito do gradiente. Para isso, em cada iteração é gerado um vetor aleatório $\epsilon \sim \mathcal{N}(0, I)$ no espaço $\mathbb{R}^n$, o qual é então projetado de forma a eliminar a componente paralela ao gradiente atual $g_k = \nabla f(x_k)$. Define-se, assim,
\begin{equation}
\xi_k = \epsilon - \frac{\epsilon^\top g_k}{g_k^\top g_k} \, g_k,
\label{eq:projected_noise}
\end{equation}
de modo que $\xi_k$ é aproximadamente ortogonal ao gradiente. Essa projeção garante que a perturbação não introduza um movimento que aumente o valor da função objetivo, mantendo a coerência direcional com o processo de descida.

A magnitude do ruído projetado é controlada por um fator de temperatura $\tau_k > 0$, que decai suavemente ao longo das iterações. Esse parâmetro atua como um fator de escala da variância do ruído, modulando a intensidade das perturbações introduzidas em cada iteração. Valores iniciais elevados de $\tau_k$ permitem maior dispersão direcional, favorecendo a exploração global do espaço de busca, enquanto o seu decaimento progressivo reduz gradualmente a variabilidade, conduzindo o método a uma fase de refinamento local. Essa estratégia segue um princípio análogo ao do \emph{simulated annealing}, em que a temperatura é reduzida de forma controlada para garantir convergência estável em regiões de menor energia [~\cite{shi2022noise, amos2020algorithm, peng2025finding}]. Estudos recentes sobre métodos quasi-Newton robustos ao ruído mostram que a redução progressiva da temperatura pode ser interpretada como um mecanismo de \emph{cooling}, garantindo que a variância do termo estocástico tenda a zero em probabilidade, preservando as propriedades assintóticas do método determinístico [\cite{guo2023overview}]. Um esquema simples e eficaz para esse controle é dado por
\begin{equation}
\tau_k = \frac{\tau_0}{1 + \lambda k}, \qquad \lambda > 0,
\label{eq:temperature_decay}
\end{equation}
onde $\tau_0 > 0$ define a intensidade inicial da perturbação e $\lambda$ controla o ritmo de decaimento. Assim, o ruído tem maior impacto nas iterações iniciais, promovendo exploração e diversidade direcional, e decai progressivamente à medida que o método se aproxima de regiões estacionárias, assegurando convergência estável.



A nova direção de busca, denotada aqui por $\tilde{s}_k$ para manter consistência com a notação quasi-Newton, passa a ser dada por
\begin{equation}
\tilde{s}_k = s_k + \tau_k \xi_k,
\label{eq:stochastic_direction_projected}
\end{equation}
em que $s_k = -X_k \nabla f(x_k)$ representa a direção determinística obtida pelo BFGS acelerado.
A ortogonalização do ruído em~\eqref{eq:projected_noise} garante, portanto, que o termo estocástico não interfira na componente de descida. De fato, como $g_k^\top \xi_k = 0$, tem-se
\[
g_k^\top \tilde{s}_k = g_k^\top (s_k + \tau_k \xi_k) = g_k^\top s_k,
\]
preservando-se assim a condição de direção de descida do método. Essa propriedade assegura que a inclusão do ruído projetado não compromete o critério de coerência direcional, mantendo o comportamento local equivalente ao do esquema determinístico.


O novo ponto iterado é então atualizado por
\[
x_{k+1} = x_k + \eta_k \tilde{s}_k,
\]
com $\eta_k > 0$ determinado por uma busca linear adequada. Nesta formulação, o vetor $s_k$ representa a direção de busca (antes da aplicação do passo $\eta_k$), enquanto o deslocamento total é dado por $x_{k+1} - x_k = \eta_k \tilde{s}_k$. 

A adição do termo $\tau_k \xi_k$ introduz pequenas variações direcionais ortogonais ao gradiente, de modo que o vetor de busca resultante oscila em torno da direção determinística $s_k$. Em termos estatísticos, pode-se mostrar que o ruído projetado possui média nula, o que implica que o deslocamento médio não se altera. De fato, como $\epsilon \sim \mathcal{N}(0,I)$ tem média zero, tem-se $\mathbb{E}[\epsilon] = 0$. A projeção em~\eqref{eq:projected_noise} é uma transformação linear de $\epsilon$, dada por
\[
\xi_k = (I - P_k)\epsilon, \qquad P_k = \frac{g_k g_k^\top}{g_k^\top g_k},
\]
de modo que
\[
\mathbb{E}[\xi_k] = (I - P_k)\mathbb{E}[\epsilon] = (I - P_k) \cdot 0 = 0.
\]
Consequentemente, o ruído projetado é centrado, isto é, não apresenta tendência média em nenhuma direção específica do espaço de busca. Assim, para a direção estocástica definida em~\eqref{eq:stochastic_direction_projected},
\[
\tilde{s}_k = s_k + \tau_k \xi_k,
\]
obtém-se
\[
\mathbb{E}[\tilde{s}_k] = s_k + \tau_k \mathbb{E}[\xi_k] = s_k,
\]
o que demonstra que o deslocamento esperado coincide com o do método determinístico. Em outras palavras, as perturbações introduzidas por $\xi_k$ produzem oscilações locais em torno de $s_k$, mas não modificam o sentido médio de descida. À medida que $\tau_k \to 0$, essas flutuações tornam-se progressivamente desprezíveis, assegurando que a dinâmica assintótica do algoritmo convirja para a de um método quasi-Newton padrão, levando a um ponto estacionário de $f$ sob hipóteses usuais de suavidade e convexidade local.

Do ponto de vista geométrico, essa perturbação projetada atua tangencialmente às superfícies de nível da função objetivo, promovendo pequenas variações em torno da trajetória de descida. Esse comportamento aumenta a diversidade direcional e permite que o algoritmo escape de vales estreitos ou planícies de baixa curvatura, sem comprometer o sentido global de descida. Em problemas multimodais, a presença desse termo é particularmente vantajosa, pois reduz a probabilidade de aprisionamento em mínimos locais e favorece uma busca mais abrangente em torno das regiões de interesse.

Em termos práticos, a calibração de $\tau_0$ é determinante para o equilíbrio entre exploração e estabilidade: valores excessivos podem provocar oscilações, enquanto valores muito baixos anulam o benefício do componente estocástico. Recomenda-se escolher $\tau_0$ em proporção à norma média dos gradientes nas primeiras iterações, garantindo perturbações compatíveis com a escala do problema. Essa escolha, combinada com o decaimento definido em~\eqref{eq:temperature_decay}, permite ao método transitar de uma fase inicial exploratória para um regime de refinamento determinístico, mantendo as propriedades quasi-Newton e a eficiência de convergência do BFGS acelerado.

Em síntese, o método proposto preserva o núcleo determinístico do BFGS acelerado, mas introduz um ruído projetado e suavemente decrescente na direção de busca. Essa modificação confere ao algoritmo maior capacidade exploratória, robustez frente a irregularidades da superfície de otimização e estabilidade teórica, constituindo uma extensão natural e eficiente do esquema quasi-Newton para cenários ruidosos ou não convexos.  

A seguir, apresenta-se o algoritmo correspondente à formulação proposta.
A estrutura geral segue o esquema quasi-Newton com atualização da inversa
da Hessiana, incorporando a aceleração matricial controlada pelos
parâmetros $\rho<\rho_{\max}$ e $\beta>\beta_{\min}$, conforme estabelecido
na análise de estabilidade. A componente estocástica é adicionada na
direção de busca, através de uma perturbação $\xi_k$ ortogonal ao gradiente
e escalada por um fator de temperatura $\tau_k$ que decai segundo
\eqref{eq:temperature_decay}. O parâmetro $\rho$ controla a mistura entre a
matriz corrente $H_k$ e a memória suavizada $U_k$, enquanto $\beta$ regula a
taxa de atualização dessa memória. O algoritmo utiliza uma busca linear do
tipo Armijo para garantir a condição de descida em cada iteração.

\begin{algorithm}[H]
\caption{BFGS Acelerado com Componente Estocástico na Direção de Busca}
\label{alg:bfgs_ac_stoc}
\begin{algorithmic}[1]
\REQUIRE $x_0$, $H_0 = I$, $U_0 = I$, $\tau_0$, $\lambda$, $\rho$, $\beta$, $\eta$, $\sigma$
\STATE \textbf{Avaliar} $f(x_0)$ e $g_0 = \nabla f(x_0)$
\FOR{$k = 0,1,2,\dots$ \textbf{até convergência}}
    \STATE $d_k \gets -H_k g_k$ \COMMENT{Direção determinística de descida}
    \STATE \textbf{Gerar} ruído $\varepsilon \sim \mathcal{N}(0,I)$
    \STATE \textbf{Projetar} $\varepsilon$ ortogonalmente ao gradiente:
        \[
        \xi_k = \varepsilon - \frac{\varepsilon^\top g_k}{g_k^\top g_k}\, g_k
        \]
    \STATE \textbf{Calcular temperatura}: $\tau_k = \tau_0 / (1 + \lambda k)$
    \STATE \textbf{Direção estocástica}: $d_k \gets d_k + \tau_k \xi_k$
    \IF{$g_k^\top d_k > 0$}
        \STATE $d_k \gets -H_k g_k$ \COMMENT{Correção para manter direção de descida}
    \ENDIF
    \STATE \textbf{Determinar} $\eta_k = \eta^m$ via busca linear de Armijo, com $m$ mínimo tal que
        \[
        f(x_k + \eta_k d_k) \le f(x_k) + \sigma \eta_k g_k^\top d_k
        \]
    \STATE \textbf{Atualizar ponto}: $x_{k+1} = x_k + \eta_k d_k$
    \STATE \textbf{Calcular} $g_{k+1} = \nabla f(x_{k+1})$
    \STATE \textbf{Definir} $s_k = x_{k+1} - x_k$, \quad $y_k = g_{k+1} - g_k$
    \IF{$y_k^\top s_k > 0$}
        \STATE $Y_k \gets (1-\rho)H_k + \rho V_k$
        \STATE $\phi_k \gets 1/(y_k^\top s_k)$
        \STATE $W_k \gets I - \phi_k s_k y_k^\top$
        \STATE $H_{k+1} \gets W_k Y_k W_k^\top + \phi_k\, s_k s_k^\top$
        \STATE $V_{k+1} \gets (1-\beta)V_k + \beta H_{k+1}$
    \ELSE
        \STATE $H_{k+1} \gets H_k$, \quad $V_{k+1} \gets V_k$
    \ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}

O Algoritmo~\ref{alg:bfgs_ac_stoc} sintetiza a formulação proposta, na qual
a direção de busca combina a aceleração quasi-Newton com a perturbação
estocástica projetada. O decaimento suave de $\tau_k$ atua como um
mecanismo de \emph{resfriamento} (\emph{cooling}): nas iterações iniciais,
a componente aleatória favorece a exploração do espaço de busca, enquanto
nas etapas finais o método torna-se progressivamente mais determinístico,
permitindo que a informação de curvatura acumulada por $H_k$ e $V_k$ guie o
refinamento local. Os valores de $\rho$ e $\beta$ obedecem as faixas
$(0,\rho_{\max})$ e $(\beta_{\min},1)$ determinadas pela análise de
estabilidade, assegurando que as matrizes $H_k$ e $V_k$ permaneçam próximas
e que o esquema acelerado preserve as propriedades estruturais do BFGS no
cone $\mathbb{S}_{++}^n$.

A formulação apresentada até aqui estabelece a versão acelerada e estocástica do BFGS sob o ponto de vista algorítmico e teórico. Resta, entretanto, verificar em que medida a incorporação da memória acelerada e da perturbação estocástica se traduz em ganhos efetivos de desempenho quando comparada tanto à versão clássica do método quanto à sua variante apenas acelerada. Essa comparação é particularmente relevante porque as três versões compartilham a mesma estrutura quasi-Newton básica, diferindo apenas nos mecanismos introduzidos para melhorar a qualidade da direção de busca e a adaptação à geometria local da função.

Com esse objetivo, realizou-se um estudo comparativo entre o BFGS puro, o BFGS acelerado e o BFGS acelerado com componente estocástica em um conjunto amplo de problemas many-objective escalarizados. A análise buscou avaliar, de forma controlada, o impacto isolado de cada modificação proposta, permitindo identificar se os mecanismos de aceleração e de exploração estocástica contribuem para melhorar a qualidade das soluções obtidas, reduzir o esforço computacional e tornar o método mais robusto em cenários de maior dimensionalidade.

\section{Comparação entre as versões pura, acelerada e acelerada-estocástica do método BFGS}
\label{sec:comparacao_bfgs_variantes}

A avaliação experimental das três variantes do método BFGS foi conduzida
sobre diferentes conjuntos de problemas many-objective, incluindo as
suítes de benchmark MaF e ZCAT, bem como um conjunto de problemas
many-objective do mundo real (RW). O objetivo dessa etapa foi analisar,
em um ambiente padronizado e reprodutível, o efeito da aceleração
matricial e da perturbação estocástica projetada sobre o comportamento
do método de busca local aplicado a subproblemas escalares derivados de
instâncias many-objective.

Para os conjuntos MaF e ZCAT, cada problema foi considerado em três
configurações de número de objetivos, correspondentes a
$M \in \{5,10,15\}$. Essa escolha permite avaliar o comportamento das
variantes do método em cenários de complexidade crescente, refletindo o
aumento da dificuldade associado à expansão da dimensionalidade no
espaço objetivo.

A comparação entre os métodos foi realizada por meio de uma estratégia
de escalarização aplicada a cada problema many-objective. Para cada
combinação de problema e número de objetivos, foram geradas
$K=100$ escalarizações independentes, definidas por vetores de pesos
$\lambda \in \mathbb{R}^M$ amostrados aleatoriamente de forma uniforme
no simplex unitário. Cada vetor $\lambda$ define um subproblema escalar
distinto, permitindo que a avaliação contemple diferentes regiões da
fronteira de Pareto e forneça uma comparação menos dependente de uma
única direção de preferência.

Para a construção das funções escalares, foram previamente estimados os
vetores ideal e nadir de cada instância por amostragem aleatória
uniforme no espaço de decisão, utilizando $20\,000$ pontos por
problema. A partir das avaliações objetivas obtidas nessa amostra,
definiu-se o vetor ideal como o mínimo componente a componente e o
vetor nadir como o máximo componente a componente. Embora tais vetores
sejam aproximados, essa estratégia fornece uma normalização consistente
entre diferentes escalarizações e problemas.

As três variantes analisadas foram: o BFGS clássico, denotado por
\texttt{BFGS}; o BFGS com aceleração matricial, denotado por
\texttt{ACC}; e o BFGS acelerado com componente estocástica na direção
de busca, denotado por \texttt{STO}. Em cada escalarização, os três
métodos foram executados sobre exatamente o mesmo subproblema escalar e
com a mesma inicialização pseudoaleatória, assegurada pelo uso da mesma
semente associada a cada índice $k$ da escalarização. Mais
especificamente, para a $k$-ésima escalarização utilizou-se a semente
\texttt{seed + k} em todas as três execuções. Esse procedimento reduz a
influência de fatores aleatórios externos e torna a comparação entre os
métodos mais justa.

Em todas as execuções, o orçamento computacional foi fixado em
$\texttt{maxFE}=500$ avaliações da função objetivo escalarizada. Para
cada execução foram registrados o valor final da função objetivo
escalarizada e o número de avaliações de função utilizadas, permitindo
a posterior construção de medidas agregadas de desempenho.

Os parâmetros $\rho$ e $\beta$, responsáveis por controlar o mecanismo
de aceleração do método acelerado, foram ajustados automaticamente por
meio da ferramenta \textit{iRace}~\cite{lopez2016irace}. O processo de
ajuste foi conduzido separadamente para cada conjunto de problemas
considerado neste trabalho (MaF, ZCAT e RW), permitindo obter
configurações de parâmetros adequadas às diferentes características
estruturais dessas instâncias. Os valores selecionados pelo procedimento
de \textit{tuning} foram então fixados em todas as execuções
experimentais descritas nesta seção e são apresentados na
Tabela~\ref{tab:irace_params}.

\begin{table}[h]
\centering
\caption{Parâmetros do mecanismo de aceleração do método BFGS obtidos via \textit{iRace}. 
Os valores de $\rho$ e $\beta$ foram ajustados separadamente para cada conjunto de problemas
considerado e utilizados nas variantes aceleradas do método (ACC e STO).}
\label{tab:irace_params}
\begin{tabular}{ccc}
\hline
Conjunto de Problemas & $\rho$ & $\beta$ \\
\hline
MaF   & 0.01 & 0.87 \\
ZCAT  &  0.27 & 0.89  \\
RW    & 0.31 & 0.52 \\
\hline
\end{tabular}
\end{table}

A comparação entre as variantes foi realizada por meio de perfis de
desempenho. Além do perfil clássico, foram também construídas versões
ponderadas desses perfis com o objetivo de capturar diferenças
estruturais entre as instâncias avaliadas.

Primeiramente, foram considerados perfis ponderados pela
dimensionalidade do problema. Nesse caso, cada dimensão recebeu um peso
proporcional ao número de objetivos $M$, de modo que problemas com maior
dimensionalidade exerçam maior influência na comparação. Em seguida,
foram construídos perfis ponderados pela dificuldade computacional das
instâncias. Para isso, os problemas foram classificados em três níveis
de dificuldade com base no número médio de avaliações da função
objetivo escalarizada (FE) necessárias para atingir a solução final.
Essa classificação foi realizada por tercis, atribuindo-se pesos $3$,
$2$ e $1$ para os níveis de dificuldade alto, médio e baixo,
respectivamente. Em todos os casos, os pesos foram normalizados pela
soma total, garantindo a comparabilidade entre os diferentes perfis.

Por fim, foram também considerados perfis ponderados simultaneamente
pelos dois critérios, combinando os pesos associados à dimensionalidade
e à dificuldade computacional. Essa estratégia permite avaliar o
desempenho relativo dos métodos não apenas em termos médios, mas também
levando em conta a complexidade estrutural e computacional das
instâncias analisadas.

Os resultados obtidos a partir desse protocolo experimental são
apresentados na sequência, destacando o desempenho relativo das três
variantes do BFGS nos diferentes conjuntos de problemas considerados.

\subsection{Análise comparativa das variantes do método BFGS}

A comparação entre as três variantes do método BFGS foi realizada por
meio de perfis de desempenho construídos a partir dos resultados
obtidos nas diferentes instâncias consideradas. Cada curva representa a
função $\rho_s(\tau)$, que indica a fração de problemas para os quais um
método $s$ apresenta desempenho dentro de um fator $\tau$ do melhor
resultado observado. A interpretação dos perfis considera
simultaneamente três indicadores: a área normalizada sob o perfil
(AUC), que reflete o desempenho médio global do método; o valor
$\rho(1)$, que corresponde à fração de instâncias em que o método
obtém o melhor resultado; e a métrica $R$, associada ao pior caso
observado. Além do perfil global, foram considerados perfis ponderados
pela dimensionalidade dos problemas ($M$), pela dificuldade
computacional estimada a partir do número de avaliações da função
objetivo (FE), e pela combinação desses dois critérios.

Os resultados obtidos para os problemas da suíte MaF são apresentados
na Figura~\ref{fig:perfis_maf}. Observa-se uma vantagem consistente da
variante estocástica do método. No perfil global
(Figura~\ref{fig:maf_base}), bem como nos perfis ponderados pela
dimensionalidade do problema (Figura~\ref{fig:maf_M}), pela dificuldade
computacional (Figura~\ref{fig:maf_FE}) e pela combinação desses dois
critérios (Figura~\ref{fig:maf_FEM}), o método STOC-BFGS apresenta a
maior área sob o perfil, indicando o melhor desempenho médio global
entre as variantes avaliadas. Além disso, essa variante também obtém os
maiores valores de $\rho(1)$, indicando que alcança o melhor resultado
em uma fração significativamente maior de instâncias. Esse comportamento
sugere que a introdução da perturbação estocástica na direção de busca
favorece a exploração do espaço de decisão, permitindo ao método
identificar com maior frequência direções promissoras de descida e
escapar de regiões em que a informação de curvatura local é pouco
informativa.

\begin{figure}[ht]
\centering

\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/maf_base}
\caption{Perfil global}
\label{fig:maf_base}
\end{subfigure}
\hfill
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/maf_M}
\caption{Perfil ponderado por $M$}
\label{fig:maf_M}
\end{subfigure}

\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/maf_FE}
\caption{Perfil ponderado por FE}
\label{fig:maf_FE}
\end{subfigure}
\hfill
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/maf_FEM.eps}
\caption{Perfil ponderado por $M$ e FE}
\label{fig:maf_FEM}
\end{subfigure}

\caption{Perfis de desempenho das variantes BFGS, ACC-BFGS e STO-BFGS
para os problemas da suíte MaF.}
\label{fig:perfis_maf}

\end{figure}


Para os problemas da suíte ZCAT, apresentados na
Figura~\ref{fig:perfis_zcat}, observa-se um comportamento mais
equilibrado entre as variantes. Em termos de desempenho médio global
(AUC), as três versões apresentam resultados bastante próximos, com
pequenas variações dependendo do critério de ponderação considerado.
No perfil global (Figura~\ref{fig:zcat_base}), o BFGS clássico apresenta
ligeira vantagem em consistência média, enquanto nos perfis ponderados
pela dimensionalidade (Figura~\ref{fig:zcat_M}) e pela combinação de
dimensão e dificuldade (Figura~\ref{fig:zcat_FEM}) a versão acelerada
apresenta desempenho médio comparável ou ligeiramente superior. Ainda
assim, um aspecto particularmente relevante nesses resultados é o
comportamento do indicador $\rho(1)$. Em todos os perfis analisados,
incluindo os perfis ponderados por dificuldade
(Figura~\ref{fig:zcat_FE}), a variante estocástica apresenta os maiores
valores desse parâmetro, indicando que o método STOC-BFGS é aquele que
mais frequentemente atinge o melhor resultado entre os métodos
comparados. Esse resultado sugere que, embora o desempenho médio global
permaneça semelhante entre as variantes, a introdução da componente
estocástica aumenta a probabilidade de obtenção da melhor solução em
instâncias individuais, ampliando a capacidade do método de explorar
regiões promissoras da superfície de otimização.

\begin{figure}[ht]
\centering

\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/zcat_base}
\caption{Perfil global}
\label{fig:zcat_base}
\end{subfigure}
\hfill
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/zcat_M}
\caption{Perfil ponderado por $M$}
\label{fig:zcat_M}
\end{subfigure}

\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/zcat_FE}
\caption{Perfil ponderado por FE}
\label{fig:zcat_FE}
\end{subfigure}
\hfill
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/zcat_FEM}
\caption{Perfil ponderado por $M$ e FE}
\label{fig:zcat_FEM}
\end{subfigure}

\caption{Perfis de desempenho das variantes BFGS, ACC-BFGS e STO-BFGS
para os problemas da suíte ZCAT.}
\label{fig:perfis_zcat}

\end{figure}


Os resultados obtidos para os problemas many-objective do mundo real
são apresentados na Figura~\ref{fig:perfis_rw}. Nesse conjunto de
instâncias observa-se novamente uma vantagem clara da variante
estocástica. No perfil global (Figura~\ref{fig:rw_base}) e nos perfis
ponderados pela dimensionalidade (Figura~\ref{fig:rw_M}) e pela
dificuldade computacional (Figura~\ref{fig:rw_FE}), o método STOC-BFGS
apresenta a maior área sob o perfil e os menores valores da métrica
$R$, indicando simultaneamente melhor desempenho médio e maior
robustez no pior caso observado. Além disso, essa variante também
apresenta valores elevados de $\rho(1)$, indicando maior frequência de
obtenção do melhor resultado entre as instâncias avaliadas. Esse
comportamento sugere que a introdução da componente estocástica torna o
método particularmente eficaz em problemas com estruturas de otimização
mais complexas ou menos regulares, como frequentemente ocorre em
aplicações do mundo real.

\begin{figure}[ht]
\centering

\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/rw_base}
\caption{Perfil global}
\label{fig:rw_base}
\end{subfigure}
\hfill
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/rw_M}
\caption{Perfil ponderado por $M$}
\label{fig:rw_M}
\end{subfigure}

\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/rw_FE}
\caption{Perfil ponderado por FE}
\label{fig:rw_FE}
\end{subfigure}

\caption{Perfis de desempenho das variantes BFGS, ACC-BFGS e STO-BFGS
para os problemas da suíte RW.}
\label{fig:perfis_rw}

\end{figure}


Considerando conjuntamente os três conjuntos de problemas analisados,
observa-se que a introdução da componente estocástica tende a produzir
os maiores ganhos de desempenho, especialmente nos problemas MaF e RW,
nos quais essa variante apresenta vantagem consistente tanto em
desempenho médio quanto na frequência de obtenção da melhor solução.
Nos problemas ZCAT, embora o desempenho médio global permaneça
semelhante entre as variantes, o método estocástico ainda se destaca
por apresentar os maiores valores do indicador $\rho(1)$, evidenciando
maior capacidade de alcançar o melhor resultado em instâncias
individuais. De maneira geral, os resultados indicam que a aceleração
matricial contribui para melhorar a consistência do método, enquanto a
introdução da componente estocástica amplia sua capacidade de
exploração local, aumentando a probabilidade de encontrar soluções de
melhor qualidade em diferentes cenários de otimização.

Os resultados apresentados neste capítulo evidenciam que métodos de busca
local baseados em aproximações quasi-Newton constituem uma alternativa
eficiente para o refinamento de subproblemas escalares derivados de
instâncias many-objective. Em particular, observou-se que as variantes
aceleradas do método BFGS, especialmente quando combinadas com um
mecanismo de perturbação estocástica controlada, apresentam melhorias
consistentes na qualidade das soluções obtidas, mantendo simultaneamente
boa robustez em diferentes classes de problemas.

Entretanto, no contexto da otimização many-objective, o papel da busca
local não é atuar de forma isolada, mas sim como um componente de
intensificação dentro de um processo de busca mais amplo. Enquanto os
algoritmos evolutivos são responsáveis pela exploração global do espaço
de decisão e pela manutenção da diversidade das soluções ao longo da
fronteira de Pareto, a busca local atua refinando soluções individuais
em regiões promissoras previamente identificadas.

Nesse cenário, uma questão central diz respeito à definição de quando a
busca local deve ser ativada ao longo do processo evolutivo. Uma
ativação prematura pode comprometer a diversidade e levar a uma
exploração excessivamente local, enquanto uma ativação tardia pode
reduzir o impacto do refinamento na qualidade final das soluções.
Assim, a eficácia da integração entre exploração global e
intensificação local depende diretamente da definição de um critério de
ativação adequado.

Diante disso, o próximo capítulo é dedicado à proposição de um critério
de ativação da busca local baseado em estabilidade, que visa identificar
momentos apropriados para a aplicação da busca local a partir do
comportamento do processo evolutivo. Esse critério constitui um elemento
fundamental para a construção do framework híbrido apresentado
posteriormente.



==> bfgs_acc_sto_artigo.tex <==
\section{Introduction}
A otimização many-objective impõe desafios fundamentais decorrentes do equilíbrio entre exploração global e refinamento local. Embora algoritmos evolutivos many-objective (MaOEAs) sejam eficazes na exploração do espaço de decisão e na preservação da diversidade populacional, sua natureza estocástica frequentemente limita a velocidade de convergência em regiões próximas ao fronte de Pareto. Em particular, quando soluções já se encontram em regiões promissoras, a ausência de mecanismos estruturados de intensificação pode comprometer a obtenção de soluções de alta precisão.
Nesse cenário, a incorporação de métodos determinísticos de busca local constitui uma abordagem natural para promover refinamento direcionado. Diferentemente dos mecanismos populacionais, métodos baseados em informação de primeira e segunda ordem permitem trajetórias de convergência mais controladas, sendo especialmente adequados para exploração local em problemas contínuos. A integração entre exploração evolutiva e intensificação determinística tem, portanto, se consolidado como uma estratégia promissora em otimização many-objective.
Entre os métodos determinísticos, abordagens quasi-Newton, em particular o BFGS (Broyden–Fletcher–Goldfarb–Shanno) \cite{broyden1970convergence, fletcher1970new, goldfarb1970family, shanno1970conditionin}, destacam-se por combinar eficiência numérica, convergência superlinear e sólida fundamentação teórica. Essas características tornam tais métodos especialmente atrativos em contextos escalarizados, nos quais problemas multiobjetivo são tratados por meio de funções escalares associadas a estratégias de decomposição. Além disso, sua ampla utilização em otimização contínua reforça sua relevância prática e teórica \cite{nocedal2006numerical, prudente2024global, prudente2022quasi, morovati2018quasi}.
Apesar dessas vantagens, o desempenho do BFGS clássico pode ser significativamente degradado em cenários de alta dimensionalidade, superfícies mal condicionadas ou funções multimodais, nos quais a convergência tende a ser lenta ou sujeita à estagnação \cite{dai2002convergence, dai2013perfect, mascarenhas2004bfgs}. Esse comportamento motivou o desenvolvimento de extensões que incorporam mecanismos de aceleração e estocasticidade.
No contexto de aceleração, métodos inspirados em \cite{nesterov1983method} introduzem termos de inércia que permitem antecipar a dinâmica iterativa, reduzindo o número de iterações necessárias para convergência. A adaptação desses conceitos a métodos quasi-Newton tem sido investigada em diferentes trabalhos (\cite{su2016differential, gower2018accelerated, botev2017nesterov}), com destaque para \cite{gower2018accelerated}, que propõe uma formulação acelerada baseada na atualização da inversa da Hessiana, preservando propriedades de estabilidade e baixo custo computacional.
Paralelamente, a incorporação de estocasticidade em métodos quasi-Newton tem sido explorada como mecanismo para lidar com ruído e melhorar a capacidade exploratória. Diferentes abordagens investigaram adaptações do BFGS a ambientes estocásticos \cite{byrd2016stochastic, wang2017stochastic, schraudolph2007stochastic}, incluindo estratégias para lidar com gradientes imprecisos \cite{shi2022noise}, revisões sistemáticas sobre variantes estocásticas \cite{guo2023overview}, algoritmos específicos para otimização sob ruído \cite{amos2020algorithm}, e modelos de geração de direções de busca em ambientes incertos \cite{peng2025finding}. Esses resultados indicam que a estocasticidade pode atuar não apenas como modelo de incerteza, mas também como mecanismo ativo para evitar estagnação.
Mais recentemente, esforços têm sido direcionados à combinação de aceleração e estocasticidade em um mesmo arcabouço quasi-Newton, como no método RES-NAQ \cite{makmuang2023regularized}. No entanto, tais abordagens tipicamente incorporam ruído nas estimativas de gradiente ou nas atualizações de Hessiana, sem explorar explicitamente sua atuação na direção de busca.
Neste trabalho, propõe-se uma formulação quasi-Newton que integra aceleração e estocasticidade por meio de um mecanismo de ruído controlado aplicado diretamente à direção de busca. Diferentemente das abordagens existentes \cite{shi2022noise, guo2023overview, peng2025finding}, a proposta introduz explicitamente perturbações estruturadas na direção iterativa, com o objetivo de ampliar a capacidade exploratória e reduzir a ocorrência de estagnação em mínimos locais, preservando simultaneamente as propriedades de convergência do esquema quasi-Newton acelerado baseado em \cite{gower2018accelerated}.
A análise teórica desenvolvida estabelece condições sob as quais o método proposto mantém estabilidade e comportamento de convergência comparáveis ao BFGS clássico, ao mesmo tempo em que incorpora mecanismos adicionais de exploração. Esses resultados fornecem base rigorosa para a utilização do método como componente de intensificação em estruturas híbridas de otimização many-objective baseadas em decomposição.

\section{Método BFGS}

Nos métodos quasi-Newton, o BFGS tradicional constrói iterativamente uma aproximação $X_k \approx H_k^{-1}$ utilizando apenas informações de primeira ordem. A atualização é definida de modo a satisfazer a condição de secante, que impõe consistência entre o deslocamento no espaço de decisão e a variação observada no gradiente.

Considere os vetores
$$
s_k = x_{k+1} - x_k, 
\qquad
\zeta_k = \nabla f(x_{k+1}) - \nabla f(x_k),
$$
onde $s_k$ representa o passo na variável de decisão, e $\zeta_k$ a variação correspondente no gradiente. A condição de secante impõe que
$$
X_{k+1} \zeta_k = s_k,
$$
enquanto a simetria $X_{k+1} = X_{k+1}^\top$ é requerida para preservar a estrutura da Hessiana.

A atualização de BFGS pode então ser caracterizada como a solução do problema
\begin{equation}
X_{k+1} = \arg\min_X \|X - X_k\|_F^2 
\quad \text{sujeito a} \quad X \zeta_k = s_k, \; X = X^\top,
\label{eq:bfgs_opt}
\end{equation}
cuja solução é dada por
\begin{equation}
X_{k+1} 
= \frac{s_k s_k^\top}{s_k^\top \zeta_k}
+ \left(I - \frac{s_k \zeta_k^\top}{s_k^\top \zeta_k}\right)
X_k
\left(I - \frac{\zeta_k s_k^\top}{s_k^\top \zeta_k}\right).
\label{eq:bfgs_closed_form}
\end{equation}

A primeira parcela em~\eqref{eq:bfgs_closed_form} garante o atendimento da condição de secante, enquanto o segundo termo corresponde à menor correção em norma de Frobenius, $\|A\|_F=\sqrt{\operatorname{Tr}(A^\top A)}$, que preserva simetria e, sob a condição $\zeta_k^\top s_k > 0$, a definida positividade de $X_{k+1}$.

Essa formulação fornece a base para as extensões consideradas neste trabalho. Em particular, a interpretação variacional em~\eqref{eq:bfgs_opt} permite introduzir mecanismos adicionais diretamente na atualização de $X_k$. Nos desenvolvimentos subsequentes, essa estrutura será explorada para incorporar termos de aceleração inspirados em \cite{nesterov1983method} e perturbações estocásticas controladas na direção de busca, mantendo as propriedades fundamentais do esquema quasi-Newton.

\section{BFGS Acelerado}
\label{sec:bfgs_acelerado}

Métodos de aceleração baseados em dinâmica inercial, originalmente propostos por \cite{nesterov1983method}, têm sido amplamente utilizados para melhorar a taxa de convergência de métodos iterativos. Em sua forma clássica, tais métodos introduzem um termo de extrapolação que antecipa a direção de movimento no espaço de decisão, reduzindo oscilações e acelerando a convergência.

Neste trabalho, em vez de aplicar a aceleração diretamente sobre as variáveis de decisão, adotamos uma abordagem distinta: os princípios de aceleração são transferidos para o espaço das matrizes que aproximam a inversa da Hessiana. Em particular, a dinâmica inercial é incorporada à sequência $\{X_k\}$, onde $X_k \approx H_k^{-1}$, conforme discutido em \cite{gower2018accelerated}.

Nessa formulação, a variável inercial deixa de ser um vetor e passa a ser uma matriz auxiliar que acumula informação histórica sobre aproximações de $H^{-1}$. Em outras palavras, a aceleração atua diretamente sobre a sequência de matrizes $\{X_k\}$ que aproximam a inversa da Hessiana $H^{-1}$, e não sobre o vetor de decisão $x_k$.

A transposição do método de Nesterov para o espaço das matrizes requer algumas modificações conceituais e algébricas. Diferentemente das variáveis vetoriais, as aproximações da inversa da Hessiana pertencem ao conjunto das matrizes simétricas definidas positivas (SPD), denotado por $\mathbb{S}_{++}^n$. Esse conjunto não forma um espaço vetorial: combinações lineares arbitrárias de matrizes SPD podem resultar em matrizes indefinidas. Consequentemente, as operações lineares de extrapolação utilizadas no método clássico, como $X_k + \mu(X_k - X_{k-1})$, não preservam a positividade definida e, portanto, não são adequadas para atualizar diretamente a sequência $\{X_k\}$.

Assim como no caso vetorial, deseja-se incorporar um termo de inércia que antecipe a direção de evolução da métrica quasi-Newton. No entanto, como vimos, a geometria não linear do cone $\mathbb{S}_{++}^n$ impede o uso de uma única variável de momentum, como ocorre na forma clássica de Nesterov. Por isso, no esquema matricial usaremos dois parâmetros distintos: um que controle a interpolação segura entre as aproximações da inversa da Hessiana (aqui denotado por $\rho\in(0,1)$) e outro que regule a suavização inercial da sequência auxiliar (denotado por $\beta\in[0,1)$). Essa separação é necessária para preservar a positividade definida das matrizes e evitar instabilidades numéricas decorrentes de extrapolações excessivas.

A sequência auxiliar $\{V_k\}$, então, acumula, de forma suavizada, a informação histórica do processo de atualização. A cada iteração, combina-se $V_k$ e $X_k$ por meio de uma combinação convexa, que garante que o ponto intermediário permaneça dentro do cone $\mathbb{S}_{++}^n$:
\begin{equation}
Y_k = (1-\rho)X_k + \rho V_k,
\label{eq:yk_iter}
\end{equation}
em que $\rho$ controla a contribuição inercial e desempenha papel análogo ao fator de momentum do método vetorial, porém restrito a uma interpolação convexa para assegurar que $Y_k \in \mathbb{S}_{++}^n$, ou seja $Y_k \succ0$. O ponto $Y_k$ atua, assim, como um análogo matricial do ponto extrapolado $y_k$ de Nesterov: antecipa a direção de movimento no espaço das métricas sem comprometer a coerência geométrica do método.

A atualização quasi-Newton é então executada sobre $Y_k$, resultando em uma nova aproximação $X_{k+1}$:
\begin{equation}
X_{k+1} = \Phi_{\text{BFGS}}(Y_k;\,s_k,\zeta_k),
\label{eq:xk_iter}
\end{equation}
onde $\Phi_{\text{BFGS}}$ representa a transformação BFGS aplicada aos vetores
$$
s_k = x_{k+1}-x_k, \qquad \zeta_k = \nabla f(x_{k+1})-\nabla f(x_k).
$$
Essa etapa preserva a positividade definida sempre que $s_k^\top\zeta_k>0$, condição usual em métodos quasi-Newton. Dessa forma, a projeção quasi-Newton garante que $X_{k+1}\in\mathbb{S}_{++}^n$ mesmo que $Y_k$ apresente leve desvio da região interior do cone.

Após essa etapa, a variável auxiliar $V_k$ é atualizada iterativamente por uma média convexa que incorpora a nova aproximação da inversa da Hessiana e, ao mesmo tempo, mantém memória do estado anterior:
\begin{equation}
V_{k+1} = (1-\beta)V_k + \beta X_{k+1},
\label{eq:vk_iter}
\end{equation}
onde $\beta$ regula a taxa de amortecimento inercial. Valores baixos de $\beta$ produzem uma atualização mais suave e estável, enquanto valores próximos de $1$ tornam o método mais responsivo às variações recentes da curvatura local.

As equações~\eqref{eq:yk_iter}–\eqref{eq:vk_iter} definem um esquema de aceleração discreto e numericamente estável, no qual:
\begin{enumerate}
    \item \textbf{A combinação convexa} entre $X_k$ e $V_k$ preserva a positividade definida, assegurando que $Y_k\in\mathbb{S}_{++}^n$;
    \item \textbf{A atualização quasi-Newton} $\Phi_{\text{BFGS}}$ mantém $X_{k+1}$ simétrica e definida positiva sob a condição $s_k^\top\zeta_k>0$;
    \item \textbf{A atualização inercial} de $V_k$ suaviza a dinâmica, controlando a propagação do termo de inércia e evitando oscilações em regiões mal condicionadas.
\end{enumerate}

Em termos conceituais, a iteração acelerada quasi-Newton pode ser vista como um sistema de duas camadas: a camada interna, representada pela transformação $\Phi_{\text{BFGS}}$, assegura a coerência geométrica no cone das SPD; a camada externa, definida pelas atualizações de $Y_k$ e $V_k$, reproduz o comportamento inercial do método de Nesterov em um formato totalmente discreto e compatível com o domínio matricial. O resultado é uma formulação iterativa que combina a adaptabilidade dos métodos quasi-Newton com uma dinâmica de aceleração controlada, dispensando a necessidade de análise contínua ou de parâmetros derivados de sistemas diferenciais.

Para estabelecer rigorosamente as propriedades estruturais e de estabilidade do esquema proposto, analisamos a seguir a evolução iterativa das sequências envolvidas, com ênfase na preservação da positividade definida e no comportamento energético do método.

\subsection{Análise iterativa e preservação de propriedades estruturais}
\label{subsec:analise_iterativa}

Para fundamentar as propriedades estruturais e de estabilidade do esquema iterativo descrito acima, são apresentados a seguir alguns resultados auxiliares. Esses resultados estabelecem condições suficientes para a preservação da positividade definida e para o decréscimo monótono de um funcional de Lyapunov, $\mathcal{E}_k$, associado às sequências $\{X_k,V_k,x_k\}$.

\begin{lemma}%[Convexidade de $\mathbb{S}_{++}^n$ e herança de cotas espectrais]
\label{lem:convex_spd_bounds}
Se $X_k,V_k\in\mathbb{S}_{++}^n$ satisfazem $mI\preceq X_k,V_k\preceq MI$ para algum $0<m\le M$, então, para todo $\rho\in(0,1)$,
$$
Y:=(1-\rho)X_k+\rho V_k\in\mathbb{S}_{++}^n
\quad\text{e}\quad
mI\preceq Y\preceq MI.
$$
\begin{proof} Para todo $z\neq 0$, $$z^\top Y_k z=(1-\rho)z^\top X_k z+\rho z^\top V_k z>0$$
Além disso, $$\lambda_{\min}(Y_k)\ge (1-\rho)\lambda_{\min}(X_k)+\rho\lambda_{\min}(V_k)\ge m$$ e 
$$\lambda_{\max}(Y_k)\le (1-\rho)\lambda_{\max}(X_k)+\rho\lambda_{\max}(V_k)\le M$$ 
\end{proof}
\end{lemma}

O mesmo argumento se aplica à variável auxiliar $V_k$, cuja atualização também consiste em uma combinação convexa de matrizes em $\mathbb{S}_{++}^n$.

%Um argumento inteiramente análogo pode ser aplicado à variável auxiliar $V_k$, cuja atualização iterativa é dada por uma média convexa entre duas matrizes simétricas definidas positivas. De fato, se $V_k, X_{k+1} \in \mathbb{S}_{++}^n$ satisfazem $mI \preceq (\cdot) \preceq MI$ para algum $0 < m \le M$, então, para qualquer $\beta \in (0,1)$,
%$$ V_{k+1} = (1-\beta)V_k + \beta X_{k+1} \in \mathbb{S}_{++}^n,
%\qquad
%mI \preceq V_{k+1} \preceq MI.$$
Logo, tanto $Y_k$ quanto $V_{k+1}$ preservam a positividade definida por construção, assegurando que todas as variáveis matriciais do método permaneçam no cone $\mathbb{S}_{++}^n$ ao longo das iterações.
A garantia de que as variáveis intermediárias $Y_k$ e $V_k$ permanecem no cone $\mathbb{S}_{++}^n$ é essencial para que a etapa quasi-Newton subsequente preserve a estrutura definida positiva da matriz de curvatura. Uma vez assegurada essa propriedade de convexidade matricial, pode-se aplicar a atualização clássica de BFGS sobre $Y_k$, conforme estabelecido no Lema \ref{lem:bfgs_spd}. Tal resultado demonstra que, sob a condição de curvatura $s_k^\top \zeta_k > 0$, a transformação de BFGS mantém a positividade definida da nova matriz $X_{k+1}$, completando assim o ciclo de estabilidade estrutural entre as etapas de extrapolação e de atualização quasi-Newton.

\begin{lemma}%[Preservação de SPD pelo BFGS]
\label{lem:bfgs_spd}
Considere $Y_k\in\mathbb{S}_{++}^n$ e vetores $s,\zeta\in\mathbb{R}^n$ tais que $\zeta^\top s>0$. 
A atualização BFGS clássica
$$
X_{k+1}
= \Big(I-\tfrac{s \zeta^\top}{\zeta^\top s}\Big)\,Y_k\,\Big(I-\tfrac{\zeta s^\top}{\zeta^\top s}\Big)
  + \tfrac{s s^\top}{\zeta^\top s}
$$
satisfaz $X_{k+1}\in\mathbb{S}_{++}^n$. 
\begin{proof}
Seja $Y_k\in\mathbb{S}_{++}^n$ e $s,\zeta\in\mathbb{R}^n$ com $\zeta^\top s>0$. 
Defina
$$
\phi := \frac{1}{\zeta^\top s} \;>\; 0
\qquad\text{e}\qquad
M := I - \phi\,\zeta s^\top .
$$
Note que $M^\top = I - \phi\, s\zeta^\top$. A atualização BFGS-inversa pode ser escrita como
$$
X_{k+1}
= \big(I-\phi\, s\zeta^\top\big)\,Y_k\,\big(I-\phi\,\zeta s^\top\big)
  + \phi\,ss^\top
= M^\top Y_k M + \phi\,ss^\top .
$$
Para qualquer $z\neq 0$,
$$
z^\top X_{k+1} z
= (Mz)^\top Y_k (Mz) \;+\; \phi\,(s^\top z)^2 .
$$
Como $Y\succ 0$, temos $(Mz)^\top Y_k (Mz) > 0$ sempre que $Mz\neq 0$. Portanto, 
no caso $Mz\neq 0$ já concluímos $z^\top X_{k+1} z>0$.

Resta analisar o caso $Mz=0$. Da definição de $M$,
$$
Mz=0 \;\;\Longleftrightarrow\;\; z - \phi\,\zeta (s^\top z)=0 
\;\;\Longleftrightarrow\;\; z = \phi\,\zeta (s^\top z).
$$
Como $z\neq 0$ e $\phi>0$, segue que $s^\top z \neq 0$. Logo, o segundo termo acima satisfaz
$$
\phi\,(s^\top z)^2 \;>\; 0,
$$
o que implica novamente $z^\top X_{k+1} z>0$. Em ambas as situações, para todo $z\neq 0$,
temos $z^\top X_{k+1} z>0$, isto é, $X_{k+1}\in\mathbb{S}_{++}^n$.
Além disso, a simetria de $X_{k+1}$ decorre do fato de que $Y_k$ é simétrica e as operações
utilizadas preservam simetria.
\end{proof}

\end{lemma}

Com base nos resultados acima, é possível conduzir a análise de estabilidade do esquema completo, considerando de forma conjunta a evolução das variáveis $x_k$ e das aproximações da Hessiana. O Teorema \ref{thm:Lyapunov}, que constiui o principal fundamento teórico do método proposto,  formaliza esse resultado, mostrando que, sob hipóteses de suavidade e passos $\eta_k$ suficientemente pequenos, existe uma função de Lyapunov $\mathcal{E}_k$ que decresce monotonamente ao longo das iterações. Essa função combina o valor da função objetivo com um termo de coerência entre as matrizes $X_k$ e $V_k$, refletindo tanto o progresso do método quanto a estabilidade das aproximações obtidas. 

Além disso, na demonstração do teorema verifica-se que essa propriedade de
decréscimo exige apenas que os parâmetros de aceleração $\rho$ e $\beta$
pertencentes ao intervalo $(0,1)$ sejam escolhidos dentro de uma faixa
compatível com as desigualdades envolvidas. Em particular, valores
moderados desses parâmetros garantem que os termos inerciais sejam
suficientemente amortecidos, assegurando que a dinâmica acoplada entre
$X_k$ e $V_k$ permaneça estável. Dessa forma, o teorema sintetiza não
apenas as propriedades de preservação estrutural e estabilidade numérica
do método, mas também estabelece condições explícitas sobre os parâmetros
de aceleração que asseguram a consistência do BFGS acelerado proposto.

\begin{theorem}%[Decrescimento tipo-Lyapunov para o esquema acelerado quasi-Newton]
\label{thm:Lyapunov}
Considere $f:\mathbb{R}^n\to\mathbb{R}$ de classe $C^1$ com gradiente 
$L$-Lipschitz em uma região compacta que contém a sequência iterativa.
Seja o esquema definido por
\begin{align*}
x_{k+1} &= x_k - \eta_k X_k \nabla f(x_k),\\[0.1cm]
Y_k &= (1-\rho)X_k + \rho V_k,\qquad \rho\in(0,\rho_{\max}),\\[0.1cm]
X_{k+1} &= \Phi_{\mathrm{BFGS}}(Y_k;\, s_k,\zeta_k),\quad
s_k := x_{k+1}-x_k,\quad 
\zeta_k := \nabla f(x_{k+1})-\nabla f(x_k),\\[0.1cm]
V_{k+1} &= (1-\beta)V_k + \beta X_{k+1},\qquad \beta\in(\beta_{\min},1),
\end{align*}
com inicialização $X_0 = V_0 = I$.

Suponha que $s_k^\top \zeta_k > 0$ para todo $k$ (o que garante que 
$X_{k+1}\in S_{++}^n$) e que existem constantes $0 < m_* \le M_* < \infty$ tais que
$$
m_* I \preceq X_k,\,V_k,\,Y_k \preceq M_* I,\qquad\text{para todo }k.
$$

Assuma ainda que os passos $\eta_k$ satisfazem uma condição de 
decréscimo suficiente, isto é, existe $c_1>0$ tal que
\begin{equation}\label{eq:suf-descent}
f(x_{k+1}) \le f(x_k) - c_1\|\nabla f(x_k)\|^2 ,
\end{equation}
como obtido, por exemplo, por uma busca de linha do tipo Armijo.

Defina, para $\kappa>0$,
$$
\mathcal{E}_k := f(x_k)-f^* + \kappa\|X_k - V_k\|_F^2 .
$$

Então, existem $\kappa^*>0$ e uma constante $c_2>0$
(dependentes apenas de $m_*,M_*,L,\rho_{\max},\beta_{\min}$)
tais que, para qualquer $\kappa\in(0,\kappa^*)$ e para todo $k$,
\begin{equation}\label{eq:lyapunov-descent}
\mathcal{E}_{k+1}
\;\le\; 
\mathcal{E}_k
\;-\;
c_1\|\nabla f(x_k)\|^2
\;-\;
c_2\|X_{k+1}-V_k\|_F^2 .
\end{equation}

Em particular, a sequência $\{\mathcal{E}_k\}$ é não crescente,
o que garante estabilidade discreta no sentido de Lyapunov e assegura
que $\|X_k - V_k\|_F \to 0$ ao longo das iterações.
\end{theorem}

\begin{proof}
Defina, para $\kappa>0$, a função de Lyapunov
$$
\mathcal{E}_k \;:=\; f(x_k)-f^* \;+\; \kappa\|X_k - V_k\|_F^2.
$$
Nosso objetivo é mostrar que, para escolhas apropriadas de
$\rho\in(0,\rho_{\max})$, $\beta\in(\beta_{\min},1)$ e $\kappa>0$
suficientemente pequeno, existem constantes $c_1,c_2>0$ tais que
\begin{equation}\label{eq:Lyap-target}
\mathcal{E}_{k+1}
\;\le\;
\mathcal{E}_k
-
c_1\|\nabla f(x_k)\|^2
-
c_2\|X_{k+1}-V_k\|_F^2
\qquad\text{para todo }k.
\end{equation}

\medskip
\noindent\textbf{Passo 1: Decomposição da variação de $\mathcal{E}_k$.}
Pela definição de $\mathcal{E}_k$,
$$
\mathcal{E}_{k+1}-\mathcal{E}_k
=
\underbrace{f(x_{k+1})-f(x_k)}_{\text{termo I}}
+
\kappa\underbrace{\Big(\|X_{k+1}-V_{k+1}\|_F^2-\|X_k-V_k\|_F^2\Big)}_{\text{termo II}}.
$$
 Pelo $L$-Lipschitz do gradiente,
$$
f(x_{k+1}) \le f(x_k) - \eta_k \nabla f(x_k)^\top X_k \nabla f(x_k) + \tfrac{L}{2}\eta_k^2 \|X_k\nabla f(x_k)\|^2.
$$
Usando $m_\ast I\preceq X_k\preceq M_\ast I$ obtém-se
$$
f(x_{k+1}) \le f(x_k) - c_1 \|\nabla f(x_k)\|^2
$$
com $c_1=\eta_k m_\ast - \tfrac{L}{2}\eta_k^2 M_\ast^2>0$ quando $\eta_k\le 1/(M_\ast L)$, o que coincide com \eqref{eq:suf-descent}.

Resta, portanto, controlar o termo II
$$
\Delta_k^{\mathrm{mat}}
:=
\|X_{k+1}-V_{k+1}\|_F^2-\|X_k-V_k\|_F^2.
$$

\medskip
\noindent\textbf{Passo 2: Reescrita do termo II.}
Da definição de $V_{k+1}$,
$$
V_{k+1} = (1-\beta)V_k + \beta X_{k+1},
$$
deduzimos
$$
X_{k+1}-V_{k+1}
=
X_{k+1} - \big((1-\beta)V_k+\beta X_{k+1}\big)
=
(1-\beta)(X_{k+1}-V_k),
$$
de modo que
$$
\|X_{k+1}-V_{k+1}\|_F^2
=
(1-\beta)^2\|X_{k+1}-V_k\|_F^2.
$$
Logo,
\begin{equation}\label{eq:Delta-mat-0}
\Delta_k^{\mathrm{mat}}
=
(1-\beta)^2\|X_{k+1}-V_k\|_F^2 - \|X_k-V_k\|_F^2.
\end{equation}

\medskip
\noindent\textbf{Passo 3: Desigualdade de Young matricial com parâmetros $\theta$ e $\varepsilon$.}
Sejam $\theta,\varepsilon\in(0,1)$ a serem fixados adiante. Escrevemos
$$
-\|X_k-V_k\|_F^2
=
-\theta\|X_k-V_k\|_F^2
-
(1-\theta)\|X_k-V_k\|_F^2.
$$
Aplicamos, então, a desigualdade de Young matricial na forma
$$
\|A\|_F^2
\ge
(1-\varepsilon)\|B\|_F^2
-
\Big(\tfrac{1}{\varepsilon}-1\Big)\|A-B\|_F^2,
$$
válida para quaisquer $A,B\in\mathbb{R}^{n\times n}$ e $\varepsilon\in(0,1)$.
Tomando $A:=X_k-V_k$ e $B:=X_{k+1}-V_k$, obtemos
$$
-\,(1-\theta)\|X_k-V_k\|_F^2
\;\le\;
-(1-\theta)(1-\varepsilon)\|X_{k+1}-V_k\|_F^2
+
(1-\theta)\Big(\tfrac{1}{\varepsilon}-1\Big)\|X_{k+1}-X_k\|_F^2.
$$
Substituindo na expressão de $\Delta_k^{\mathrm{mat}}$ em
\eqref{eq:Delta-mat-0}, resulta
\begin{align}
\Delta_k^{\mathrm{mat}}
&\le
(1-\beta)^2\|X_{k+1}-V_k\|_F^2
-\theta\|X_k-V_k\|_F^2 \nonumber\\
&\quad
-(1-\theta)(1-\varepsilon)\|X_{k+1}-V_k\|_F^2
+
(1-\theta)\Big(\tfrac{1}{\varepsilon}-1\Big)\|X_{k+1}-X_k\|_F^2
\nonumber\\[0.1cm]
&=
\underbrace{\Big((1-\beta)^2-(1-\theta)(1-\varepsilon)\Big)}_{=:~\Gamma_1}\,
\|X_{k+1}-V_k\|_F^2
-
\theta\|X_k-V_k\|_F^2
\nonumber\\
&\quad
+
\underbrace{(1-\theta)\Big(\tfrac{1}{\varepsilon}-1\Big)}_{=:~\Gamma_0}\,
\|X_{k+1}-X_k\|_F^2.\label{eq:Delta-mat-1}
\end{align}

\medskip
\noindent\textbf{Passo 4: Cota de $\|X_{k+1}-X_k\|_F^2$.}
Pelo Lema quasi-Newton (baseado na forma de BFGS sobre $Y_k$) e pelas
cotas espectrais $m_*I\preceq X_k,V_k,Y_k\preceq M_*I$, existe uma
constante $A>0$ (dependente apenas de $m_*,M_*,L$) tal que
\begin{equation}\label{eq:bound-Xdiff-1}
\|X_{k+1}-Y_k\|_F
\;\le\;
A\,\|s_k\|\,\|\zeta_k\|.
\end{equation}
Como $s_k = x_{k+1}-x_k = -\eta_k X_k\nabla f(x_k)$, segue que
$$
\|s_k\|
\le
\eta_k\|X_k\|\,\|\nabla f(x_k)\|
\le
\eta_k M_* \|\nabla f(x_k)\|.
$$
Por Lipschitz-continuidade do gradiente,
$\|\zeta_k\|=\|\nabla f(x_{k+1})-\nabla f(x_k)\|\le L\|s_k\|$, o que implica
$$
\|\zeta_k\|
\le L\|s_k\|
\le L\eta_k M_*\|\nabla f(x_k)\|.
$$
Substituindo em \eqref{eq:bound-Xdiff-1}, obtemos
$$
\|X_{k+1}-Y_k\|_F
\le
A\,\|s_k\|\,\|\zeta_k\|
\le
AL M_*^2 \eta_k^2 \|\nabla f(x_k)\|^2.
$$
Consequentemente, existe $A_1>0$ tal que
\begin{equation}\label{eq:bound-Xdiff-2}
\|X_{k+1}-Y_k\|_F^2
\;\le\;
A_1\,\eta_k^4\,\|\nabla f(x_k)\|^4.
\end{equation}

Além disso, como $Y_k = (1-\rho)X_k + \rho V_k$, obtemos $Y_k-X_k=\rho(V_k-X_k)$. Deste fato e da desilgualdade triangular em $X_{k+1}-X_k=X_{k+1}-Y_k+Y_k-X_k$, temos
\begin{equation}\label{eq:bound-Xdiff-3}
\|X_{k+1}-X_k\|_F
\;\le\;
\|X_{k+1}-Y_k\|_F+\rho\|X_{k}-V_k\|_F
\end{equation}
 e então, de \eqref{eq:bound-Xdiff-2} e da desigualdade de Cauchy-Schwarz (caso especial), concluímos que  

\begin{equation}\label{eq:bound-Xdiff-4}
\|X_{k+1}-X_k\|_F^2
\;\le\;
2A_1\,\eta_k^4\,\|\nabla f(x_k)\|^4
+
2\,\rho^2\,\|X_k-V_k\|_F^2.
\end{equation}


\medskip
\noindent\textbf{Passo 5: Substituição em $\Delta_k^{\mathrm{mat}}$ e escolha de $\beta_{\min}$ e $\rho_{\max}$.}
Substituindo a estimativa \eqref{eq:bound-Xdiff-4} em \eqref{eq:Delta-mat-1}, obtemos
\begin{align}
\Delta_k^{\mathrm{mat}}
&\le
\Gamma_1\,\|X_{k+1}-V_k\|_F^2
-
\theta\|X_k-V_k\|_F^2
+
\Gamma_0\Big(2A_1\eta_k^4\|\nabla f(x_k)\|^4 + 2\rho^2\|X_k-V_k\|_F^2\Big)
\nonumber\\[0.1cm]
&=
\Gamma_1\,\|X_{k+1}-V_k\|_F^2
+
\underbrace{\big(-\theta + 2\Gamma_0 \rho^2\big)}_{=:~\Gamma_2}\,
\|X_k-V_k\|_F^2
+
2\Gamma_0 A_1\eta_k^4\|\nabla f(x_k)\|^4.
\label{eq:Delta-mat-2}
\end{align}

Para controlar simultaneamente os coeficientes $\Gamma_1$ e $\Gamma_2$,
impomos, sem perda de generalidade, a relação $\theta+\varepsilon=1$.
Sob essa escolha, a validade da desigualdade de Lyapunov
\eqref{eq:lyapunov-descent} reduz-se a garantir que
$$
\Gamma_1 < 0
\qquad\text{e}\qquad
\Gamma_2 < 0.
$$

\medskip
\noindent\textbf{Escolha de $\beta_{\min}$.}
A expressão de $\Gamma_1$ no caso $\theta+\varepsilon=1$ torna-se
$$
\Gamma_1 = (1-\beta)^2 - (1-\theta)(1-\varepsilon)
           = (1-\beta)^2 - \theta(1-\theta).
$$
A função $\theta(1-\theta)$ atinge seu máximo no ponto $\theta=\tfrac{1}{2}$,
com valor $1/4$. Assim,
$$
\Gamma_1 < 0
\quad\Longleftrightarrow\quad
(1-\beta)^2 < \tfrac14
\quad\Longleftrightarrow\quad
\beta > \tfrac12.
$$
Portanto, qualquer parâmetro
$$
\beta \in (\beta_{\min},1),
\qquad
\beta_{\min} := \tfrac12,
$$
garante a existência de uma constante $\gamma_1>0$ tal que
\begin{equation}\label{eq:Gamma1-neg}
\Gamma_1 \le -\gamma_1 < 0.
\end{equation}

\medskip
\noindent\textbf{Escolha de $\rho_{\max}$.}
Pela definição de $\Gamma_0$ em \eqref{eq:Delta-mat-1}, e usando
$\theta+\varepsilon=1$, obtemos $\Gamma_0=\theta$. Assim,
$$
\Gamma_2 = -\theta + 2\theta\rho^2
          = \theta(2\rho^2 - 1).
$$
A condição $\Gamma_2<0$ equivale a
$$
2\rho^2 - 1 < 0
\quad\Longleftrightarrow\quad
\rho < \frac{1}{\sqrt{2}}.
$$
Logo, para qualquer
$$
\rho \in (0,\rho_{\max}),
\qquad
\rho_{\max}:=\frac{1}{\sqrt{2}},
$$
existe uma constante $\gamma_2>0$ tal que
\begin{equation}\label{eq:Gamma2-neg}
\Gamma_2 \le -\gamma_2 < 0.
\end{equation}

\medskip
Concluímos, portanto, que a análise de Lyapunov exige parâmetros de aceleração
restritos às faixas
$$
\beta \in (\beta_{\min},1),
\qquad
\rho \in (0,\rho_{\max}),
$$
com $\beta_{\min}=\tfrac12$ e
$\rho_{\max} = \tfrac{1}{\sqrt{2}}$, assegurando que tanto
$\Gamma_1$ quanto $\Gamma_2$ contribuam com termos dissipativos na
desigualdade de decréscimo \eqref{eq:lyapunov-descent}.

\medskip
\noindent\textbf{Passo 6: Combinação dos termos e escolha de $\kappa^*$.}
Com \eqref{eq:Gamma1-neg} e \eqref{eq:Gamma2-neg}, a desigualdade
\eqref{eq:Delta-mat-2} implica que, para $\rho\in(0,\rho_{\max})$ e
$\beta\in(\beta_{\min},1)$,
$$
\Delta_k^{\mathrm{mat}}
\le
-\gamma_1\|X_{k+1}-V_k\|_F^2
-\gamma_2\|X_k-V_k\|_F^2
+
2\Gamma_0 A_1\eta_k^4\|\nabla f(x_k)\|^4.
$$
Multiplicando por $\kappa>0$ e somando a \eqref{eq:suf-descent}, obtemos
\begin{align}
\mathcal{E}_{k+1}-\mathcal{E}_k
&\le
-c_1\|\nabla f(x_k)\|^2
-\kappa\gamma_1\|X_{k+1}-V_k\|_F^2
-\kappa\gamma_2\|X_k-V_k\|_F^2
+
2\kappa \Gamma_0 A_1\eta_k^4\|\nabla f(x_k)\|^4.
\label{eq:Delta-Ek-pre}
\end{align}

Como a sequência $(x_k)$ permanece em uma região compacta e o gradiente
é Lipschitz-contínuo, existe $G_*>0$ tal que
$\|\nabla f(x_k)\|\le G_*$ para todo $k$. Além disso, a busca linear
garante que $\eta_k\le\eta_{\max}$. Assim,
$$
\eta_k^4\|\nabla f(x_k)\|^4
\le
\eta_{\max}^4 G_*^2\,\|\nabla f(x_k)\|^2.
$$
Definindo
$$
C_* := 2\Gamma_0 A_1 \eta_{\max}^4 G_*^2,
$$
segue que
$$
2\kappa \Gamma_0 A_1\eta_k^4\|\nabla f(x_k)\|^4
\le
\kappa C_* \|\nabla f(x_k)\|^2.
$$

Escolhemos, então, $\kappa>0$ suficientemente pequeno para que
$$
\kappa C_* \le \frac{c_1}{2}.
$$
Note que tal escolha sempre existe, e definimos
$$
\kappa^* := \frac{c_1}{2C_*},
$$
de modo que a condição acima é satisfeita para qualquer
$\kappa\in(0,\kappa^*)$.

Sob essa escolha, a desigualdade \eqref{eq:Delta-Ek-pre} reduz-se a
\begin{equation}\label{eq:Delta-Ek-final}
\mathcal{E}_{k+1}-\mathcal{E}_k
\;\le\;
-\frac{c_1}{2}\|\nabla f(x_k)\|^2
-\kappa\gamma_1\|X_{k+1}-V_k\|_F^2.
\end{equation}
Definindo $c_2 := \kappa\gamma_1>0$, obtemos exatamente a forma
\eqref{eq:Lyap-target} com $c_1$ substituído por $c_1/2$, o que não
altera a natureza do resultado.

Em particular, $\{\mathcal{E}_k\}$ é não crescente para qualquer
$\kappa\in(0,\kappa^*)$, o que garante estabilidade no sentido de
Lyapunov e implica que $\|X_k - V_k\|_F \to 0$ ao longo das iterações.

\end{proof}

\paragraph{Interpretação.}
O Teorema~\ref{thm:Lyapunov} estabelece uma propriedade de estabilidade no sentido de Lyapunov para o esquema acelerado quasi-Newton. Em particular, a condição de decréscimo~\eqref{eq:lyapunov-descent} garante que a sequência de energia $\{\mathcal{E}_k\}$ é não crescente, controlando simultaneamente a evolução da variável primal $x_k$ e das sequências matriciais $X_k$ e $V_k$.

O termo dissipativo $\|X_{k+1}-V_k\|_F^2$ promove o alinhamento entre a atualização quasi-Newton e o estado inercial, implicando que $X_k$ e $V_k$ tendem a coincidir assintoticamente. Esse mecanismo atua como amortecimento da dinâmica acelerada, prevenindo a amplificação de oscilações induzidas pelo termo de inércia.

Como consequência, o método preserva a positividade definida das matrizes, mantém cotas espectrais uniformes e converge para um regime estacionário caracterizado por $\nabla f(x_k)\to 0$ e $X_k \simeq V_k$, sem comprometer as propriedades estruturais da atualização BFGS.

\subsection{Componente Estocástico na Direção de Busca}
\label{sec:stochastic_bfgs}

A formulação proposta incorpora aleatoriedade controlada diretamente na direção de busca do método quasi-Newton. Diferentemente de abordagens que introduzem estocasticidade na estimativa do gradiente ou na atualização da Hessiana, o ruído é aplicado ao vetor de deslocamento, preservando a estrutura determinística da atualização de $X_k$ e as propriedades locais de convergência do esquema BFGS.

A motivação dessa escolha é aumentar a capacidade exploratória do método e reduzir a probabilidade de estagnação em mínimos locais ou regiões de baixa curvatura. Resultados recentes indicam que perturbações probabilísticas moderadas podem melhorar o comportamento global de métodos quasi-Newton sem degradar seu desempenho local \cite{shi2022noise, guo2023overview, amos2020algorithm, peng2025finding}.

Para preservar a natureza descendente da direção de busca, o ruído é projetado de modo a eliminar sua componente paralela ao gradiente $g_k = \nabla f(x_k)$. Seja $\epsilon \sim \mathcal{N}(0, I)$; define-se
\begin{equation}
\xi_k = \epsilon - \frac{\epsilon^\top g_k}{g_k^\top g_k} \, g_k,
\label{eq:projected_noise}
\end{equation}
de modo que $g_k^\top \xi_k = 0$. A direção estocástica é então dada por
\begin{equation}
\tilde{s}_k = s_k + \tau_k \xi_k,
\label{eq:stochastic_direction_projected}
\end{equation}
onde $s_k = -X_k \nabla f(x_k)$ e $\tau_k > 0$ controla a intensidade da perturbação.

A ortogonalidade de $\xi_k$ garante que
$$
g_k^\top \tilde{s}_k = g_k^\top s_k,
$$
preservando a condição de descida. Além disso, como $\mathbb{E}[\xi_k] = 0$, tem-se $\mathbb{E}[\tilde{s}_k] = s_k$, de modo que o comportamento médio do método coincide com o do esquema determinístico.

A magnitude do ruído é controlada por um fator de temperatura $\tau_k$ que decai ao longo das iterações, por exemplo,
\begin{equation}
\tau_k = \frac{\tau_0}{1 + \lambda k}, \qquad \lambda > 0,
\label{eq:temperature_decay}
\end{equation}
o que permite uma transição progressiva entre uma fase exploratória inicial e um regime de refinamento local. Esse mecanismo é consistente com estratégias de \emph{cooling} utilizadas em métodos estocásticos e garante que a variância da perturbação tenda a zero, preservando a dinâmica assintótica do método determinístico \cite{guo2023overview}.

O ponto iterado é atualizado por
$$
x_{k+1} = x_k + \eta_k \tilde{s}_k,
$$
com $\eta_k$ obtido por uma busca linear adequada. Nesse contexto, o termo estocástico introduz variações tangenciais às superfícies de nível da função objetivo, aumentando a diversidade direcional sem comprometer o sentido global de descida.

Em síntese, o método preserva o núcleo determinístico do BFGS acelerado, ao mesmo tempo em que incorpora um ruído projetado e suavemente decrescente na direção de busca. Essa modificação amplia a capacidade exploratória do algoritmo e melhora sua robustez em cenários não convexos, mantendo coerência com as propriedades estruturais estabelecidas na análise anterior.

%A seguir, apresenta-se o algoritmo correspondente à formulação proposta.

\begin{algorithm}%[H]
\caption{BFGS Acelerado com Componente Estocástico na Direção de Busca}
\label{alg:bfgs_ac_stoc}
\begin{algorithmic}[1]
\REQUIRE $x_0$, $H_0 = I$, $U_0 = I$, $\tau_0$, $\lambda$, $\rho$, $\beta$, $\eta$, $\sigma$
\STATE \textbf{Avaliar} $f(x_0)$ e $g_0 = \nabla f(x_0)$
\FOR{$k = 0,1,2,\dots$ \textbf{até convergência}}
    \STATE $d_k \gets -H_k g_k$ \COMMENT{Direção determinística de descida}
    \STATE \textbf{Gerar} ruído $\varepsilon \sim \mathcal{N}(0,I)$
    \STATE \textbf{Projetar} $\varepsilon$ ortogonalmente ao gradiente:
        $$
        \xi_k = \varepsilon - \frac{\varepsilon^\top g_k}{g_k^\top g_k}\, g_k
        $$
    \STATE \textbf{Calcular temperatura}: $\tau_k = \tau_0 / (1 + \lambda k)$
    \STATE \textbf{Direção estocástica}: $d_k \gets d_k + \tau_k \xi_k$
    \IF{$g_k^\top d_k > 0$}
        \STATE $d_k \gets -H_k g_k$ \COMMENT{Correção para manter direção de descida}
    \ENDIF
    \STATE \textbf{Determinar} $\eta_k = \eta^m$ via busca linear de Armijo, com $m$ mínimo tal que
        $$
        f(x_k + \eta_k d_k) \le f(x_k) + \sigma \eta_k g_k^\top d_k
        $$
    \STATE \textbf{Atualizar ponto}: $x_{k+1} = x_k + \eta_k d_k$
    \STATE \textbf{Calcular} $g_{k+1} = \nabla f(x_{k+1})$
    \STATE \textbf{Definir} $s_k = x_{k+1} - x_k$, \quad $y_k = g_{k+1} - g_k$
    \IF{$y_k^\top s_k > 0$}
        \STATE $Y_k \gets (1-\rho)H_k + \rho V_k$
        \STATE $\phi_k \gets 1/(y_k^\top s_k)$
        \STATE $W_k \gets I - \phi_k s_k y_k^\top$
        \STATE $H_{k+1} \gets W_k Y_k W_k^\top + \phi_k\, s_k s_k^\top$
        \STATE $V_{k+1} \gets (1-\beta)V_k + \beta H_{k+1}$
    \ELSE
        \STATE $H_{k+1} \gets H_k$, \quad $V_{k+1} \gets V_k$
    \ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}

O Algoritmo~\ref{alg:bfgs_ac_stoc} sintetiza a formulação proposta, combinando a atualização quasi-Newton acelerada com uma perturbação estocástica projetada na direção de busca. O decaimento de $\tau_k$ induz uma transição gradual entre uma fase exploratória inicial e um regime de refinamento local, enquanto os parâmetros $\rho$ e $\beta$ são escolhidos dentro das faixas $(0,\rho_{\max})$ e $(\beta_{\min},1)$, conforme estabelecido pela análise de estabilidade, garantindo a preservação das propriedades estruturais no cone $\mathbb{S}_{++}^n$.

A formulação apresentada define uma extensão acelerada e estocástica do método BFGS, cuja análise teórica assegura estabilidade e coerência geométrica. Resta avaliar empiricamente o impacto dessas modificações em termos de qualidade das soluções e eficiência computacional.

Para esse fim, realizamos uma comparação entre o BFGS clássico, o BFGS acelerado e a versão acelerada com componente estocástica em um conjunto de problemas many-objective escalarizados. Essa análise permite isolar o efeito de cada mecanismo proposto, avaliando sua contribuição para o desempenho do método em cenários de maior complexidade.

\section{Comparação entre as versões pura, acelerada e acelerada-estocástica do método BFGS}


==> bfgs_gama.tex <==
\section{Método BFGS}

Nos métodos quasi-Newton, o BFGS constrói iterativamente uma aproximação $X_k \approx H_k^{-1}$ da inversa da Hessiana, usando apenas informação de primeira ordem. A cada iteração, $X_k$ é atualizada de modo a satisfazer a \emph{condição de secante}, que impõe coerência entre o deslocamento nas variáveis e a variação do gradiente.

Sejam
$$
s_k = x_{k+1} - x_k, \qquad \zeta_k = \nabla f(x_{k+1}) - \nabla f(x_k),
$$
respectivamente, o passo na variável de decisão e a variação do gradiente entre as iterações $k$ e $k+1$. A condição de secante exige que a nova aproximação satisfaça $X_{k+1}\,\zeta_k = s_k$, isto é, que a inversa aproximada mapeie a diferença de gradientes $\zeta_k$ no deslocamento real $s_k$, impondo-se ainda a simetria $X_{k+1} = X_{k+1}^\top$.

A atualização resulta do problema de mínima correção em norma de Frobenius:
\begin{equation}
X_{k+1} = \arg\min_X \|X - X_k\|_F^2 
\quad \text{s.a.} \quad X \zeta_k = s_k,\; X = X^\top,
\label{eq:bfgs_opt}
\end{equation}
cuja solução fechada é
\begin{equation}
X_{k+1} = \frac{s_k s_k^\top}{s_k^\top \zeta_k}
+ \left(I - \frac{s_k \zeta_k^\top}{s_k^\top \zeta_k}\right)
X_k
\left(I - \frac{\zeta_k s_k^\top}{s_k^\top \zeta_k}\right),
\label{eq:bfgs_closed_form}
\end{equation}
com $\|A\|_F=\sqrt{\operatorname{Tr}(A^\top A)}$. O primeiro termo garante o atendimento da condição de secante; o segundo ajusta $X_k$ de forma simétrica e mínima em norma. A iteração preserva simetria e definição positiva sempre que $\zeta_k^\top s_k > 0$ — condição satisfeita sob convexidade local ou controle do tamanho do passo.

Geometricamente, \eqref{eq:bfgs_opt} é uma \emph{projeção} de $X_k$ sobre o conjunto das matrizes que satisfazem a condição de secante. Essa leitura permite aplicar à sequência $\{X_k\}$ as técnicas de aceleração de \cite{nesterov1983method}, adaptadas ao domínio matricial — ideia que se desenvolve nas seções seguintes.


\subsection{Método Acelerado de Nesterov}
\label{sec:nesterov_intro}

O método do gradiente atualiza
\begin{equation}
x_{k+1} = x_k - \alpha \nabla f(x_k),
\label{eq:gradiente_puro}
\end{equation}
e, sob convexidade e gradiente Lipschitz-contínuo, converge a taxa $O(1/k)$ \cite{bubeck2015convex}; em problemas mal condicionados, porém, tende a oscilar e a perder eficiência. Para mitigar isso, \cite{polyak1964some} introduziu o termo inercial (\emph{heavy-ball method}),
\begin{align}
v_{k+1} &= \mu v_k - \alpha \nabla f(x_k), \label{eq:momentum_v}\\
x_{k+1} &= x_k + v_{k+1}, \label{eq:momentum_x}
\end{align}
em que $\mu \in [0,1)$ pondera o histórico recente: $\mu = 0$ recupera o gradiente puro~\eqref{eq:gradiente_puro} e valores maiores acumulam impulso ao longo das direções de menor curvatura, acelerando na prática, embora sem garantia da taxa ótima.

\cite{nesterov1983method} obteve a taxa assintoticamente ótima $O(1/k^2)$ avaliando o gradiente em um ponto \emph{extrapolado}, e não em $x_k$:
\begin{align}
y_k &= x_k + \mu (x_k - x_{k-1}), \label{eq:nesterov_y}\\
x_{k+1} &= y_k - \alpha \nabla f(y_k). \label{eq:nesterov_x}
\end{align}
A diferença essencial em relação a Polyak é que o gradiente é avaliado no ponto extrapolado $y_k$; é isso que permite provar a taxa $O(1/k^2)$, ótima entre os métodos de primeira ordem \cite{bubeck2015convex, su2016differential}. Para fins de análise e implementação estável, é comum reescrever o método com uma terceira sequência $\{v_k\}$, que atua como memória inercial suavizada:
\begin{align}
y_k &= (1 - \mu)\, x_k + \mu\, v_k, \label{eq:nesterov_y_alt}\\
x_{k+1} &= y_k - \alpha \nabla f(y_k), \label{eq:nesterov_x_alt}\\
v_{k+1} &= (1 - \mu)\, v_k + \mu\, x_{k+1}. \label{eq:nesterov_v}
\end{align}
Os três papéis — extrapolação ($y_k$), descida ($x_{k+1}$) e atualização inercial ($v_{k+1}$) — constituem a expressão algorítmica da aceleração de Nesterov.

A escolha de $\alpha$ e $\mu$ governa estabilidade e velocidade. Para $f$ convexa com gradiente $L$-Lipschitz, $\|\nabla f(x)-\nabla f(y)\|\le L\|x-y\|$, e $\mu_f$-fortemente convexa,
$$
f(y) \ge f(x) + \nabla f(x)^\top (y - x) + \tfrac{\mu_f}{2}\|y - x\|^2,
$$
as constantes $L$ e $\mu_f$ limitam, respectivamente, a máxima e a mínima curvatura local; no caso quadrático $f(x)=\tfrac12 x^\top A x - b^\top x + c$ com $A$ SPD, valem $L=\lambda_{\max}(A)$ e $\mu_f=\lambda_{\min}(A)$. No cenário clássico adota-se $\alpha = 1/L$ e
$$
\mu = \frac{\sqrt{L} - \sqrt{\mu_f}}{\sqrt{L} + \sqrt{\mu_f}},
$$
o que produz convergência linear $(1 - \sqrt{\mu_f/L})^k$; no caso meramente convexo ($\mu_f = 0$), sequências $\mu_k \approx 1 - O(1/k)$ recuperam a taxa $O(1/k^2)$ \cite{bubeck2015convex, nesterov1983method}.

Quando $L$ e $\mu_f$ são desconhecidos, essa calibração teórica torna-se inviável e a escolha passa a ser empírica. A análise de \cite{lessard2016analysis} mostra que a convergência pode falhar quando $L/\mu_f$ é grande; na prática, valores de $\mu$ entre $0.8$ e $0.95$ mantêm estabilidade mesmo em problemas mal condicionados, enquanto \cite{sutskever2013importance} e \cite{liu2020improved} relatam ganhos com cronogramas crescentes de $\mu$ (de $\approx 0.9$ até $\mu_{\max}\in\{0.99,\,0.995,\,0.999\}$). O passo $\alpha$, limitado por $1/L$ na teoria \cite{bubeck2015convex, nesterov2013introductory}, é tipicamente reduzido ou adaptado ao longo das iterações \cite{ruder2016overview, peng2025finding}. Em síntese, $\alpha$ controla a magnitude da descida e $\mu$ a persistência inercial; fora do regime clássico, o par $(\alpha,\,\mu)$ é ajustado de forma empírica, com aumentos de momentum compensados por passos mais conservadores.


\subsection{Aceleração de Nesterov com parâmetros desacoplados}
\label{sec:nesterov_desacoplado}

Na forma \eqref{eq:nesterov_y_alt}--\eqref{eq:nesterov_v}, um único parâmetro $\mu$ desempenha três papéis simultâneos: pondera a extrapolação em $y_k$, a memória inercial em $v_{k+1}$ e, implicitamente, o gradiente. Para expor essa rigidez, separamos primeiro os pesos da extrapolação ($\rho$) e da atualização inercial ($\beta$):
\begin{align}
y_k &= (1-\rho)\,x_k + \rho\,v_k, \label{eq:dec_y}\\
x_{k+1} &= y_k - \alpha\,\nabla f(y_k), \label{eq:dec_x}\\
v_{k+1} &= (1-\beta)\,v_k + \beta\,x_{k+1}. \label{eq:dec_v}
\end{align}
Substituindo a descida \eqref{eq:dec_x} na atualização inercial \eqref{eq:dec_v},
$$
v_{k+1} = (1-\beta)\,v_k + \beta\,y_k - \beta\alpha\,\nabla f(y_k),
$$
o gradiente surge com coeficiente $\beta\alpha$, isto é, \emph{amarrado} ao mesmo $\beta$ que pondera $v_k$ e $y_k$. Essa rigidez é removida atribuindo ao gradiente um coeficiente próprio $\gamma$:
\begin{equation}
v_{k+1} = (1-\beta)\,v_k + \beta\,y_k - \gamma\alpha\,\nabla f(y_k).
\label{eq:nesterov_gamma}
\end{equation}
Como $-\alpha\nabla f(y_k) = x_{k+1}-y_k$ por \eqref{eq:dec_x}, a expressão \eqref{eq:nesterov_gamma} equivale à \emph{forma de resíduo}
\begin{equation}
v_{k+1} = (1-\beta)\,v_k + \beta\,y_k + \gamma\,(x_{k+1}-y_k)
        = (1-\beta)\,v_k + (\beta-\gamma)\,y_k + \gamma\,x_{k+1}.
\label{eq:residuo}
\end{equation}
A escolha $\gamma=\beta$ recupera exatamente a forma original \eqref{eq:dec_v}. Portanto, $\gamma$ é um grau de liberdade \emph{adicional} que nada altera no caso exato e só passa a importar quando $x_{k+1}-y_k$ deixa de ser o passo de gradiente ideal $-\alpha\nabla f(y_k)$.

\paragraph{Conexão com o BFGS.} É precisamente esse o caso ao acelerar a sequência de matrizes $\{X_k\}$ do BFGS: o resíduo $X_{k+1}-Y_k = -H_k\,\nabla f(Y_k)$ é o \emph{passo efetivamente dado pelo método}, e não o passo de gradiente puro. A forma de resíduo \eqref{eq:residuo} generaliza-se então de modo natural ao domínio matricial:
\begin{align}
Y_k &= (1-\rho)\,X_k + \rho\,V_k, \\
X_{k+1} &= \mathrm{BFGS}(Y_k), \\
V_{k+1} &= (1-\beta)\,V_k + (\beta-\gamma)\,Y_k + \gamma\,X_{k+1},
\end{align}
onde $\mathrm{BFGS}(Y_k)$ denota a atualização \eqref{eq:bfgs_closed_form} aplicada a $Y_k$. O parâmetro $\gamma$ reescala o deslocamento aproximado dentro da memória inercial: amortece-o quando a estimativa BFGS ainda é ruidosa (início da execução) e amplifica-o quando se deseja incorporá-lo de forma mais agressiva.

\paragraph{Preservação das propriedades matriciais.} Os três coeficientes de \eqref{eq:residuo} somam~$1$ para qualquer $\gamma$, pois $(1-\beta)+(\beta-\gamma)+\gamma = 1$. Isso garante a consistência baricêntrica: se $X_k=V_k=Y_k=M$, então $V_{k+1}=M$. Como o cone das matrizes simétricas definidas positivas (SPD) é convexo, combinações convexas de matrizes SPD permanecem SPD; basta, então, que os coeficientes sejam não-negativos:
$$
0 \le \gamma \le \beta \le 1, \qquad 0 \le \rho \le 1.
$$
Nessa faixa, $Y_k$ e $V_{k+1}$ são automaticamente SPD. Fora dela --- em particular para $\gamma>\beta$, que torna $\beta-\gamma<0$ --- o termo $Y_k$ entra com peso negativo e a definição positiva deixa de ser assegurada pelo argumento de convexidade, exigindo verificação caso a caso. Esse é o \emph{trade-off} introduzido por $\gamma$: maior liberdade de correção em troca da preservação automática do cone. Cabe ressaltar que a combinação convexa euclidiana preserva o cone SPD, mas não corresponde à média geodésica natural nesse cone; se a propriedade a preservar for mais restritiva (determinante ou posto fixos), combinações lineares no espaço ambiente saem do conjunto e seria necessária uma interpolação riemanniana. Para SPD pura, contudo, a forma acima é suficiente.

==> convergence.tex <==
\section{Convergence Analysis}
\label{sec:convergence}

In this section, we analyze the convergence properties of the proposed Accelerated Geometry BFGS (AG-BFGS) algorithm. The analysis establishes conditions under which the method retains the stability and convergence guarantees of classical BFGS, while incorporating inertial momentum-like effects in the Hessian updates. In particular, we aim to characterize admissible regions for $(\rho,\beta,\gamma)$ that ensure both the dynamical stability of the accelerated system and the preservation of the structural properties of the quasi-Newton approximations.

\subsection{Iterative Analysis and Preservation of Structural Properties}
\label{subsec:analise_iterativa}

To establish the structural and stability properties of the proposed Accelerated Geometry BFGS (AG-BFGS) scheme described in Algorithm \ref{alg:bfgs_ac_stoc} (Section \ref{sec:accelerated}), we present a set of auxiliary results. These results provide sufficient conditions for the preservation of positive definiteness and for the monotonic decrease of a Lyapunov functional, $\mathcal{E}_k$, associated with the sequences $\{X_k, V_k, Y_k, x_k\}$.

A central requirement is the boundedness of the eigenvalues of the metric sequence $X_k,~ Y_k,~V_k$. In particular, it is necessary to establish the existence of constants $0< m\leq M$ such that  $mI \preceq X_k, Y_k, V_k \preceq MI$ for some $0 < m \le M$. These bounds ensure that the metric approximation remains uniformly positive definite and well conditioned, preventing instability of the search directions and potential divergence caused by the inertial Hessian dynamics.

\begin{lemma}[Boundedness of Eingenvalues]
\label{lem:convex_spd_bounds}
Let $X_k, V_k \in \mathbb{S}_{++}^n$ satisfy $mI \preceq X_k, V_k \preceq MI$ for some $0 < m \le M$. Then, for any $\rho \in (0,1)$,
$$
Y := (1-\rho)X_k + \rho V_k \in \mathbb{S}_{++}^n
\quad\text{and}\quad
mI \preceq Y \preceq MI.
$$

\begin{proof}
For any $z \neq 0$, we have that
$$
z^\top Y z = (1-\rho) z^\top X_k z + \rho z^\top V_k z > 0.
$$
Moreover,
$$
\lambda_{\min}(Y) \ge (1-\rho)\lambda_{\min}(X_k) + \rho\lambda_{\min}(V_k) \ge m,
$$
and
$$
\lambda_{\max}(Y) \le (1-\rho)\lambda_{\max}(X_k) + \rho\lambda_{\max}(V_k) \le M,
$$
which concludes the proof.

\end{proof}
\end{lemma}

An entirely analogous argument applies to the auxiliary variable $V_k$, whose update is also given by a convex combination of matrices in $\mathbb{S}_{++}^n$. Consequently, both $Y_k$ and $V_{k+1}$ preserve positive definiteness by construction, ensuring that all matrix variables remain in the cone $\mathbb{S}_{++}^n$ throughout the iterations.

%Ensuring that the intermediate variables $Y_k$ and $V_k$ remain in $\mathbb{S}_{++}^n$ is essential for the subsequent BFGS step to preserve the positive definiteness of the curvature approximation. Once this convexity property is guaranteed, the classical BFGS update can be safely applied to $Y_k$, as stated in Lemma~\ref{lem:bfgs_spd}. 
Under the curvature condition $s_k^\top \zeta_k > 0$, the BFGS transformation preserves positive definiteness, thereby completing the structural stability cycle between extrapolation and quasi-Newton update.


\begin{lemma}[Positive Definiteness]
\label{lem:bfgs_spd}
Let $Y_k \in \mathbb{S}_{++}^n$ and $s, \zeta \in \mathbb{R}^n$ be such that $\zeta^\top s > 0$. The classical BFGS update
$$
X_{k+1}
= \Big(I-\tfrac{s \zeta^\top}{\zeta^\top s}\Big)\,Y_k\,\Big(I-\tfrac{\zeta s^\top}{\zeta^\top s}\Big)
  + \tfrac{s s^\top}{\zeta^\top s}
$$
satisfies $X_{k+1} \in \mathbb{S}_{++}^n$.

\begin{proof}
Let $\phi := \frac{1}{\zeta^\top s} > 0$ and define $M := I - \phi\,\zeta s^\top$. 

Then $M^\top = I - \phi\, s\zeta^\top$, and the update can be written as
\begin{equation} \begin{array}{lcl}
X_{k+1} &
=& \big(I-\phi\, s\zeta^\top\big)\,Y_k\,\big(I-\phi\,\zeta s^\top\big) + \phi\,ss^\top  \\
&=& M^\top Y_k M + \phi\,ss^\top .
\end{array}
\nonumber
\end{equation}
For any $z \neq 0$, we have that
$$
z^\top X_{k+1} z = (Mz)^\top Y_k (Mz) + \phi (s^\top z)^2.
$$
If $Mz \neq 0$, the first term is strictly positive since $Y_k \succ 0$. If $Mz = 0$, then $z = \phi \zeta (s^\top z)$, which implies $s^\top z \neq 0$, and hence the second term is strictly positive. Therefore, $z^\top X_{k+1} z > 0$ for all $z \neq 0$, proving that $X_{k+1} \in \mathbb{S}_{++}^n$. Symmetry follows from the symmetry of $Y_k$ and the update structure.
\end{proof}
\end{lemma}

The following theorem provides the main theoretical foundation of the proposed method. It establishes that, under standard smoothness assumptions and sufficiently small step sizes $\eta$, there exists a Lyapunov function $\mathcal{E}_k$ that decreases monotonically throughout the iterations. This function combines the objective value with a consistency term between $X_k$ and $V_k$, capturing both the optimization progress and the stability of the matrix sequence. Moreover, the proof shows that this descent property only requires that, choosing $\rho \in [0,1)$,  the acceleration parameters $\beta$ and $\gamma$ be in suitable subintervals. 

\begin{theorem}[Numerical Stability]
\label{thm:Lyapunov}
Let $f:\mathbb{R}^n\to\mathbb{R}$ be $C^1$ with $L$-Lipschitz gradient on a compact set that contains the iterates. Consider the updates. Consider
\begin{align*}
x_{k+1} &= x_k - \eta X_k \nabla f(x_k),\\
Y_k &= (1-\rho)X_k + \rho V_k, \\
%\qquad \rho\in(0,\rho_{\max}),\\
X_{k+1} &= \Phi_{\mathrm{BFGS}}(Y_k;\, s_k,\zeta_k),\\
V_{k+1} &= (1-\beta)V_k + (\beta-\gamma) Y_k + \gamma X_{k+1}
%,\qquad \beta\in(\beta_{\min},1),
\end{align*}
with $s_k:= x_{k+1} - x_k$, and $\zeta_k:= \nabla{f}(x_{k+1}) - \nabla{f}(x_k)$. Assume that $0< \rho< 1$, $0 < \gamma<1$ and that $\beta$ is chosen such that 

\begin{equation}
2(1-\beta)^2(1-\rho)^2<1. \footnote{Observe that, in a conservative case in which $0< \beta <1$, this condition holds if 
$
\max\left\{
0,\,
1-\frac{1}{\sqrt{2}(1-\rho)}
\right\}
<
\beta
<
1.$}
\label{eq:cond_param_teo}
\end{equation}

Assume $s_k^\top \zeta_k > 0$ for all $k$, and that there exist $0 < m_* \le M_* < \infty$ such that
\begin{equation}
m_* I \preceq X_k, V_k, Y_k \preceq M_* I, ~~~ \forall k.
\label{eq:teo_cotas}
\end{equation}

Suppose further that the step sizes satisfy
\begin{equation}
f(x_{k+1}) \le f(x_k) - c_1 \|\nabla f(x_k)\|^2 \qquad \forall k.
\label{eq:teo_decrescimo}
\end{equation}
for some $c_1 > 0$ \footnote{ This $c_1$ can be obtained using an appropriate line search such as Armijo line search.}.


For $\kappa>0$, define
\begin{equation}
\mathcal{E}_k := f(x_k)-f^* + \kappa\|X_k - V_k\|_F^2.
\label{eq:teo_lyapunov}
\end{equation}


Then there exist $\kappa^*>0$ and $c_2>0$ such that, for any $\kappa \in (0,\kappa^*)$,
\begin{equation}
\mathcal{E}_{k+1}
\leq
\mathcal{E}_k
-
\frac{c_1}{2}\|\nabla f(x_k)\|^2
-
c_2\|X_k-V_k\|_F^2,
\qquad \forall k.
\label{eq:teo_estabilidade}
\end{equation}

Observe that $\kappa^*>0$ and $c_2>0$ depend only on $m_*,~ M_*,~ \rho_{max},~ \beta_{min}$.
In particular, $\{\mathcal{E}_k\}$ is non-increasing, implying Lyapunov stability and $\|X_k - V_k\|_F \to 0$.
\end{theorem}


\begin{proof}
For $\kappa>0$, define the Lyapunov function
$$
\mathcal{E}_k \;:=\; f(x_k)-f^* \;+\; \kappa\|X_k - V_k\|_F^2.
$$
Our goal is to show that, for suitable choices of $\rho,~\beta,$ and $\gamma$ and sufficiently small $\kappa>0$, there exist constants $c_1,c_2>0$ such that
\begin{equation}\label{eq:Lyap-target}
\mathcal{E}_{k+1}-\mathcal{E}_k
\;\le\;
-
\frac{c_1}{2}\|\nabla f(x_k)\|^2
-
c_2\|X_{k+1}-V_k\|_F^2,
\qquad\text{for all }k.
\end{equation}

\medskip
\noindent\textbf{Step 1: Decompose $\mathcal{E}_k$.}
From the definition, we have the
$$
\mathcal{E}_{k+1}-\mathcal{E}_k
=
\underbrace{f(x_{k+1})-f(x_k)}_{\text{Term I}}
+
\kappa\underbrace{\Big(\|X_{k+1}-V_{k+1}\|_F^2-\|X_k-V_k\|_F^2\Big)}_{ \text{Term II} (\Delta_k^{\mathrm{mat}})}.
$$
By the sufficient decrease condition
$$
\underbrace{f(x_{k+1})-f(x_k)}_{\text{Term I}} \le  - c_1 \|\nabla f(x_k)\|^2,
$$


%By the $L$-Lipschitz continuity of the gradient, we also have that
%$$
%f(x_{k+1}) \le f(x_k) - \eta_k \nabla f(x_k)^\top X_k \nabla f(x_k)
%+ \tfrac{L}{2}\eta_k^2 \|X_k\nabla f(x_k)\|^2.
%$$
%Using $m_\ast I \preceq X_k \preceq M_\ast I$, we obtain
%$$
%\underbrace{f(x_{k+1})-f(x_k)}_{\text{Term I}} \le  - c_1 \|\nabla f(x_k)\|^2,
%$$

\noindent with $c_1 = \eta_k m_\ast - \tfrac{L}{2}\eta_k^2 M_\ast^2 > 0$ whenever $\eta_k \le 1/(M_\ast L)$. %, consistent with Equation~ \eqref{eq:suf-descent}.
Therefore
\begin{equation}
E_{k+1}-E_k
\leq
-c_1\|\nabla f(x_k)\|^2
+
\kappa\Delta_k^{\mathrm{mat}},
\label{eq:Ek_delta}
\end{equation}
and it remains to control Term II ($\Delta_k^{\mathrm{mat}}$).

\medskip
\noindent\textbf{Step 2: Rewrite term II.}

\noindent Consider 
\begin{equation}
V_{k+1}=(1-\beta)V_k+\beta Y_k-\gamma(Y_k-X_{k+1}),
\label{eq:Vk_nova}
\end{equation}
as defined in Equations (\ref{eq:acc_bfgs}).

\noindent Define
\begin{equation}
D_k:=X_k-V_k,
\qquad
R_k:=X_{k+1}-Y_k,
\label{eq:Dk_Rk}
\end{equation}
and using Equation (\ref{eq:Vk_nova}), we have
\begin{align}
X_{k+1}-V_{k+1}
&=
(1-\beta)(X_{k+1}-V_k)
+
(\gamma-\beta)(Y_k-X_{k+1}).
\label{eq:XmenosV_reorg}
\end{align}
With $$Y_k=(1-\rho)X_k+\rho V_k,$$
we obtain
$$
Y_{k}-V_{k} = (1-\rho)(X_k-V_k) = (1-\rho)D_k.
$$
By definition of $R_k$, we have 

\begin{equation}
X_{k+1}-V_k
=
R_k+(1-\rho)D_k.
\label{eq:XmenosVk}
\end{equation}

\noindent Substituting \eqref{eq:XmenosVk} in \eqref{eq:XmenosV_reorg} we obtain
\begin{align}
X_{k+1}-V_{k+1}
&=
(1-\beta)\left[R_k+(1-\rho)D_k\right]
-(\gamma-\beta)R_k \nonumber\\
&=
(1-\beta)(1-\rho)D_k
+
(1-\gamma)R_k.
\label{eq:XmenosV_final}
\end{align}

\medskip
\noindent\textbf{Step 3: Estimate term II ($\Delta_k^{\mathrm{mat}}$).}

\noindent From \eqref{eq:XmenosV_final},
\begin{equation}
\|X_{k+1}-V_{k+1}\|_F^2=\left\|(1-\beta)(1-\rho)D_k+(1-\gamma)R_k\right\|_F^2.
\end{equation}

\noindent Using the matrix Young inequality,
$$
\|A+B\|_F^2
\leq
(1+\alpha)\|A\|_F^2
+
\left(1+\frac{1}{\alpha}\right)\|B\|_F^2,
$$
taking $A=(1-\beta)(1-\rho)D_k$, $B=(1-\gamma)R_k,$ and choosing $\alpha=1$, we obtain

\begin{equation}
\|X_{k+1}-V_{k+1}\|_F^2\leq2(1-\beta)^2(1-\rho)^2\|D_k\|_F^2+
2(1-\gamma)^2\|R_k\|_F^2.
\label{eq:young_final}
\end{equation}

\noindent Since $\|D_k\|_F^2=\|X_k-V_k\|_F^2$, it follows that
\begin{align}
\Delta_k^{\mathrm{mat}} &= \|X_{k+1}-V_{k+1}\|_F^2
-
\|X_k-V_k\|_F^2 \\
&\leq
\left[
2(1-\beta)^2(1-\rho)^2-1
\right]\|D_k\|_F^2+
2(1-\gamma)^2\|R_k\|_F^2.
\label{eq:delta_mat_bound}
\end{align}



\medskip
\noindent\textbf{Step 4: Bounds for $R_k$.}



\noindent By the quasi-Newton estimate applied to the BFGS transformation at $Y_k$, there exists a constant $A_1>0$ such that
\begin{equation}
\|R_k\|_F^2=\|X_{k+1}-Y_k\|_F^2\leq
A_1\eta_k^4\|\nabla f(x_k)\|^4.
\label{eq:Rk_bound}
\end{equation}

\noindent Changing \eqref{eq:Rk_bound} with \eqref{eq:delta_mat_bound}, we obtain the following.
\begin{align}
\Delta_k^{\mathrm{mat}}
&\leq
\left[
2(1-\beta)^2(1-\rho)^2-1
\right]\|D_k\|_F^2
\nonumber\\
&\quad+
2A_1(1-\gamma)^2
\eta_k^4\|\nabla f(x_k)\|^4.
\label{eq:delta_mat_final}
\end{align}





\medskip
\noindent\textbf{Step 5: Bounds for the parameters.}


In order for the coefficient of $||D_k||_F^2$ to be dissipative, we impose

\begin{equation}
2(1-\beta)^2(1-\rho)^2<1.
\label{eq:cond_beta_rho}
\end{equation}
Since $0<\rho<1$ and $0<\beta<1$, %it follows that $1-\rho>0$ and $1-\beta>0$. Therefore, 
\eqref{eq:cond_beta_rho} is equivalent to

\begin{equation}
\beta>1-\frac{1}{\sqrt{2}(1-\rho)}.
\label{eq:beta_cond}
\end{equation}

\noindent Consequently, choosing $0<\rho<1,$, a sufficient admissible region is given by

\begin{equation}
\max\left\{
0,\,
1-\frac{1}{\sqrt{2}(1-\rho)}
\right\}
<
\beta
<
1,
\qquad
0<\gamma\leq 1.
\label{eq:regiao_admissivel}
\end{equation}


\noindent Within this region, there exists a constant $\omega>0$ such that

\begin{equation}
1-2(1-\beta)^2(1-\rho)^2
\geq
\omega.
\label{eq:omega_def}
\end{equation}
Therefore, from \eqref{eq:delta_mat_final}, we obtain

\begin{equation}
\Delta_k^{\mathrm{mat}}
\leq
-\omega||D_k||_F^2
+
2A_1(1-\gamma)^2
\eta_k^4||\nabla f(x_k)||^4.
\label{eq:delta_mat_dissip}
\end{equation}


\medskip
\noindent\textbf{Step 6: Combining the decrease of $f$ and the choice of $\kappa$.}


Substituting \eqref{eq:delta_mat_dissip} into \eqref{eq:Ek_delta} yields

\begin{align}
E_{k+1}-E_k
&\leq
-c_1||\nabla f(x_k)||^2
-\kappa\omega|D_k|_F^2+
2\kappa A_1(1-\gamma)^2
\eta_k^4||\nabla f(x_k)||^4.
\label{eq:Ek_pre_final}
\end{align}

\noindent Since the sequence ${x_k}$ remains in a compact region and $\nabla f$ is continuous, there exists a constant $G_*>0$ such that

\begin{equation}
||\nabla f(x_k)||\leq G_*,
\qquad
\forall k.
\label{eq:G_bound}
\end{equation}

\noindent Moreover, assume that $0<\eta_k\leq \eta_{\max}$. Then,

\begin{equation}
\eta_k^4||\nabla f(x_k)||^4
\leq
\eta_{\max}^4G_*^2||\nabla f(x_k)||^2.
\label{eq:quartic_bound_new}
\end{equation}

\noindent Define

\begin{equation}
C_*:=2A_1(1-\gamma)^2\eta_{\max}^4G_*^2.
\label{eq:Cstar_new}
\end{equation}

\noindent Thus,

\[
2A_1(1-\gamma)^2
\eta_k^4\|\nabla f(x_k)\|^4
\leq
C_*\|\nabla f(x_k)\|^2.
\]

\noindent Choose $\kappa>0$ sufficiently small so that

\begin{equation}
\kappa C_*
\leq
\frac{c_1}{2}.
\label{eq:kappa_choice_new}
\end{equation}

\noindent For example, it suffices to take

\begin{equation}
0<\kappa<\kappa^*
:=
\frac{c_1}{2C_*}.
\label{eq:kappa_star_new}
\end{equation}

\noindent With this choice, we obtain

\begin{equation}
E_{k+1}-E_k
\leq
-\frac{c_1}{2}||\nabla f(x_k)||^2
-\kappa\omega||D_k||_F^2.
\label{eq:Ek_final_decay_new}
\end{equation}

\noindent Since $D_k=X_k-V_k$, it follows that

\begin{equation}
E_{k+1}
\leq
E_k
-
\frac{c_1}{2}\|\nabla f(x_k)\|^2
-
c_2\|X_k-V_k\|_F^2,
\label{eq:Ek_final_new}
\end{equation}
in which
\[
c_2:=\kappa\omega>0.
\]

Therefore, the sequence ${E_k}$ is non-increasing. Consequently, the accelerated BFGS scheme is stable in the discrete Lyapunov sense.
\end{proof}

\section{Interpretation of the Acceleration Parameters}

An interesting feature of the proposed formulation is that the stability condition obtained from the Lyapunov analysis does not directly constrain the value of the parameter $\beta$ itself, but rather the effective magnitude of the inertia introduced into the system. Indeed, the dissipativity condition derived above (Equation \ref{eq:cond_beta_rho}) can be written as

%\begin{equation}
%2(1-\beta)^2(1-\rho)^2<1.
%\label{eq:cond_dissipativa}
%\end{equation}

%Equivalently,

\begin{equation}
|1-\beta|
<
\frac{1}{\sqrt{2}(1-\rho)}.
\label{eq:cond_beta}
\end{equation}

Notice that the parameter $\beta$ always appears multiplied by the factor $(1-\rho)$. Consequently, the stability of the dynamics depends not only on the absolute value of $\beta$, but on the interaction between these two parameters. This observation motivates the definition of an \emph{effective inertia},

\begin{equation}
\theta:=(1-\beta)(1-\rho).
\label{eq:theta_efetiva}
\end{equation}

From this perspective, the parameter $\rho$ acts as a moderator of the influence of $\beta$. When $\rho$ is close to zero, the factor $(1-\rho)$ remains close to one, and stability imposes a relatively narrow range for $\beta$. In this case,

\[
\rho\rightarrow0
\quad\Longrightarrow\quad
0.2929<\beta<1.7071.
\]

On the other hand, as $\rho$ approaches $1$, the factor $(1-\rho)$ tends to zero, significantly reducing the dynamical impact of $\beta$. As a consequence, the admissible region for $\beta$ becomes progressively larger,

\[
\rho\rightarrow1
\quad\Longrightarrow\quad
\beta\in\mathbb{R}.
\]

This result indicates that large values of $\beta$, including values greater than $1$, may be employed without compromising the stability of the accelerated system, provided that they are accompanied by sufficiently large values of $\rho$. In other words, the parameter $\rho$ acts as a damping mechanism capable of compensating for the increased inertia introduced by $\beta$.

Beyond dynamical stability, it is also necessary to preserve the geometric properties of the auxiliary sequence $V_k$. Expanding the update

\begin{equation}
V_{k+1}=(1-\beta)V_k+\beta Y_k-\gamma(Y_k-X_{k+1}),
\label{eq:Vk_expand}
\end{equation}
and substituting

\[
Y_k=(1-\rho)X_k+\rho V_k,
\]
yields

\begin{equation}
V_{k+1}
=
\bigl[1-\beta(1-\rho)-\gamma\rho\bigr]V_k
+
(\beta-\gamma)(1-\rho)X_k
+
\gamma X_{k+1}.
\label{eq:Vk_convexa}
\end{equation}

The coefficients in \eqref{eq:Vk_convexa} sum to one, so that $V_{k+1}$ can be interpreted as an affine combination of $V_k$, $X_k$, and $X_{k+1}$. To ensure that this combination is convex, and therefore automatically preserves positive definiteness whenever $V_k$, $X_k$, and $X_{k+1}$ belong to the cone $\mathbb{S}_{++}^n$, it suffices to impose

\begin{equation}
0\leq\gamma\leq\beta,
\qquad
\beta(1-\rho)+\gamma\rho\leq1.
\label{eq:cond_convexa}
\end{equation}

\noindent The second inequality implies

\begin{equation}
\beta
\leq
\frac{1-\gamma\rho}{1-\rho}.
\label{eq:beta_spd}
\end{equation}

Once again, the fundamental role of $\rho$ becomes apparent. When $\rho=0$, the classical restriction $\beta\leq1$ is recovered. However, for $\rho>0$, the upper bound increases progressively. For example, when $\rho=0.5$, one obtains approximately $\beta\leq2$, whereas for $\rho=0.9$, values as large as $\beta\leq10$ become admissible without violating the convexity of the update.

Therefore, the parameter $\rho$ plays a dual role in the proposed accelerated dynamics. From the stability viewpoint, it reduces the effective inertia associated with $\beta$. From the geometric viewpoint, it enlarges the admissible range of $\beta$ while preserving the membership of the sequence $V_k$ in the cone of symmetric positive-definite matrices. This interplay makes it possible to explore significantly more aggressive acceleration regimes than those typically considered in conventional momentum-based schemes, while simultaneously maintaining stability and geometric structure.









Theorem~\ref{thm:Lyapunov} establishes Lyapunov stability for the proposed  accelerated geometry scheme. The decay condition, given by Equation \eqref{eq:teo_estabilidade}, ensures that the energy sequence $\{\mathcal{E}_k\}$ decreases monotonically, jointly controlling the evolution of the primal variable $x_k$ and the matrix sequences $X_k$ and $V_k$. The dissipative term $\|X_{k+1}-V_k\|_F^2$ enforces alignment between the quasi-Newton update and the inertial state, implying that $X_k$ and $V_k$ asymptotically coincide. This mechanism acts as a damping effect, preventing oscillations induced by the inertial term. As a consequence, the method preserves positive definiteness, maintains uniform spectral bounds, and converges towards a stationary regime characterized by $\nabla f(x_k)\to 0$ and $X_k \approx V_k$, without compromising the structural properties of the BFGS update.


==> convergence_old.tex <==
A central requirement is the boundedness of the eigenvalues of the metric sequence $X_k,~ V_k$. In particular, it is necessary to establish the existence of constants $0< m\leq M$ such that  $mI \preceq X_k, V_k \preceq MI$ for some $0 < m \le M$. These bounds ensure that the metric approximation remains uniformly positive definite and well conditioned, preventing instability of the search directions and potential divergence caused by the inertial Hessian dynamics.

\begin{lemma}[Boundedness of Eingenvalues]
\label{lem:convex_spd_bounds}
Let $X_k, V_k \in \mathbb{S}_{++}^n$ satisfy $mI \preceq X_k, V_k \preceq MI$ for some $0 < m \le M$. Then, for any $\rho \in (0,1)$,
$$
Y := (1-\rho)X_k + \rho V_k \in \mathbb{S}_{++}^n
\quad\text{and}\quad
mI \preceq Y \preceq MI.
$$

\begin{proof}
For any $z \neq 0$, we have that
$$
z^\top Y z = (1-\rho) z^\top X_k z + \rho z^\top V_k z > 0.
$$
Moreover,
$$
\lambda_{\min}(Y) \ge (1-\rho)\lambda_{\min}(X_k) + \rho\lambda_{\min}(V_k) \ge m,
$$
and
$$
\lambda_{\max}(Y) \le (1-\rho)\lambda_{\max}(X_k) + \rho\lambda_{\max}(V_k) \le M,
$$
which concludes the proof.

\end{proof}
\end{lemma}


An entirely analogous argument applies to the auxiliary variable $V_k$, whose update is also given by a convex combination of matrices in $\mathbb{S}_{++}^n$. Consequently, both $Y_k$ and $V_{k+1}$ preserve positive definiteness by construction, ensuring that all matrix variables remain in the cone $\mathbb{S}_{++}^n$ throughout the iterations.

Ensuring that the intermediate variables $Y_k$ and $V_k$ remain in $\mathbb{S}_{++}^n$ is essential for the subsequent BFGS step to preserve the positive definiteness of the curvature approximation. Once this convexity property is guaranteed, the classical BFGS update can be safely applied to $Y_k$, as stated in Lemma~\ref{lem:bfgs_spd}. Under the curvature condition $s_k^\top \zeta_k > 0$, the BFGS transformation preserves positive definiteness, thereby completing the structural stability cycle between extrapolation and quasi-Newton update.

\begin{lemma}[Positive Definiteness]
\label{lem:bfgs_spd}
Let $Y_k \in \mathbb{S}_{++}^n$ and $s, \zeta \in \mathbb{R}^n$ be such that $\zeta^\top s > 0$. The classical BFGS update
$$
X_{k+1}
= \Big(I-\tfrac{s \zeta^\top}{\zeta^\top s}\Big)\,Y_k\,\Big(I-\tfrac{\zeta s^\top}{\zeta^\top s}\Big)
  + \tfrac{s s^\top}{\zeta^\top s}
$$
satisfies $X_{k+1} \in \mathbb{S}_{++}^n$.

\begin{proof}
Let $\phi := \frac{1}{\zeta^\top s} > 0$ and define $M := I - \phi\,\zeta s^\top$. 

Then $M^\top = I - \phi\, s\zeta^\top$, and the update can be written as
\begin{equation} \begin{array}{lcl}
X_{k+1} &
=& \big(I-\phi\, s\zeta^\top\big)\,Y_k\,\big(I-\phi\,\zeta s^\top\big) + \phi\,ss^\top  \\
&=& M^\top Y_k M + \phi\,ss^\top .
\end{array}
\nonumber
\end{equation}
For any $z \neq 0$, we have that
$$
z^\top X_{k+1} z = (Mz)^\top Y_k (Mz) + \phi (s^\top z)^2.
$$
If $Mz \neq 0$, the first term is strictly positive since $Y_k \succ 0$. If $Mz = 0$, then $z = \phi \zeta (s^\top z)$, which implies $s^\top z \neq 0$, and hence the second term is strictly positive. Therefore, $z^\top X_{k+1} z > 0$ for all $z \neq 0$, proving that $X_{k+1} \in \mathbb{S}_{++}^n$. Symmetry follows from the symmetry of $Y_k$ and the update structure.
\end{proof}
\end{lemma}

Building on these results, we now analyze the stability of the entire scheme jointly considering the evolution of the primal variable $x_k$ and the Hessian approximations. The following theorem provides the main theoretical foundation of the proposed method. It establishes that, under standard smoothness assumptions and sufficiently small step sizes $\eta_k$, there exists a Lyapunov function $\mathcal{E}_k$ that decreases monotonically throughout the iterations. This function combines the objective value with a consistency term between $X_k$ and $V_k$, capturing both the optimization progress and the stability of the matrix sequence.

Moreover, the proof shows that this descent property only requires the acceleration parameters $\rho$ and $\beta$ to lie in suitable subintervals of $(0,1)$. In particular, moderate values ensure that inertial effects remain sufficiently damped, preserving the stability of the coupled dynamics between $X_k$ and $V_k$. The theorem thus characterizes not only structural preservation and numerical stability, but also explicit admissible ranges for the acceleration parameters.

\begin{theorem}[Numerical Stability]
\label{thm:Lyapunov}
Let $f:\mathbb{R}^n \to \mathbb{R}$ be an $C^1$ function with a continuous gradient of $L$ -Lipschitz in a compact region containing the iterates. Consider
\begin{align*}
x_{k+1} &= x_k - \eta_k X_k \nabla f(x_k),\\
Y_k &= (1-\rho)X_k + \rho V_k,\qquad \rho\in(0,\rho_{\max}),\\
X_{k+1} &= \Phi_{\mathrm{BFGS}}(Y_k;\, s_k,\zeta_k),\\
V_{k+1} &= (1-\beta)V_k + \beta X_{k+1},\qquad \beta\in(\beta_{\min},1),
\end{align*}
with $X_0 = V_0 = I$.

Assume $s_k^\top \zeta_k > 0$ for all $k$, and that there exist $0 < m_* \le M_* < \infty$ such that
$$
m_* I \preceq X_k, V_k, Y_k \preceq M_* I.
$$
Suppose further that the step sizes satisfy
\begin{equation}\label{eq:suf-descent}
f(x_{k+1}) \le f(x_k) - c_1 \|\nabla f(x_k)\|^2.
\end{equation}
for some $c_1 > 0$. This $c_1$ can be obtained using an appropriate line search. 

For $\kappa>0$, define
$$
\mathcal{E}_k := f(x_k)-f^* + \kappa\|X_k - V_k\|_F^2.
$$

Then there exist $\kappa^*>0$ and $c_2>0$ such that, for any $\kappa \in (0,\kappa^*)$,
\begin{equation}\label{eq:lyapunov-descent}
\mathcal{E}_{k+1}
\le
\mathcal{E}_k
-
c_1\|\nabla f(x_k)\|^2
-
c_2\|X_{k+1}-V_k\|_F^2.
\end{equation}
Observe that $\kappa^*>0$ and $c_2>0$ depend only on $m_*,~ M_*,~ \rho_{max},~ \beta_{min}$.
In particular, $\{\mathcal{E}_k\}$ is non-increasing, implying Lyapunov stability and $\|X_k - V_k\|_F \to 0$.
\end{theorem}


\begin{proof}
For $\kappa>0$, define the Lyapunov function
$$
\mathcal{E}_k \;:=\; f(x_k)-f^* \;+\; \kappa\|X_k - V_k\|_F^2.
$$
Our goal is to show that, for suitable choices of 
$\rho\in(0,\rho_{\max})$, $\beta\in(\beta_{\min},1)$, and sufficiently small $\kappa>0$, there exist constants $c_1,c_2>0$ such that
\begin{equation}\label{eq:Lyap-target}
\mathcal{E}_{k+1}
\;\le\;
\mathcal{E}_k
-
c_1\|\nabla f(x_k)\|^2
-
c_2\|X_{k+1}-V_k\|_F^2,
\qquad\text{for all }k.
\end{equation}

\medskip
\noindent\textbf{Step 1: Decomposition of $\mathcal{E}_k$.}
From the definition, we have the
$$
\mathcal{E}_{k+1}-\mathcal{E}_k
=
\underbrace{f(x_{k+1})-f(x_k)}_{\text{Term I}}
+
\kappa\underbrace{\Big(\|X_{k+1}-V_{k+1}\|_F^2-\|X_k-V_k\|_F^2\Big)}_{\text{Term II}}.
$$
By the $L$-Lipschitz continuity of the gradient, we also have that
$$
f(x_{k+1}) \le f(x_k) - \eta_k \nabla f(x_k)^\top X_k \nabla f(x_k)
+ \tfrac{L}{2}\eta_k^2 \|X_k\nabla f(x_k)\|^2.
$$
Using $m_\ast I \preceq X_k \preceq M_\ast I$, we obtain
$$
f(x_{k+1}) \le f(x_k) - c_1 \|\nabla f(x_k)\|^2,
$$
with $c_1 = \eta_k m_\ast - \tfrac{L}{2}\eta_k^2 M_\ast^2 > 0$ whenever $\eta_k \le 1/(M_\ast L)$, consistent with Equation~ \eqref{eq:suf-descent}.

It remains to control Term II given by
$$
\Delta_k^{\mathrm{mat}}
:=
\|X_{k+1}-V_{k+1}\|_F^2 - \|X_k-V_k\|_F^2.
$$

\medskip
\noindent\textbf{Step 2: Rewrite term II.}
From the definition of $V_{k+1}$, 
$$
V_{k+1} = (1-\beta)V_k + \beta X_{k+1},
$$
we obtain
$$
X_{k+1}-V_{k+1} = (1-\beta)(X_{k+1}-V_k),
$$
and hence
$$
\|X_{k+1}-V_{k+1}\|_F^2 = (1-\beta)^2 \|X_{k+1}-V_k\|_F^2.
$$
Therefore,
\begin{equation}\label{eq:Delta-mat-0}
\Delta_k^{\mathrm{mat}}
=
(1-\beta)^2\|X_{k+1}-V_k\|_F^2 - \|X_k-V_k\|_F^2.
\end{equation}

\medskip
\noindent\textbf{Step 3: Matrix Young inequality.}
Let $\theta,\varepsilon\in(0,1)$ be specified later. We write
$$
-\|X_k-V_k\|_F^2
=
-\theta\|X_k-V_k\|_F^2
-
(1-\theta)\|X_k-V_k\|_F^2.
$$
Using the matrix Young inequality,
$$
\|A\|_F^2
\ge
(1-\varepsilon)\|B\|_F^2
-
\Big(\tfrac{1}{\varepsilon}-1\Big)\|A-B\|_F^2,
$$
with $A:=X_k-V_k$ and $B:=X_{k+1}-V_k$, we obtain
$$
-\,(1-\theta)\|X_k-V_k\|_F^2
\le
-(1-\theta)(1-\varepsilon)\|X_{k+1}-V_k\|_F^2
+
(1-\theta)\Big(\tfrac{1}{\varepsilon}-1\Big)\|X_{k+1}-X_k\|_F^2.
$$
Substituting into Equation~\eqref{eq:Delta-mat-0} yields
\begin{align}
\Delta_k^{\mathrm{mat}}
&\le
\underbrace{\Big((1-\beta)^2-(1-\theta)(1-\varepsilon)\Big)}_{=:~\Gamma_1}\|X_{k+1}-V_k\|_F^2
-
\theta\|X_k-V_k\|_F^2 \nonumber\\
&\quad
+
\underbrace{(1-\theta)\Big(\tfrac{1}{\varepsilon}-1\Big)}_{=:~\Gamma_0}\|X_{k+1}-X_k\|_F^2.
\label{eq:Delta-mat-1}
\end{align}

\medskip
\noindent\textbf{Step 4: Bounds for $\|X_{k+1}-X_k\|_F^2$.}
Using the quasi-Newton lemma and spectral bounds ($m_*I\preceq X_k,V_k,Y_k\preceq M_*I$), there exists $A>0$, depending only on $m_*,M_*,L$, such that
\begin{equation}\label{eq:bound-Xdiff-1}
\|X_{k+1}-Y_k\|_F
\;\le\;
A\,\|s_k\|\,\|\zeta_k\|.
\end{equation}
With $s_k=-\eta_k X_k\nabla f(x_k)$ and the Lipschitz continuity of the gradient, we obtain
$$
\|X_{k+1}-Y_k\|_F
\le
A\,\|s_k\|\,\|\zeta_k\|
\le
AL M_*^2 \eta_k^2 \|\nabla f(x_k)\|^2.
$$
In this way, there exists $A_1>0$ such that 
\begin{equation}\label{eq:bound-Xdiff-2}
\|X_{k+1}-Y_k\|_F^2
\;\le\;
A_1\,\eta_k^4\,\|\nabla f(x_k)\|^4.
\end{equation}

Moreover, since $Y_k-X_k=\rho(V_k-X_k)$ and using the triangular inequality, we have 
\begin{equation}\label{eq:bound-Xdiff-3}
\|X_{k+1}-X_k\|_F
\;\le\;
\|X_{k+1}-Y_k\|_F+\rho\|X_{k}-V_k\|_F.
\end{equation}
From Equation~\eqref{eq:bound-Xdiff-2} and the special case of the Cauchy-Schwarz inequality, we have that  
\begin{equation}\label{eq:bound-Xdiff-4}
\|X_{k+1}-X_k\|_F^2
\le
2A_1 \eta_k^4 \|\nabla f(x_k)\|^4
+
2\rho^2 \|X_k-V_k\|_F^2.
\end{equation}

\medskip
\noindent\textbf{Step 5: Selection of parameters.}
Substituting Equation~\eqref{eq:bound-Xdiff-4} into Equation~\eqref{eq:Delta-mat-1} gives the following result:
\begin{align}
\Delta_k^{\mathrm{mat}}
&\le
\Gamma_1\,\|X_{k+1}-V_k\|_F^2
-
\theta\|X_k-V_k\|_F^2
+
\Gamma_0\Big(2A_1\eta_k^4\|\nabla f(x_k)\|^4 + 2\rho^2\|X_k-V_k\|_F^2\Big)
\nonumber\\[0.1cm]
&=
\Gamma_1\,\|X_{k+1}-V_k\|_F^2
+
\underbrace{\big(-\theta + 2\Gamma_0 \rho^2\big)}_{=:~\Gamma_2}\,
\|X_k-V_k\|_F^2
+
2\Gamma_0 A_1\eta_k^4\|\nabla f(x_k)\|^4.
\label{eq:Delta-mat-2}
\end{align}

************ AQUI AQUI AQUI ****************

Without loss of generality, imposing $\theta+\varepsilon=1$, to guaranty the validity of Equation~\eqref{eq:lyapunov-descent}, we need to have
$$
\Gamma_1 < 0 \;\Longleftrightarrow\; \beta > \tfrac12,
\qquad
\Gamma_2 < 0 \;\Longleftrightarrow\; \rho < \tfrac{1}{\sqrt{2}}.
$$


\medskip
\noindent\textbf{Choice of $\beta_{\min}$.}
Under the condition $\theta+\varepsilon=1$, the expression for $\Gamma_1$ becomes
$$
\Gamma_1 = (1-\beta)^2 - (1-\theta)(1-\varepsilon)
           = (1-\beta)^2 - \theta(1-\theta).
$$
The function $\theta(1-\theta)$ achieves its maximum at $\theta=\tfrac{1}{2}$,
with value $1/4$. Therefore,
$$
\Gamma_1 < 0
\quad\Longleftrightarrow\quad
(1-\beta)^2 < \tfrac14
\quad\Longleftrightarrow\quad
\beta > \tfrac12.
$$
Hence, any parameter
$$
\beta \in (\beta_{\min},1),
\qquad
\beta_{\min} := \tfrac12,
$$
ensures the existence of a constant $\gamma_1>0$ such that
\begin{equation}\label{eq:Gamma1-neg}
\Gamma_1 \le -\gamma_1 < 0.
\end{equation}

\medskip
\noindent\textbf{Choice of $\rho_{\max}$.}
From the definition of $\Gamma_0$ in \eqref{eq:Delta-mat-1}, and using
$\theta+\varepsilon=1$, we obtain $\Gamma_0=\theta$. Thus,
$$
\Gamma_2 = -\theta + 2\theta\rho^2
          = \theta(2\rho^2 - 1).
$$
The condition $\Gamma_2<0$ is equivalent to
$$
2\rho^2 - 1 < 0
\quad\Longleftrightarrow\quad
\rho < \frac{1}{\sqrt{2}}.
$$
Therefore, for any
$$
\rho \in (0,\rho_{\max}),
\qquad
\rho_{\max} := \frac{1}{\sqrt{2}},
$$
there exists a constant $\gamma_2>0$ such that
\begin{equation}\label{eq:Gamma2-neg}
\Gamma_2 \le -\gamma_2 < 0.
\end{equation}

\medskip
We conclude that the Lyapunov analysis requires the acceleration parameters to be within the ranges
$$
\beta \in (\beta_{\min},1),
\qquad
\rho \in (0,\rho_{\max}),
$$
with $\beta_{\min}=\tfrac12$ and $\rho_{\max} = \tfrac{1}{\sqrt{2}}$, ensuring that both
$\Gamma_1$ and $\Gamma_2$ contribute dissipative terms in the descent inequality given by Equation~\eqref{eq:lyapunov-descent}.


\medskip
\noindent\textbf{Step 6: Choose $\kappa^*$.}
Using Equations~\eqref{eq:Gamma1-neg} and \eqref{eq:Gamma2-neg}, Equation~\eqref{eq:Delta-mat-2} implies that, for $\rho\in(0,\rho_{\max})$ and
$\beta\in(\beta_{\min},1)$,
$$
\Delta_k^{\mathrm{mat}}
\le
-\gamma_1\|X_{k+1}-V_k\|_F^2
-\gamma_2\|X_k-V_k\|_F^2
+
2\Gamma_0 A_1\eta_k^4\|\nabla f(x_k)\|^4.
$$
Multiplying by $\kappa>0$ and adding Equation~\eqref{eq:suf-descent}, we obtain
\begin{equation}
\begin{array}{lcl}
\mathcal{E}_{k+1}-\mathcal{E}_k
&\le &
-c_1\|\nabla f(x_k)\|^2
-\kappa\gamma_1\|X_{k+1}-V_k\|_F^2  -\\
&  & -\kappa\gamma_2\|X_k-V_k\|_F^2 +
2\kappa \Gamma_0 A_1\eta_k^4\|\nabla f(x_k)\|^4.
\label{eq:Delta-Ek-pre}
\end{array}
\end{equation}

Since the sequence $(x_k)$ remains in a compact region and the gradient is Lipschitz continuous, there exists $G_*>0$ such that
$\|\nabla f(x_k)\|\le G_*$ for all $k$. Moreover, the line search ensures that $\eta_k\le\eta_{\max}$. Therefore,
$$
\eta_k^4\|\nabla f(x_k)\|^4
\le
\eta_{\max}^4 G_*^2\,\|\nabla f(x_k)\|^2.
$$
Defining
$$
C_* := 2\Gamma_0 A_1 \eta_{\max}^4 G_*^2,
$$
it follows that
$$
2\kappa \Gamma_0 A_1\eta_k^4\|\nabla f(x_k)\|^4
\le
\kappa C_* \|\nabla f(x_k)\|^2.
$$

We now choose $\kappa>0$ sufficiently small such that
$$
\kappa C_* \le \frac{c_1}{2}.
$$
Such a choice always exists, and we define
$$
\kappa^* := \frac{c_1}{2C_*},
$$
so that the above condition holds for any
$\kappa\in(0,\kappa^*)$.

Under this choice, Equation~\eqref{eq:Delta-Ek-pre} reduces to
\begin{equation}\label{eq:Delta-Ek-final}
\mathcal{E}_{k+1}-\mathcal{E}_k
\;\le\;
-\frac{c_1}{2}\|\nabla f(x_k)\|^2
-\kappa\gamma_1\|X_{k+1}-V_k\|_F^2.
\end{equation}
Defining $c_2 := \kappa\gamma_1>0$, we recover exactly Equation~\eqref{eq:Lyap-target} (up to replacing $c_1$ by $c_1/2$, which does not affect the result).

In particular, the sequence $\{\mathcal{E}_k\}$ is non-increasing for any
$\kappa\in(0,\kappa^*)$, which ensures Lyapunov stability and implies that $\|X_k - V_k\|_F \to 0$ along the iterations.

\end{proof}








==> experiments.tex <==
\section{Numerical Experiments}
\label{sec:experiments}

In this section, we evaluate the performance of the proposed optimization algorithm, which extends the classical BFGS method by incorporating two additional mechanisms: an accelerated geometry component and a stochastic component applied to the search directions. The objective of the experimental study is not only to assess the overall effectiveness of the proposed approach but also to investigate the individual contribution of each additional component to the optimization process.

To this end, in comparative analysis, three algorithmic variants are considered. The first corresponds to the standard BFGS algorithm, which serves as a baseline method and does not include either of the proposed enhancements. The second variant combines BFGS with the accelerated geometry mechanism only (AG-BFGS), allowing the impact of the geometric acceleration strategy to be isolated and analyzed independently of the stochastic component. Finally, the third variant corresponds to the complete proposed algorithm, Accelerated Geometry BFGS with stochastic component in the search directions (AGS-BFGS), where both the accelerated geometry mechanism and the stochastic search-direction component are employed simultaneously.

This experimental design enables systematic ablation-style analysis of the proposed method. By progressively introducing additional components, it becomes possible to evaluate how each mechanism affects convergence behavior, robustness, and overall optimization performance. The experiments reported in the following compare these variants across a set of benchmark optimization problems using standard performance metrics and statistical analyzes.



\subsection{Experimental Setup}

The proposed method, Accelerated Geometry BFGS with Stochastic Component in the Search Directions, is compared with the following methods:
\begin{itemize}
    \item Classical BFGS; and
    \item Accelerated Geometry BFGS.
 %   \item Stochastic quasi-Newton variants from the literature.
\end{itemize}

All methods are implemented in a common framework using identical initialization and stopping criteria. Step sizes are determined through a backtracking line search and the parameters for stochastic perturbation are selected to balance exploration and stability.

\subsection{Benchmark Problems}

We consider a collection 23 benchmark functions \cite{Fogel91,Back93, Torn89,Wolpert95}, including:
\begin{itemize}
    \item Ill-conditioned convex functions;
    \item Nonconvex multimodal functions;
    \item High-dimensional optimization problems.
\end{itemize}

The functions are briefly described below. $n$ denotes the dimension of the search space, $x^*$ is the minimum point,  $f_{min}$ is the minimum value of the function and $S \subseteq \mathbf{R}^n$: 

\vspace{8pt}

\noindent \textbf{Sphere function}

\vspace{4pt}

\noindent$f_1(x) = \sum_{i=1}^{n} x_i^2$, $n = 30$, $S = [-100,~100]^n$, $x^* = (0, \cdots, 0)$, $f_{min} = 0$

\vspace{4pt}

\noindent \textbf{Schwefel's Problem 2.22} 

\vspace{4pt}

\noindent$f_2(x) = \sum_{i=1}^{n} \left|x_i\right| + \prod_{i=1}^{n} |x_i|$, $n=30$, $[-10,10]^n$, $x^* = (0, \cdots, 0)$, $f_{min} =0$ 

\vspace{4pt}

 

\noindent \textbf{Schwefel's Problem 1.2}

\vspace{4pt}

\noindent$f_3(x) =\sum_{i=1}^{n}\left(\sum_{j=1}^{i} x_j\right)^2$, $n=30$, $[-100,100]^n$, $x^* = (0, \cdots, 0)$, $f_{min} =0$ 

\vspace{4pt}


\noindent \textbf{Schwefel's Problem 2.21}

\vspace{4pt}

\noindent$f_4(x) = \max_i |x_i|$, $n=30$, $[-100,100]^n$, $x^* = (0, \cdots, 0)$, $f_{min} =0$

\vspace{4pt}

\noindent \textbf{Generalized Rosenbrock’s Function}

\vspace{4pt}

\noindent$f_5(x)= \sum_{i=1}^{n} \left[100(x_{i+1}-x_i^2)^2 + (x_i-1)^2\right]$, $n=30$, $[-30,30]^n$, $x^* = (1, \cdots, 1)$, $f_{min} =0$ 

\vspace{4pt}


\noindent \textbf{Step Function}

\vspace{4pt}

\noindent$f_6(x) =\sum_{i=1}^{n} \left(\lfloor x_i + 0.5\rfloor\right)^2$, $n=30$, $[-100,100]^n$, $x^* = (0, \cdots, 0)$, $f_{min} =0$ 

\vspace{4pt}

\noindent \textbf{Quartic Function i.e. Noise}

\vspace{4pt}


\noindent$f_7(x)=\sum_{i=1}^{n}\left[i x_i^4\right] + random(0,1)$,  $n=30$, $[1.28,1.28]^n$, $x^* = (0, \cdots, 0)$, $f_{min} =0$

\vspace{4pt}


\noindent \textbf{Generalized Schwefel’s Problem 2.26}

\vspace{4pt}

\noindent$f_8(x) = \sum_{i=1}^{n} -x_i \sin(\sqrt{|x_i|})$, $n=30$ $[-500,500]^n$, $x^* = (420.9687, \cdots, 420.9687)$, $f_{min} =-12569.5$

\vspace{4pt}


\noindent \textbf{Generalized Rastrigin’s Function}

\vspace{4pt}

\noindent$f_9(x) = \sum_{i=1}^{n}\left[x_i^2 - 10\cos(2\pi x_i) + 10\right]$, $n=30$, $ [-5.12,5.12]^n$, $x^* = (0, \cdots, 0)$, $f_{min} =0$

\vspace{4pt}


\noindent \textbf{Ackley’s Function}

\vspace{4pt}

\noindent$f_{10}(x) =-20\exp\left(-0.2\sqrt{\frac{1}{n}\sum_{i=1}^n x_i^2}\right) - \exp\left(\frac{1}{n}\sum_{i=1}^n \cos(2\pi x_i)\right) + 20 + e$, $n=30$, $ [-32,32]^n$, $x^* = (0, \cdots, 0)$, $f_{min} =0$

\vspace{4pt}

\noindent \textbf{Generalized Griewank Function}

\vspace{4pt}

\noindent$f_{11}(x) = \frac{1}{4000}\sum_{i=1}^n x_i^2 - \prod_{i=1}^n \cos\left(\frac{x_i}{\sqrt{i}}\right) + 1$, $n=30$,  $[-600,600]^n$, $x^* = (0, \cdots, 0)$, $f_{min} =0$


\vspace{4pt}

\noindent  \textbf{Generalized Penalized Functions}

\vspace{4pt}

\noindent$f_{12}(x) = 0.1\left[10\sin^2(\pi y_1) + \sum_{i=1}^{n-1} (y_i-1)^2\left(1+10\sin^2(\pi y_{i+1})\right) + (y_n-1)^2\right]$, where $y_i = 1 + \frac{x_i+1}{4}$, $n=30$, $[-50,50]^n$, $x^* = (1, \cdots, 1)$, $f_{min} =0$

\vspace{4pt}

\noindent $\begin{array}{clc}f_{13}(x)
&=&
0.1\left\{
\sin^2(3\pi x_1)
+
\sum_{i=1}^{n-1}
(x_i-1)^2
\left[
1+\sin^2(3\pi x_{i+1})
\right] + \right.\\
&&
\left. +
(x_n-1)^2
\left[
1+\sin^2(2\pi x_n)
\right]
\right\}
+
\sum_{i=1}^{n}u(x_i,5,100,4)  \end{array}$
 
\noindent in which
$u(x_i,a,k,m)=
\begin{cases}
k(x_i-a)^m, & x_i>a,\\
0, & -a\le x_i\le a,\\
k(-x_i-a)^m, & x_i<-a.
\end{cases}$

\noindent$y_i = 1+ \frac{1}{4}(x_i+ 1)$, $n = 30$, $[-50, 50]^n $, $x^* = (1, \cdots, 1)$, $f_{min} =0$

 \vspace{4pt}


\noindent \textbf{Shekel’s Foxholes Function}

\vspace{4pt}

\noindent$f_{14}(x)=
\left[
\frac{1}{500}
+
\sum_{j=1}^{25}
\frac{1}{
j+\sum_{i=1}^{2}(x_i-a_{ij})^6
}
\right]^{-1}$,  $n = 2$, $[-65.536, 65.536]^n $, 

\noindent$x^* = (-32,-32)$, $f_{min} \approx 1$ 

\vspace{4pt}

\noindent in which  $a_{ij} = \left(\begin{array}{cccccccccc} -32& -16& 0& 16& 32 & -32 & \cdots & 0& 16& 32  \\ -32& -32 & -32 & -32& -32 & -16 & \cdots & 32 & 32 & 32\end{array}\right)$

\vspace{4pt}

\noindent \textbf{Kowalik’s Function}

\vspace{4pt}

\noindent$f_{15}(x)=\sum_{i=1}^{11}\left[a_i-\frac{x_1(b_i^2+b_i x_2)}{b_i^2+b_i x_3+x_4}\right]^2$, in which $a_i$ and $b_i$ are given in Table \ref{tab:kowal}, 


\begin{table}[h!]
\centering
\begin{tabular}{c|c|c}
\hline
i & $a_i$ & $b_i^ {-1}$ \\
\hline
1 & 0.1957 & 0.25 \\
2 &   0.1947 & 0.5 \\
3& 0.1735 & 1 \\
4& 0.1600 & 2 \\
5 & 0.0844 & 4 \\
6 & 0.0627 & 6 \\
7 & 0.0456 & 8 \\
8 &0.0342 & 10 \\
9 & 0.0323 & 12 \\
10 & 0.0235 & 14\\
11 & 0.0246 & 16 \\
\hline
\end{tabular}
\caption{Kowalick's function}
\label{tab:kowal}
\end{table}



%\begin{table}[h!]
%\centering
%\begin{tabular}{c|ccccccccccc}
%\hline
%$i$ & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 \\ \hline
%$a_i$ & 0.1957 & 0.1947 & 0.1735 & 0.1600 & 0. 0844 & 0.0627 & 0.0456 %& 0.0342 & 0.0323 & 0.0235 & 0.0246 \\ \hline 
%$b_i^ {-1}$ & 0.25 & 0.5 & 1 & 2 & 4 & 6 & 8 & 18 & 12 & 14 &16 \\
%\hline
%\end{tabular}
%\caption{Kowalick's function}
%\label{tab:kowal}
%\end{table}


\vspace{4pt}

\noindent and $n = 4$, $[-5, 5]^n $, $x^* =(0.1928,0.1908,0.1231,0.1358)$, $f_{min} =0.000375$

\vspace{4pt}


\noindent \textbf{Six-Hump Camel-Back Function}

\vspace{4pt}

\noindent$f_{16}(x)=4x_1^2-2.1x_1^4+\frac{x_1^6}{3}+x_1x_2-4x_2^2+4x_2^4$,  $n = 2$, $[-5, 5]^n $, 

\vspace{4pt}

\noindent $x^* =(0.08983,-0.7123),~(0.08983,0.7123)$, $f_{min} =-1.0316285$

\vspace{4pt}

\noindent \textbf{Branin Function}

\vspace{4pt}

\noindent$f_{17}(x)=\left(x_2-\frac{5.1}{4\pi^2}x_1^2+\frac{5}{\pi}x_1-6\right)^2+10\left(1-\frac{1}{8\pi}\right)\cos x_1+10$,  $n = 2$, $[-5, 10]^2 $, 

\vspace{4pt}

\noindent $x^* =(-3.142, 12.275),~(3.142, 12.275), ~ (9.425,2.425)$, $f_{min} =0.398$

\vspace{4pt}


\noindent \textbf{Goldstein-Price Function}

\vspace{4pt}

\noindent$ \begin{array}{lcl}f_{18}(x)&=&\left[1+(x_1+x_2+1)^2\left(19-14x_1+3x_1^2-14x_2+6x_1x_2+3x_2^2\right)\right]\nonumber\\ &&\quad\times\left[30+(2x_1-3x_2)^2\left(18-32x_1+12x_1^2+48x_2-36x_1x_2+27x_2^2\right)\right] \end{array}$  

\vspace{4pt}

\noindent$n = 2$, $[-2, 2]^n $, $x^* =(0,-1)$, $f_{min} =3$

\vspace{4pt}

\noindent \textbf{Hartman’s Family}

\vspace{4pt}

\noindent$f_{19}(x)=-\sum_{i=1}^{4}c_i\exp\left(-\sum_{j=1}^{3}a_{ij}(x_jp_{ij})^2\right)$,  $n = 4$, $[0, 1]^n $,

\vspace{4pt}

\noindent $x^* =(0.114,0.556,0.852)$, $f_{min} =-3.86$.

\vspace{4pt}

\noindent$f_{20}(x)=-\sum_{i=1}^{4}c_i\exp\left(-\sum_{j=1}^{6}a_{ij}(x_jp_{ij})^2\right)$, $n = 6$, $[0, 1]^n $, 

\vspace{4pt}

\noindent $x^* =(0.201,0.150,0.477,0.275,0.311,0.657)$, $f_{min} =.3.32$.

\vspace{4pt}

\noindent The coefficients for functions $f_{19}$ and $f_{20}$ are given in Tables \ref{tab:Hartman1} and \ref{tab:Hartman2} respectively.

\begin{table}[h!]
\centering
\begin{tabular}{c|ccc|c|ccc}
$i$ & $a_{i1}$ & $a_{i2}$ & $a_{i3}$ & $c_{i}$ & $p_{i1}$ & $p_{i2}$ & $p_{i3}$ \\ 
\hline 
1& 3 & 10 & 30 & 1& 0.3689 & 0.1170 & 0.2673 \\
2 & 0.1 & 10 & 35 & 1.2 & 0.4699 & 0.4387 & 0.7470 \\
3 & 3 & 10 & 30 & 3 & 0.1091 & 0.8732 & 0.5547 \\
4 & 0.1 & 10 & 35 & 3.2 & 0.038150 & 0.5743 & 0.8828 \\
\hline
\hline
\end{tabular}
\caption{Hartman function $f_{19}$}
\label{tab:Hartman1}
\end{table}


\begin{table}[h!]
\centering
\small
\begin{tabular}{c|cccccc|c|cccccc}
\hline
$i$ & $a_{i1}$ & $a_{i2}$ & $a_{i3}$ & $a_{i4}$ & $a_{i5}$ & $a_{i6}$&  $c_{i}$ & $p_{i1}$ & $p_{i2}$ & $p_{i3}$ & $p_{i4}$ & $p_{i5}$ & $p_{i6}$\\ 
\hline 
1& 10 & 3 & 17 &3.5 & 1.7& 8& 1& 0.1312 & 0.1696 & 0.5569 & 0.0124 & 0.8283 & 0.5886 \\
2 & 0.05 & 10 & 17 & 0.1 & 8 & 14 & 1.2 & 0.2329 & 0.4135 & 0.8307 & 0.3736 & 0.1004 & 0.9991 \\
3 & 3 & 3.5 & 1.7 &10 & 17 & 8 & 3 & 0.2348 & 0.1415 & 0.3522 & 0.2883 & 0.3047 & 0.6650 \\
4 & 17 & 8 & 0.05& 10 & 0.1& 14 & 3.2 & 0.4047 & 0.8828 & 0.8732 & 0.5743 & 0.1091 & 0.0381 \\
\hline
\end{tabular}
\caption{Hartman function $f_{20}$}
\label{tab:Hartman2}
\end{table}
  

\noindent \textbf{Shekel’s Family}

\vspace{4pt}

\noindent$f_{21}(x)=-\sum_{i=1}^{5}\left[(x-a_i)(x-a_i)^T+c_i\right]^{-1}$, $n = 5$, $[0, 10]^n $, 5 local minima $x^* =a_i$, $f_{min} /approx \frac{1}{c_i}$

\vspace{4pt}

\noindent$f_{22}(x)=-\sum_{i=1}^{7}\left[(x-a_i)(x-a_i)^T+c_i\right]^{-1}$,  $n = 7$, $[0, 10]^n $, 7 local minima $x^* =a_i$, $f_{min} /approx \frac{1}{c_i}$

\vspace{4pt}

\noindent$f_{23}(x)=-\sum_{i=1}^{10}\left[(x-a_i)(x-a_i)^T+c_i\right]^{-1}$,  $n = 10$, $[0, 10]^n $, 10 local minima $x^* =a_i$, $f_{min} /approx \frac{1}{c_i}$

\vspace{4pt}

\noindent These functions have five, seven, and ten local minima for $f_{21}$, $f_{22}$ and $f_{23}$, respectively.  

\vspace{4pt}

\noindent$x^* \approx a_i$, $f_{min} /approx \frac{1}{c_i}$ for  $1 \leq i \leq m$.  The coefficients are
defined by Table \ref{tab:shekel}.

\begin{table}[h!]
\centering
\small
\begin{tabular}{c|cccc|c}
\hline
$i$ & $a_{i1}$ & $a_{i2}$ & $a_{13}$ & $a_{14}$ & $c_1$ \\ \hline
1 & 4 & 4 & 4 & 4 & 0.1 \\ 
2 & 1 & 1 & 1 & 1 & 0.2 \\
3 & 8 & 8 & 8 & 8 & 0.2 \\
4 & 6 & 6 & 6 & 6 & 0.4 \\
5 & 3 & 7 & 3 & 7 & 0.4 \\
6 & 2 & 9 & 2 & 9 & 0.6 \\
7 & 5 & 5 & 3 & 3 &0.3 \\
8 & 8 & 1 & 8 & 1 & 0.7 \\
9 & 6 & 2 & 6 & 2 & 0.5 \\
10 & 7 & 3.6 & 7 & 3.6 & 0.5 \\
\hline
\end{tabular}
\caption{Shekel's functions $f_{21}, f_{22}, f_{23}$}
\label{tab:shekel}
\end{table}


%\end{description}



\subsection{Results and Discussion}

The results show that the proposed method consistently outperforms classical BFGS in scenarios involving ill-conditioning and multimodality. In particular, the stochastic perturbation enables the method to escape flat regions and shallow local minima more effectively.

Compared to deterministic accelerated variants, the proposed approach demonstrates improved robustness, especially in the presence of noisy or poorly scaled gradients. The incorporation of stochasticity in the search direction provides a controlled exploration mechanism without degrading the quality of curvature estimates.

Moreover, the method achieves comparable or superior convergence rates in terms of function evaluations, highlighting the efficiency of combining acceleration and stochastic perturbations.



==> func_regina.tex <==
\noindent{\textbf{Ellipsoidal Function}}: The Ellipsoidal Function is a convex unimodal benchmark defined by

\begin{equation}
f_{\mathrm{E}}(\mathbf{x})
=
\sum_{i=1}^{D}
\lambda_i x_i^2,
\qquad
\lambda_i
=
10^{6\frac{i-1}{D-1}},
\end{equation}
where $\mathbf{x}\in[-100,100]^D$ and $D$ is the problem dimension.

\noindent The coefficients $\lambda_i$ vary from $1$ to $10^6$, yielding an ill-conditioned optimization problem with condition number $10^6$. The global minimizer is located at
$\mathbf{x}^{\star}=\mathbf{0}$ e $f(\mathbf{x}^{\star})=0.$
Since the variables are uncoupled, the function is separable.

\noindent{\textbf{Rotated Ellipsoidal Function}}: The rotated version is obtained by applying an orthogonal transformation to the search space. Let $Q\in\mathbb{R}^{D\times D}$ be an orthogonal matrix satisfying $Q^{\top}Q=QQ^{\top}=I.$
Defining $\mathbf{z}=Q^{\top}\mathbf{x}$, the Rotated Ellipsoidal Function is given by

\begin{equation}
f_{\mathrm{RE}}(\mathbf{x})
=
\sum_{i=1}^{D}
\lambda_i z_i^2,
\qquad
\lambda_i
=
10^{6\frac{i-1}{D-1}}.
\end{equation}

In the experiments, the matrix $Q$ is generated through a QR decomposition of a Gaussian random matrix and then kept fixed. The rotation preserves the condition number and the location of the global optimum, $\mathbf{x}^{\star}=\mathbf{0}$ e $f(\mathbf{x}^{\star})=0$, while introducing interactions among the variables, making the problem non-separable.
The same orthogonal matrix $Q$ is employed in all subsequent rotated benchmark functions.

\noindent{\textbf{Discus Function}}: The Discus Function, also known as the Tablet Function, is defined by

\begin{equation}
f_{\mathrm{D}}(\mathbf{x})
=
10^6 x_1^2
+
\sum_{i=2}^{D} x_i^2,
\end{equation}

where $\mathbf{x}\in[-100,100]^D$ and $D$ denotes the problem dimension.

This function is characterized by a single highly scaled direction and $D-1$ directions with unit scaling, resulting in an ill-conditioned optimization problem with condition number $10^6$. The global minimizer is given by $\mathbf{x}^{\star}=\mathbf{0}$ and $f(\mathbf{x}^{\star})=0$. Since the variables are uncoupled, the function is separable.

\noindent{\textbf{Rotated Discus Function}}: Using the same orthogonal transformation introduced for the Rotated Ellipsoidal Function, let $\mathbf{z}=Q^{\top}\mathbf{x}$. The Rotated Discus Function is defined as

\begin{equation}
f_{\mathrm{RD}}(\mathbf{x})
=
10^6 z_1^2
+
\sum_{i=2}^{D} z_i^2.
\end{equation}

The orthogonal transformation preserves both the condition number and the location of the global optimum, while introducing dependencies among the variables. Consequently, the Rotated Discus Function is non-separable and retains the global optimum $\mathbf{x}^{\star}=\mathbf{0}$ with $f(\mathbf{x}^{\star})=0$.

\noindent{\textbf{Bent Cigar Function}}: The Bent Cigar Function is defined by

\begin{equation}
f_{\mathrm{BC}}(\mathbf{x})
=
x_1^2
+
10^6
\sum_{i=2}^{D} x_i^2,
\end{equation}

where $\mathbf{x}\in[-100,100]^D$ and $D$ denotes the problem dimension.

This function exhibits a single direction with unit scaling and $D-1$ highly scaled directions. As a consequence, it defines an ill-conditioned optimization problem with condition number $10^6$. The global minimizer is given by $\mathbf{x}^{\star}=\mathbf{0}$ and $f(\mathbf{x}^{\star})=0$. Since the variables are uncoupled, the function is separable.

\noindent{\textbf{Rotated Bent Cigar Function}}: Using the same orthogonal transformation introduced for the Rotated Ellipsoidal Function, let $\mathbf{z}=Q^{\top}\mathbf{x}$. The Rotated Bent Cigar Function is defined as

\begin{equation}
f_{\mathrm{RBC}}(\mathbf{x})
=
z_1^2
+
10^6
\sum_{i=2}^{D} z_i^2.
\end{equation}

The orthogonal transformation preserves both the condition number and the location of the global optimum, while introducing interactions among the variables. Consequently, the Rotated Bent Cigar Function is non-separable and retains the global optimum $\mathbf{x}^{\star}=\mathbf{0}$ with $f(\mathbf{x}^{\star})=0$.

\noindent{\textbf{Sharp Ridge Function}}: The Sharp Ridge Function is defined by

\begin{equation}
f_{\mathrm{SR}}(\mathbf{x})
=
x_1^2
+
100
\sqrt{\sum_{i=2}^{D} x_i^2},
\end{equation}

where $\mathbf{x}\in[-100,100]^D$ and $D$ denotes the problem dimension.

The function combines a quadratic term along the first coordinate with a ridge-shaped structure in the remaining directions. This geometry creates a narrow valley with a sharp transition in curvature, making the optimization process challenging, particularly for methods that rely on local curvature information. The global minimizer is given by $\mathbf{x}^{\star}=\mathbf{0}$ and $f(\mathbf{x}^{\star})=0$. Since the variables are uncoupled, the function is separable.

\noindent{\textbf{Rotated Sharp Ridge Function}}: Using the same orthogonal transformation introduced for the Rotated Ellipsoidal Function, let $\mathbf{z}=Q^{\top}\mathbf{x}$. The Rotated Sharp Ridge Function is defined as

\begin{equation}
f_{\mathrm{RSR}}(\mathbf{x})
=
z_1^2
+
100
\sqrt{\sum_{i=2}^{D} z_i^2}.
\end{equation}

The orthogonal transformation preserves the location of the global optimum while introducing dependencies among the variables. Consequently, the Rotated Sharp Ridge Function is non-separable and retains the global optimum $\mathbf{x}^{\star}=\mathbf{0}$ with $f(\mathbf{x}^{\star})=0$.

\noindent{\textbf{Different Powers Function}}: The Different Powers Function is defined by

\begin{equation}
f_{\mathrm{DP}}(\mathbf{x})
=
\left(
\sum_{i=1}^{D}
|x_i|^{p_i}
\right)^{\frac{1}{2}},
\end{equation}

where

\begin{equation}
p_i
=
2+4\frac{i-1}{D-1},
\qquad
i=1,\ldots,D,
\end{equation}

and $\mathbf{x}\in[-100,100]^D$.

The exponents increase gradually from $2$ to $6$, yielding directions with different growth rates and sensitivities. As a consequence, the function exhibits heterogeneous curvature across the search space, providing a challenging benchmark for optimization algorithms. The global minimizer is given by $\mathbf{x}^{\star}=\mathbf{0}$ and $f(\mathbf{x}^{\star})=0$. Since each variable contributes independently to the objective value, the function is separable.

\noindent{\textbf{Rotated Different Powers Function}}: Using the same orthogonal transformation introduced for the Rotated Ellipsoidal Function, let $\mathbf{z}=Q^{\top}\mathbf{x}$. The Rotated Different Powers Function is defined as

\begin{equation}
f_{\mathrm{RDP}}(\mathbf{x})
=
\left(
\sum_{i=1}^{D}
|z_i|^{p_i}
\right)^{\frac{1}{2}},
\end{equation}

where

\begin{equation}
p_i
=
2+4\frac{i-1}{D-1},
\qquad
i=1,\ldots,D.
\end{equation}

The orthogonal transformation preserves the location of the global optimum while coupling the variables through the rotated coordinates. Consequently, the Rotated Different Powers Function is non-separable and retains the global optimum $\mathbf{x}^{\star}=\mathbf{0}$ with $f(\mathbf{x}^{\star})=0$.


***************************************************************

\section{Benchmark Problems}

All benchmark functions are defined on the domain
$\mathbf{x}\in[-100,100]^D$, where $D$ denotes the problem dimension.
Unless otherwise stated, all functions attain their global minimum at
$\mathbf{x}^{\star}=\mathbf{0}$ with objective value
$f(\mathbf{x}^{\star})=0$.

The rotated benchmarks are constructed through the orthogonal transformation $\mathbf{z}=Q^{\top}\mathbf{x}$, where $Q\in\mathbb{R}^{D\times D}$ satisfies 
$Q^{\top}Q=QQ^{\top}=I.$ In the numerical experiments, the matrix $Q$ is generated through a QR decomposition of a Gaussian random matrix and then kept fixed. This transformation preserves the location of the global optimum and the geometric properties of the original problem while introducing interactions among the variables, thereby producing non-separable benchmark functions.

\textbf{Separable Functions}

{\textbf{Ellipsoidal Function}}
\begin{equation}
f_{\mathrm{E}}(\mathbf{x})
=
\sum_{i=1}^{D}
\lambda_i x_i^2,
\qquad
\lambda_i
=
10^{6\frac{i-1}{D-1}}.
\end{equation}

The coefficients $\lambda_i$ vary from $1$ to $10^6$, yielding a separable ill-conditioned problem with condition number $10^6$.

\medskip

\noindent{\textbf{Discus Function}}
\begin{equation}
f_{\mathrm{D}}(\mathbf{x})
=
10^6x_1^2
+
\sum_{i=2}^{D}x_i^2.
\end{equation}

This function contains a single highly scaled direction and has condition number $10^6$.

\medskip

\noindent{\textbf{Bent Cigar Function}}
\begin{equation}
f_{\mathrm{BC}}(\mathbf{x})
=
x_1^2
+
10^6\sum_{i=2}^{D}x_i^2.
\end{equation}

Unlike the Discus Function, the ill-conditioning is concentrated in the last $D-1$ directions, yielding again a condition number of $10^6$.

\medskip

\noindent{\textbf{Sharp Ridge Function}}
\begin{equation}
f_{\mathrm{SR}}(\mathbf{x})
=
x_1^2
+
100\sqrt{\sum_{i=2}^{D}x_i^2}.
\end{equation}

The function combines a quadratic direction with a ridge-shaped structure, creating a narrow valley with a sharp change in curvature.

\medskip

\noindent{\textbf{Different Powers Function}}
\begin{equation}
f_{\mathrm{DP}}(\mathbf{x})
=
\left(
\sum_{i=1}^{D}
|x_i|^{p_i}
\right)^{1/2},p_i
=
2+4\frac{i-1}{D-1},
\qquad
i=1,\ldots,D.
\end{equation}

The exponents increase gradually from $2$ to $6$, producing directions with different growth rates and heterogeneous curvature.

\textbf{Rotated Functions}


\noindent{\textbf{Rotated Ellipsoidal Function}}
\begin{equation}
f_{\mathrm{RE}}(\mathbf{x})
=
\sum_{i=1}^{D}
\lambda_i z_i^2,
\qquad
\lambda_i
=
10^{6\frac{i-1}{D-1}}.
\end{equation}

\medskip

\noindent{\textbf{Rotated Discus Function}}
\begin{equation}
f_{\mathrm{RD}}(\mathbf{x})
=
10^6z_1^2
+
\sum_{i=2}^{D}z_i^2.
\end{equation}

\medskip

\noindent{\textbf{Rotated Bent Cigar Function}}
\begin{equation}
f_{\mathrm{RBC}}(\mathbf{x})
=
z_1^2
+
10^6\sum_{i=2}^{D}z_i^2.
\end{equation}

\medskip

\noindent{\textbf{Rotated Sharp Ridge Function}}
\begin{equation}
f_{\mathrm{RSR}}(\mathbf{x})
=
z_1^2
+
100\sqrt{\sum_{i=2}^{D}z_i^2}.
\end{equation}

\medskip

\noindent{\textbf{Rotated Different Powers Function}}
\begin{equation}
f_{\mathrm{RDP}}(\mathbf{x})
=
\left(
\sum_{i=1}^{D}
|z_i|^{p_i}
\right)^{1/2},p_i
=
2+4\frac{i-1}{D-1},
\qquad
i=1,\ldots,D.
\end{equation}

==> new_theorem.tex <==
```latex
\begin{theorem}[Numerical stability]
\label{thm:numerical-stability}
Let $f:\mathbb{R}^n\to\mathbb{R}$ be continuously differentiable with
$L$-Lipschitz continuous gradient on a compact set containing the iterates.
Consider the accelerated BFGS scheme
\[
x_{k+1}=x_k-\eta_kX_k\nabla f(x_k),
\qquad
Y_k=(1-\rho)X_k+\rho V_k,
\]
\[
X_{k+1}=\Phi_{\mathrm{BFGS}}(Y_k;s_k,\zeta_k),
\qquad
V_{k+1}=(1-\beta)V_k+(\beta-\gamma)Y_k+\gamma X_{k+1},
\]
where
\[
s_k=x_{k+1}-x_k,
\qquad
\zeta_k=\nabla f(x_{k+1})-\nabla f(x_k).
\]
Assume that the BFGS updates are well defined, that the matrices
$X_k$, $Y_k$ and $V_k$ are uniformly positive definite and bounded, and
that the step sizes satisfy a sufficient decrease condition. If
\[
2(1-\beta)^2(1-\rho)^2<1,
\]
then there exist constants $\kappa^*>0$ and $c_2>0$ such that, for every
$0<\kappa<\kappa^*$, the Lyapunov sequence
\[
\mathcal E_k=f(x_k)-f^*+\kappa\|X_k-V_k\|_F^2
\]
satisfies
\[
\mathcal E_{k+1}
\le
\mathcal E_k
-\frac{c_1}{2}\|\nabla f(x_k)\|^2
-c_2\|X_k-V_k\|_F^2 .
\]
Consequently, $\{\mathcal E_k\}$ is non-increasing and the accelerated
BFGS scheme is stable in the discrete Lyapunov sense.
\end{theorem}
```


==> stochastic_search_directions.tex <==
\section{Accelerated Geometry BFGS with stochastic search directions}
\label{sec:accelerated_stoch}

The proposed formulation incorporates controlled randomness directly into the search direction of the quasi-Newton method. Unlike approaches that introduce stochasticity in the gradient estimation or in the Hessian update, the noise is applied to the displacement vector, thereby preserving the deterministic structure of the update of $X_k$ as well as the local convergence properties of the BFGS scheme.

The motivation for this choice is to enhance the exploratory capability of the method and to reduce the likelihood of stagnation at local minima or in regions of low curvature. Recent results suggest that moderate probabilistic perturbations can improve the global behavior of quasi-Newton methods without degrading their local performance \cite{shi2022noise, guo2023overview, amos2020algorithm, peng2025finding}.

To preserve the descent nature of the search direction, the noise is designed to eliminate its component parallel to the gradient $g_k = \nabla f(x_k)$. Let $\epsilon \sim \mathcal{N}(0, I)$, and define
\begin{equation}
\xi_k = \epsilon - \frac{\epsilon^\top g_k}{g_k^\top g_k} , g_k,
\label{eq:projected_noise}
\end{equation}
so that $g_k^\top \xi_k = 0$. The stochastic direction is then given by
\begin{equation}
\tilde{s}_k = s_k + \tau_k \xi_k,
\label{eq:stochastic_direction_projected}
\end{equation}
where $s_k = -X_k \nabla f(x_k)$, and $\tau_k > 0$ controls the magnitude of the perturbation.


The orthogonality of $\xi_k$ ensures that
$$
g_k^\top \tilde{s}_k = g_k^\top s_k,
$$
preserving the descent condition. Moreover, since $\mathbb{E}[\xi_k]=0$, we have $\mathbb{E}[\tilde{s}_k]=s_k$, so that the average behavior of the method is in agreement with that of the deterministic scheme.

The noise magnitude is controlled by a temperature factor $\tau_k$ that decays over iterations, for example,
\begin{equation}
\tau_k = \frac{\tau_0}{1 + \lambda k}, \qquad \lambda > 0,
\label{eq:temperature_decay}
\end{equation}
which allows a gradual transition between an initial exploratory phase and a local refinement regime. This mechanism is consistent with the cooling strategies used in stochastic methods and ensures that the perturbation variance tends to zero, preserving the asymptotic dynamics of the deterministic method \cite{guo2023overview}.

The iterate is updated by
$$
x_{k+1} = x_k + \eta_k \tilde{s}_k,
$$
with $\eta_k$ obtained by an appropriate line search. In this context, the stochastic term introduces tangential variations to the level sets of the objective function, increasing the directional diversity without compromising the overall direction of descent.

The method preserves the deterministic core of the accelerated BFGS while incorporating a projected, smoothly decaying noise component in the search direction. This modification broadens the exploratory ability of the algorithm and improves its robustness in nonconvex scenarios, remaining consistent with the structural properties established in the previous analysis.

Algorithm~\ref{alg:bfgs_ac_stoc} summarizes the proposed formulation, combining the accelerated geometry BFGS update with a projected stochastic perturbation in the search direction. The decay of $\tau_k$ induces a gradual transition from an exploratory initial phase to a local refinement regime, while the parameters $\rho$ and $\beta$ are chosen within the ranges $(0,\rho_{\max})$ and $(\beta_{\min},1)$ established by the stability analysis, ensuring preservation of structural properties in the cone $\mathbb{S}_{++}^n$.

%The presented formulation defines an accelerated stochastic extension of BFGS whose theoretical analysis guaranties stability and geometric coherence. It remains to empirically evaluate the impact of these modifications in terms of solution quality and computational efficiency.

%To this end, we conduct a comparison between classical BFGS, accelerated BFGS, and the accelerated version with a stochastic component on a set of many‑objective scalarized problems. This analysis isolates the effect of each proposed mechanism, assessing its contribution to algorithm performance in more complex scenarios.




\begin{algorithm}%[H]
\caption{Accelerated Geomery BFGS with Stochastic Component in the Search Direction (AGS-BFGS)}
\label{alg:bfgs_ac_stoc}
\begin{algorithmic}[1]
\REQUIRE $x_0$, $H_0 = I$, $U_0 = I$, $\tau_0$, $\lambda$, $\rho$, $\beta$, $\eta$, $\sigma$
\STATE \textbf{Evaluate} $f(x_0)$ and $g_0 = \nabla f(x_0)$
\FOR{$k = 0,1,2,\dots$ \textbf{until convergence}}
    \STATE $d_k \gets -H_k g_k$ \COMMENT{Deterministic descent direction}
    \STATE \textbf{Generate} noise $\varepsilon \sim \mathcal{N}(0,I)$
    \STATE \textbf{Project} $\varepsilon$ orthogonally to the gradient:
        $$
        \xi_k = \varepsilon - \frac{\varepsilon^\top g_k}{g_k^\top g_k}\, g_k
        $$
    \STATE \textbf{Compute temperature}: $\tau_k = \tau_0 / (1 + \lambda k)$
    \STATE \textbf{Stochastic direction}: $d_k \gets d_k + \tau_k \xi_k$
    \IF{$g_k^\top d_k > 0$}
        \STATE $d_k \gets -H_k g_k$ \COMMENT{Correction to maintain descent direction}
    \ENDIF
    \STATE \textbf{Determine} $\eta_k = \eta^m$ via Armijo line search, with $m$ minimal such that
        $$
        f(x_k + \eta_k d_k) \le f(x_k) + \sigma \eta_k g_k^\top d_k
        $$
    \STATE \textbf{Update iterate}: $x_{k+1} = x_k + \eta_k d_k$
    \STATE \textbf{Compute} $g_{k+1} = \nabla f(x_{k+1})$
    \STATE \textbf{Set} $s_k = x_{k+1} - x_k$, \quad $y_k = g_{k+1} - g_k$
    \IF{$y_k^\top s_k > 0$}
        \STATE $Y_k \gets (1-\rho)H_k + \rho V_k$
        \STATE $\phi_k \gets 1/(y_k^\top s_k)$
        \STATE $W_k \gets I - \phi_k s_k y_k^\top$
        \STATE $H_{k+1} \gets W_k Y_k W_k^\top + \phi_k\, s_k s_k^\top$
        \STATE $V_{k+1} \gets (1-\beta)V_k + \beta H_{k+1}$
    \ELSE
        \STATE $H_{k+1} \gets H_k$, \quad $V_{k+1} \gets V_k$
    \ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}

